Feature Removal Is a Unifying Principle for Model Explanation Methods

Researchers have proposed a wide variety of model explanation approaches, but it remains unclear how most methods are related or when one method is preferable to another. We examine the literature and find that many methods are based on a shared principle of explaining by removing - essentially, measuring the impact of removing sets of features from a model. These methods vary in several respects, so we develop a framework for removal-based explanations that characterizes each method along three dimensions: 1) how the method removes features, 2) what model behavior the method explains, and 3) how the method summarizes each feature's influence. Our framework unifies 26 existing methods, including several of the most widely used approaches (SHAP, LIME, Meaningful Perturbations, permutation tests). Exposing the fundamental similarities between these methods empowers users to reason about which tools to use, and suggests promising directions for ongoing model explainability research.

==> Explaining by Removing - MLRSA/0_abstract.tex <==
\begin{abstract}
Researchers have proposed a wide variety of model explanation approaches, but it remains unclear how most methods are related or when one method is preferable to another. We examine the literature and find that many methods are based on a shared principle of \textit{explaining by removing}---essentially, measuring the impact of removing sets of features from a model. These methods vary in several respects, so we develop a framework for \textit{removal-based explanations} that characterizes each method along three dimensions: 1)~how the method removes features, 2)~what model behavior the method explains, and 3)~how the method summarizes each feature's influence. Our framework unifies 26 existing methods, including several of the most widely used approaches (SHAP, LIME, Meaningful Perturbations, permutation tests). Exposing the fundamental similarities between these methods empowers users to reason about which tools to use, and suggests promising directions for ongoing model explainability research.\footnote{Since its
% this work's
initial publication, an extended version
of this work
% has appeared
was published in the Journal of Machine Learning Research~\cite{covert2021explaining}.}
\end{abstract}


==> Explaining by Removing - MLRSA/1_intro.tex <==
\section{Introduction}

The proliferation of black-box models has made machine learning (ML) explainability an increasingly important subject, and researchers have now proposed a wide variety of model explanation approaches \cite{breiman2001random, chen2018learning, covert2020understanding, lundberg2017unified, owen2014sobol, petsiuk2018rise, ribeiro2016should, sundararajan2017axiomatic, vstrumbelj2009explaining, zeiler2014visualizing}. Despite progress in the field, the relationships and trade-offs among these methods have not been rigorously investigated, and researchers have not always formalized their fundamental ideas about how to interpret models~\citep{lipton2018mythos}. This makes the literature difficult to navigate and raises questions about whether existing methods relate to human processes for explaining complex decisions~\citep{miller2017explainable, miller2019explanation}.

Here, we present a comprehensive framework that unifies a substantial portion of the model explanation literature. Our framework is based on the observation that many methods can be understood as \textit{simulating feature removal} to quantify each feature's influence on a model. The intuition behind these methods is similar (depicted in Figure~\ref{fig:concept}), but each one takes a slightly different approach to the removal operation: some replace features with neutral values~\citep{petsiuk2018rise, zeiler2014visualizing}, others marginalize over a distribution of values~\citep{lundberg2017unified, strobl2008conditional}, and still others train separate models for each subset of features~\citep{lipovetsky2001analysis, vstrumbelj2009explaining}. These methods also vary in other respects, as we describe below.

We refer to this class of approaches as \textit{removal-based explanations} and identify 26\footnote{This total count does not include minor variations on the approaches we identified.} existing methods that rely on the feature removal principle, including several of the most widely used methods (SHAP, LIME, Meaningful Perturbations, permutation tests). We then develop a framework that shows how each method arises from various combinations of three choices: 1)~how the method removes features from the model, 2)~what model behavior the method analyzes, and 3)~how the method summarizes each feature's influence on the model. By characterizing each method in terms of three precise mathematical choices, we are able to systematize their shared elements and reveal that they rely on the same fundamental approach---feature removal.

\input{inserts/concept}

The model explanation field has grown significantly in the past decade, and we take a broader view of the literature than existing unification theories. Our framework's flexibility lets us establish links between disparate classes of methods (e.g., computer vision-focused methods, global methods, game-theoretic methods, feature selection methods) and show that the literature is more interconnected than previously recognized. Exposing these underlying connections potentially raises questions about the degree of novelty in recent work, but we also believe that each method has the potential to offer unique advantages, either conceptually or computationally.

Through this work, we hope to empower users to reason more carefully about which tools to use, and we aim to provide researchers with new theoretical tools to build on in ongoing research. Our contributions include:

\begin{enumerate}[leftmargin=2pc]
    \item We present a framework that unifies 26 existing explanations methods. Our framework for \textbf{removal-based explanations} integrates classes of methods that were previously considered disjoint, including local and global approaches, as well as feature attribution and feature selection methods.
    
    \item We develop new mathematical tools to represent different approaches to removing features from ML models. \textit{Subset functions} provide a common representation for various feature removal techniques, revealing that this choice is interchangeable between methods.
    % \item We develop new mathematical tools to represent different approaches to removing features from brittle ML models. \textit{Subset functions} and \textit{model extensions} provide a common representation for various feature removal techniques, revealing that this choice is interchangeable between methods.
    
    \item We generalize numerous explanation methods to express them within our framework, exposing connections that were often not apparent in the original works. In particular, for several approaches we disentangle the implicit aims of the methods from the approximations that make them usable in practice.
\end{enumerate}

We begin with background on the model explanation problem and a review of prior work (Section~\ref{sec:background}), and we then introduce our framework (Section~\ref{sec:removal_based_explanations}). The remaining
% next several
sections examine our framework in detail by showing how it encompasses existing methods. Section~\ref{sec:removal} discusses how methods remove features, Section~\ref{sec:behaviors} formalizes the model behaviors analyzed by each method, and Section~\ref{sec:explanations} describes each method's approach to summarizing each feature's influence. Finally, Section~\ref{sec:discussion} concludes and discusses future research directions.


==> Explaining by Removing - MLRSA/2_background.tex <==
\section{Background} \label{sec:background}

Here, we introduce the model explanation problem and briefly review existing approaches and related unification theories.

\subsection{Preliminaries}

Consider a supervised ML model $f$ that is used to predict a response variable $Y \in \mathcal{Y}$ using the input $X = (X_1, X_2, \ldots, X_d)$, where each $X_i$ represents an individual feature, such as a patient's age. We use uppercase symbols (e.g., $X$) to denote random variables and lowercase ones (e.g., $x$) to denote their values. We also use $\mathcal{X}$ to denote the domain of the full feature vector $X$ and $\mathcal{X}_i$ to denote the domain of each feature $X_i$. Finally, $x_S \equiv \{x_i : i \in S\}$ denotes a subset of features for $S \subseteq D \equiv \{1, 2, \ldots d\}$, and $\bar S \equiv D \setminus S$ represents a set's complement.

ML interpretability broadly aims to provide insight into how models make predictions. This is particularly important when $f$ is a complex model, such as a neural network or a decision forest. The most active area of research in the field is \textit{local interpretability}, which explains individual predictions, such as an individual patient diagnosis~\cite{lundberg2017unified, ribeiro2016should, sundararajan2017axiomatic}; in contrast, \textit{global interpretability} explains the model's behavior across the entire dataset~\cite{breiman2001random, covert2020understanding, owen2014sobol}. Both problems are usually addressed using \textit{feature attribution}, where a score is assigned to explain each feature's influence. However, recent work has also proposed the strategy of \textit{local feature selection}~\citep{chen2018learning}, and other papers have introduced methods to identify sets of relevant features~\citep{dabkowski2017real, fong2017interpretable, zhou2014object}.

Whether the aim is local or global interpretability, explaining the inner workings of complex models is fundamentally difficult, so it is no surprise that researchers keep devising new approaches. Commonly cited categories of approaches include perturbation-based methods~\citep{lundberg2017unified, zeiler2014visualizing}, gradient-based methods~\citep{simonyan2013deep, sundararajan2017axiomatic}, and inherently interpretable models~\citep{rudin2019stop, zhou2016learning}. However, these categories refer to loose collections of approaches that seldom share a precise mechanism.

Besides the inherently interpretable models, virtually all of these approaches generate explanations by considering some class of perturbation to the input and using the outcomes to explain each feature's influence. Certain methods consider infinitesimal perturbations by calculating gradients~\citep{simonyan2013deep, smilkov2017smoothgrad, sundararajan2017axiomatic, xu2020attribution}, but there are many possible perturbations~\citep{fong2017interpretable, lundberg2017unified, ribeiro2016should, zeiler2014visualizing}. Our work is based on the observation that numerous perturbation strategies can be understood as simulating feature removal.

\subsection{Related work}

Prior work has made solid progress in exposing connections among disparate explanation methods. Lundberg \& Lee proposed the unifying framework of \textit{additive feature attribution methods} and showed that LIME, DeepLIFT, LRP and QII are all related to SHAP~\citep{bach2015pixel, datta2016algorithmic, lundberg2017unified, ribeiro2016should, shrikumar2016not}. Similarly, Ancona et al. showed that Grad * Input, DeepLIFT, LRP and Integrated Gradients are all understandable as modified gradient backpropagations~\cite{ancona2017towards, shrikumar2016not, sundararajan2017axiomatic}. Most recently, Covert et al. showed that several global explanation methods can be viewed as \textit{additive importance measures}, including permutation tests, Shapley Net Effects, and SAGE~\citep{breiman2001random, covert2020understanding, lipovetsky2001analysis}.

Relative to prior work, the unification we propose is considerably broader but nonetheless precise. As we describe below, our framework characterizes methods along three dimensions. The choice of how to remove features has been considered by many works~\citep{aas2019explaining, frye2020shapley, hooker2019please, janzing2019feature, lundberg2017unified, merrick2019explanation, sundararajan2019many, chang2018explaining, agarwal2019explaining}. The choice of what model behavior to analyze has been considered explicitly by only a few works~\citep{covert2020understanding, lundberg2020local}, as has the choice of how to summarize each feature's influence based on a set function~\citep{covert2020understanding, datta2016algorithmic, frye2019asymmetric, lundberg2017unified, vstrumbelj2009explaining}. To our knowledge, ours is the first work to consider all three dimensions simultaneously and unite them under a single framework.

Besides the methods that we focus on, there are also methods that do not rely on the feature removal principle. We direct readers to survey articles for a broader overview of the literature~\cite{adadi2018peeking, guidotti2018survey}.


==> Explaining by Removing - MLRSA/3_rbe.tex <==
\section{Removal-Based Explanations} \label{sec:removal_based_explanations}

We now introduce our framework and briefly describe the methods it unifies.

\input{inserts/table_jmlr}

\subsection{A unified framework}

We develop a unified model explanation framework by connecting methods that define a feature's influence through the impact of removing it from a model. This perspective encompasses a substantial portion of the explainability literature: we find that 26 existing methods rely on this mechanism, including many of the most widely used approaches~\citep{breiman2001random, fong2017interpretable, lundberg2017unified, ribeiro2016should}.

These methods all remove groups of features from the model, but, beyond that, they take a diverse set of approaches. For example, LIME fits a linear model to an \textit{interpretable representation} of the input~\citep{ribeiro2016should}, L2X selects the most informative features for a single example~\citep{chen2018learning}, and Shapley Effects examines how much of the model's variance is explained by each feature~\citep{owen2014sobol}. Perhaps surprisingly, their differences are easy to systematize because each method removes discrete sets of features.
% because these methods all remove discrete sets of features, their differences are easy to systematize.

As our main contribution, we introduce a framework that shows how these methods can be specified using only three choices.

\begin{definition}
    {\normalfont \textbf{Removal-based explanations}} are model explanations that quantify the impact of removing sets of features from the model. These methods are determined by three choices:
    
    \begin{enumerate}
        \item (Feature removal) How the method removes features from the model (e.g., by setting them to default values or by marginalizing over a distribution of values)
        \item (Model behavior) What model behavior the method analyzes (e.g., the probability of the true class or the model loss)
        \item (Summary technique) How the method summarizes each feature's impact on the model (e.g., by removing a feature individually or by calculating the Shapley values)
    \end{enumerate}
\end{definition}

This precise yet flexible framework represents each choice as a specific type of mathematical function, as we show later. The framework unifies disparate explanation methods by unraveling each method's separate choices along these three dimensions. By allowing explicit reasoning about the trade-offs among different approaches, this perspective offers a step towards a better understanding of the literature.

% This precise yet flexible framework represents each choice as a specific type of mathematical function, as we show later. The framework unifies disparate explanation methods,
% % parts of the explainability literature,
% and, by unraveling each method's choices, offers a
% % first
% step towards a better understanding of the literature by allowing explicit reasoning about the trade-offs among different approaches.

\input{inserts/methods_grid_jmlr}

\subsection{Overview of existing approaches}

We now outline some of our findings, which we present in more detail in the following
% next several
sections. In particular, we preview how existing methods fit into our framework and highlight groups of methods that appear similar in light of our feature removal perspective.

Table~\ref{tab:methods} lists the methods unified by our framework
% this framework unifies
(with acronyms introduced in the next section). These methods represent diverse parts of the interpretability literature, including global methods~\citep{breiman2001random, owen2014sobol}, computer vision-focused methods~\citep{petsiuk2018rise, zeiler2014visualizing, zhou2014object, fong2017interpretable}, game-theoretic methods~\citep{covert2020understanding, lundberg2017unified, vstrumbelj2010efficient} and feature selection methods~\citep{chen2018learning, fong2019understanding, yoon2018invase}. They all have a shared
% are all unified by their
reliance on feature removal.

Disentangling the details of each method shows that many approaches share one or more of the same choices. For example, most methods choose to explain individual predictions (the model behavior), and the most popular summary technique is the Shapley value~\citep{shapley1953value}. These common choices raise important questions about how different these methods truly are and how their choices are justified.
% ; we explore these questions in the remainder of the paper.

To highlight similarities among the methods, we visually depict the space of removal-based explanations in Figure~\ref{fig:methods_grid}. Visualizing our framework reveals several regions in the space of methods that are crowded (e.g., methods that marginalize out removed features with their conditional distribution and that calculate Shapley values), while certain methods are relatively unique and spatially isolated (e.g., RISE, or LIME for tabular data).
% ; L2X and INVASE).
Empty positions in the grid reveal opportunities to develop new methods; in fact, every empty position represents a viable new explanation method.
% ; we explore these possibilities in our experiments (Section~\ref{sec:experiments}).

\input{inserts/common_jmlr}

Finally, Table~\ref{tab:common_combinations} shows groups of methods that differ in only one dimension of the framework. These methods are neighbors in the space of explanation methods (Figure~\ref{fig:methods_grid}), and it is remarkable how many instances of neighboring methods exist in the literature. Certain methods even have neighbors along every dimension of the framework (e.g., SHAP, SAGE, Occlusion, PredDiff, conditional permutation tests), reflecting how intimately connected the literature has become. The explainability literature is evolving and maturing, and our perspective provides a new approach for reasoning about the subtle relationships and trade-offs among existing approaches.

==> Explaining by Removing - MLRSA/4_removal.tex <==
\section{Feature Removal} \label{sec:removal}

Here, we define the mathematical tools necessary to remove features from ML models and then examine how existing explanation methods remove features.

\subsection{Functions on subsets of features}

Most ML models make predictions given a specific set of features $X = (X_1, \ldots, X_d)$.
% In machine learning, we typically use models that make predictions given certain features $X = (X_1, \ldots, X_d)$.
Mathematically, these models are functions are of the form $f: \mathcal{X} \mapsto \mathcal{Y}$, and we use $\mathcal{F}$ to denote the set of all such possible mappings. The principle behind removal-based explanations is to remove certain features to understand their impact on a model, but since most models require all the features to make predictions, removing a feature is more difficult
% complicated
than simply not giving the model access to it. 

% We begin by defining the mathematical tools necessary to represent functions on subsets of features.
To remove features from a model, or to make predictions given a subset of features, we require a different mathematical object than $f \in \mathcal{F}$. Instead of functions with domain $\mathcal{X}$, we consider functions with domain $\mathcal{X} \times \mathcal{P}(D)$, where $\mathcal{P}(D)$ denotes the power set of $D \equiv \{1, \ldots, d\}$. To ensure invariance to the held-out features, these functions must depend only on a set of features specified by a subset $S \in \mathcal{P}(D)$,
% features specified by the subset $S \in \mathcal{P}(D)$,
so we formalize \textit{subset functions} as follows.

% \vskip 0.125in
\vskip 0.2in

\begin{definition} \label{def:subset_function}
    {\normalfont A \textbf{subset function}} is a mapping of the form
    
    \begin{equation*}
        F: \mathcal{X} \times \mathcal{P}(D) \mapsto \mathcal{Y}
    \end{equation*}
    
    \noindent that is invariant to the dimensions that are not in the specified subset. That is, we have $F(x, S) = F(x', S)$ for all $(x, x', S)$ such that $x_S = x'_S$. We define $F(x_S) \equiv F(x, S)$ for convenience because the held-out values $x_{\bar S}$ are not used by $F$.
\end{definition}

A subset function's invariance property is crucial to ensure that only the specified feature values determine the function's output, while guaranteeing that the other feature values do not matter. Another way of viewing subset functions is that they simulate the use of partial inputs or missing data.
% simulate the presence of missing data.
While we use $\mathcal{F}$ to represent standard prediction functions, we use $\mathfrak{F}$ to denote the set of all possible subset functions.

We introduce subset functions here because they help conceptualize how different methods remove features from ML models. Removal-based explanations typically begin with an existing model $f \in \mathcal{F}$, and in order to quantify each feature's influence, they must establish a convention for removing it from the model. A natural approach is to define a subset function $F \in \mathfrak{F}$ based on the original model $f$. To formalize this idea, we define a model's \textit{subset extension} as follows.

\begin{definition} \label{def:extension}
    A {\normalfont \textbf{subset extension}} of a model $f \in \mathcal{F}$ is a subset function $F \in \mathfrak{F}$ that agrees with $f$ in the presence of all features. That is, the model $f$ and its subset extension $F$ must satisfy
    
    \begin{equation*}
        F(x) = f(x) \quad \forall x \in \mathcal{X}.
    \end{equation*}
\end{definition}

% \begin{definition} \label{def:extension}
%     An {\normalfont \textbf{extension}} of a model $f \in \mathcal{F}$ is a subset function $F \in \mathfrak{F}$ that agrees with $f$ in the presence of all features. That is, the model $f$ and its extension $F$ must satisfy
    
%     \begin{equation*}
%         F(x) = f(x) \quad \forall x \in \mathcal{X}.
%     \end{equation*}
% \end{definition}

As we show next, specifying a subset function $F \in \mathfrak{F}$, often as a subset extension of an existing model $f \in \mathcal{F}$, is the first step towards defining a removal-based explanation.

% As we show next, extending an existing model is the first step towards specifying a removal-based explanation method.

\subsection{Removing features from machine learning models} \label{sec:missingness_strategies}

% Removal-based explanations have
Existing methods have devised numerous ways to evaluate models while withholding groups of features. Although certain methods use different terminology to describe their approaches (e.g., deleting information, ignoring features, using neutral values, etc.), the goal of all these methods is to measure a feature's influence through the impact of removing it from the model. Most proposed techniques can be understood as subset extensions $F \in \mathfrak{F}$ of an existing model $f \in \mathcal{F}$ (Definition~\ref{def:extension}).

We now examine each method's specific approach (see Appendix~\ref{app:methods} for more details):
% We now examine each method's approach. Since our descriptions are brief, we provide more details about each method in Appendix~\ref{app:methods}. The various strategies used to remove features include:
% We now examine the approaches each method takes. Since our descriptions are brief, we provide more details about each method in Appendix~\ref{app:methods}. The various strategies used to remove features include:

\begin{itemize}[leftmargin=2pc]
    \item (Zeros) Occlusion~\citep{zeiler2014visualizing}, RISE~\citep{petsiuk2018rise} and causal explanations (CXPlain)~\citep{schwab2019cxplain} remove features simply by setting them to zero:
    
    \begin{equation}
        F(x_S) = f(x_S, 0). \label{eq:zeros}
    \end{equation}
    
    \item (Default values) LIME for image data~\citep{ribeiro2016should} and the Masking Model method (MM)~\citep{dabkowski2017real} remove features by setting them to user-defined default values (e.g., gray pixels for images). Given default values $r \in \mathcal{X}$, these methods calculate

    \begin{equation}
        F(x_S) = f(x_S, r_{\bar S}). \label{eq:default}
    \end{equation}
    
    This is a generalization of the previous approach, and in some cases features may be given different default values (e.g., their mean).
    
    % LIME does not necessarily toggle features on and off. There are interpretable features that may or may not be binary. There's some notion of a neighborhood, which in the case of binary features applies some weighting to different coalitions of features.
    % For tabular LIME, see https://github.com/marcotcr/lime/blob/master/lime/discretize.py#L127 and https://github.com/marcotcr/lime/blob/master/lime/lime_tabular.py#L544
    
    % \item (Missingness during training) Learning to Explain (L2X)~\citep{chen2018learning} and Instance-wise Variable Selection (INVASE)~\citep{yoon2018invase} use a model that has missingness introduced at training time. Removed features are replaced with zeros so that the model makes the following approximation:
    
    % \begin{equation}
    %     F(x_S) = f(x_S, 0) \approx p(Y | X_S = x_S).
    % \end{equation}
    
    % This approach differs from Occlusion and RISE because the model is trained to recognize zeros as missing values rather than zero-valued features. A model trained with a loss function other than cross entropy loss would approximate a different quantity (e.g., the conditional expectation $\E[Y | X_S = x_S]$ for MSE loss).
    
    \item (Extend pixel values) Minimal image representation (MIR)~\citep{zhou2014object} removes features in images by extending the values of neighboring pixels. This effect is achieved through a gradient-space manipulation.
    % See https://github.com/zhoubolei/cnnvisualizer/blob/master/minimal_image/tools/reconstruct.m and https://github.com/zhoubolei/cnnvisualizer/blob/master/minimal_image/tools/buildGradientBases.m
    
    \item (Blurring) Meaningful Perturbations (MP)~\citep{fong2017interpretable} and Extremal Perturbations (EP)~\citep{fong2019understanding} remove features from images by blurring them with a Gaussian kernel. This approach is \textit{not} an extension of $f$ because the blurred image retains dependence on the removed features. Blurring fails to remove large, low frequency objects (e.g., mountains), but it provides an approximate way to remove information from images.
    
    \item (Generative model) FIDO-CA~\cite{chang2018explaining} removes feature by replacing them with a sample from a conditional generative model (e.g.~\cite{yu2018generative}). The held-out features are drawn from a generative model represented by $p_G(X_{\bar S} | X_S)$, or $\tilde x_{\bar S} \sim p_G(X_{\bar S} | X_S)$ and predictions are made as follows:
    
    \begin{equation}
        F(x_S) = f(x_S, \tilde x_{\bar S}).
    \end{equation}
    
    \item (Marginalize with conditional) SHAP~\cite{lundberg2017unified}, LossSHAP~\cite{lundberg2020local} and SAGE~\cite{covert2020understanding} present a strategy for removing features by marginalizing them out using their conditional distribution, denoted by $p(X_{\bar S} \mid X_S = x_S)$:
    
    \begin{equation}
        F(x_S) = \E\big[f(X) \mid X_S = x_S\big]. \label{eq:conditional_expectation}
    \end{equation}
    
    This approach is computationally challenging in practice, but recent works try to achieve close approximations~\cite{aas2019explaining, aas2021explaining, frye2020shapley}. Shapley Effects~\cite{owen2014sobol} implicitly uses this convention to analyze function sensitivity, while conditional permutation tests~\cite{strobl2008conditional} and Prediction Difference Analysis (PredDiff~\cite{zintgraf2017visualizing}) propose simple approximations, with the latter conditioning only on groups of bordering pixels.

    % \item (Marginalize with conditional) SHAP~\citep{lundberg2017unified}, LossSHAP~\citep{lundberg2020local} and SAGE~\citep{covert2020understanding} present a strategy for removing features by marginalizing them out using their conditional distribution $p(X_{\bar S} \; | \; X_S = x_S)$:
    
    % \begin{equation}
    %     F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]. \label{eq:conditional_expectation}
    % \end{equation}
    
    % This approach is computationally challenging in practice, but recent work tries to achieve close approximations~\citep{aas2019explaining, frye2020shapley}. Shapley Effects~\citep{owen2014sobol} implicitly uses this convention to analyze function sensitivity, while conditional permutation tests~\citep{strobl2008conditional} and Prediction Difference Analysis (PredDiff)~\citep{zintgraf2017visualizing} do so to remove individual features.

    \item (Marginalize with marginal) KernelSHAP (a practical implementation of SHAP)~\cite{lundberg2017unified} removes
    % and SAGE sampling (a practical implementation of SAGE) remove
    features by marginalizing them out using their joint marginal distribution $p(X_{\bar S})$:
    % using the \textit{interventional expectation}.
    % The removed features are marginalized out using their joint marginal distribution $p(X_{\bar S})$:
    
    \begin{equation}
        F(x_S) = \E\big[f(x_S, X_{\bar S})\big]. \label{eq:marginal}
    \end{equation}
    
    This is the default behavior in SHAP's implementation,\footnote{\url{https://github.com/slundberg/shap}} and recent work discusses the benefits of this approach~\citep{janzing2019feature}. Permutation tests~\citep{breiman2001random} also use this approach to remove individual features from a model.

    \item (Marginalize with product of marginals) Quantitative Input Influence (QII)~\citep{datta2016algorithmic} removes held-out features by marginalizing them out using the product of the marginal distributions $p(X_i)$:
    
    \begin{equation}
        F(x_S) = \E_{\prod_{i \in D} p(X_i)}\big[f(x_S, X_{\bar S})\big]. \label{eq:qii}
    \end{equation}
    
    \item (Marginalize with uniform) The updated version of the Interactions Method for Explanation (IME)~\citep{vstrumbelj2010efficient}
    % IME~\citep{vstrumbelj2010efficient}
    removes features by marginalizing them out with a uniform distribution over the feature space. If we let $u_i(X_i)$ denote a uniform distribution over $\mathcal{X}_i$ (with extremal values defining the boundaries for continuous features), then features are removed as follows:
    
    \begin{equation}
        F(x_S) = \E_{\prod_{i \in D} u_i(X_i)}\big[f(x_S, X_{\bar S})\big]. \label{eq:ime_uniform}
    \end{equation}
    
    \item (Marginalize with replacement distributions) LIME for tabular data replaces features with independent draws from \textit{replacement distributions} (our term), each of which depends on the original feature values. When a feature $X_i$ with value $x_i$ is removed, discrete features are drawn from the distribution $p(X_i \; | \; X_i \neq x_i)$; when quantization is used for continuous features (LIME's default behavior\footnote{\url{https://github.com/marcotcr/lime}}), continuous features are simulated by first generating a different quantile and then simulating from a truncated normal distribution within that bin. If we denote each feature's replacement distribution given the original value $x_i$ as $q_{x_i}(X_i)$, then LIME for tabular data removes features as follows:
    
    \begin{equation}
        F(x, S) = \E_{\prod_{i \in D} q_{x_i}(X_i)}\big[f(x_S, X_{\bar S})\big].
    \end{equation}
    
    Although this function $F$ agrees with $f$ given all features, it is \textit{not} an extension because it does not satisfy the invariance property for subset functions.
    
    \item (Tree distribution) Path-dependent TreeSHAP~\cite{lundberg2020local} removes features using the distribution induced by the underlying tree model, which roughly approximates the conditional distribution. When splits for held-out
    % removed
    features are encountered in the model's trees, TreeSHAP averages predictions from the multiple paths in proportion to how often the dataset follows each path.
    
    \item (Surrogate model) Learning to Explain (L2X~\cite{chen2018learning}) and REAL-X~\cite{jethani2021have} train separate surrogate models $F$ to match the original model's predictions when groups of features are held out. The surrogate model accommodates missing features, allowing us to represent it as a subset function $F \in \mathfrak{F}$, and it aims to provide the following approximation:
    
    \begin{equation}
        F(x_S) \approx \E\big[f(X) \mid X_S = x_S\big]. \label{eq:surrogate}
    \end{equation}
    
    The surrogate model approach was also proposed separately in the context of Shapley values~\cite{frye2020shapley}.
    
    \item (Missingness during training) Instance-wise Variable Selection (INVASE~\cite{yoon2018invase}) uses a model that has missingness introduced at training time. Removed features are replaced with zeros, so that the model makes the following approximation:
    
    \begin{equation}
        F(x_S) = f(x_S, 0) \approx p(Y \mid X_S = x_S). \label{eq:missingness}
    \end{equation}
    
    This approximation occurs for models trained cross entropy loss, but other loss functions may lead to different results (e.g., the conditional expectation for MSE loss). Introducing missingness during training differs from the default values approach because the model is trained to recognize zeros (or other replacement values) as missing values rather than zero-valued features.
    
    \item (Separate models) The original version of IME~\cite{vstrumbelj2009explaining} is not based on a single model $f$, but rather on separate models trained for each feature subset, or $\{f_S : S \subseteq D\}$. The prediction for a subset of features is given by that subset's model:
    
    \begin{equation}
        F(x_S) = f_S(x_S).
    \end{equation}
    
    Shapley Net Effects~\cite{lipovetsky2001analysis} uses an identical approach in the context of linear models, with SPVIM generalizing the approach to black-box models~\cite{williamson2020efficient}. Similarly, feature ablation, also known as leave-one-covariate-out (LOCO~\cite{lei2018distribution}), trains models to remove individual features, and the univariate predictors approach (used mainly for feature selection) uses models trained with individual features~\cite{guyon2003introduction}.
    Although the separate models approach is technically a subset extension of the model $f_D$ trained with all features, its predictions given subsets of features are not based on $f_D$.
    
    % \item (Tree distribution) Dependent TreeSHAP~\citep{lundberg2020local} removes features using the distribution induced by the model, which roughly approximates the conditional distribution. When splits for removed features are encountered in the model's trees, TreeSHAP averages predictions from the multiple paths in proportion to how often the dataset follows each path.
    
    % \item (Separate models) Shapley Net Effects~\citep{lipovetsky2001analysis} and the original version of IME~\citep{vstrumbelj2009explaining}
    % % the Interactions Method for Explanation (IME,~\citep{vstrumbelj2009explaining})
    % are not based on a single model $f$ but rather on separate models trained for each subset, which we denote as $\{f_S : S \subseteq D\}$. The prediction for a subset of features is given by that subset's model:
    
    % \begin{equation}
    %     F(x_S) = f_S(x_S).
    % \end{equation}
    
    % Although this approach is technically an extension of the model $f_D$ trained with all features, its predictions given subsets of features are not based on $f_D$. Similarly, feature ablation, also known as leave-one-covariate-out (LOCO)~\citep{lei2018distribution}, trains models to remove individual features, and the univariate predictors approach (used mainly for feature selection) uses models trained with individual features~\citep{guyon2003introduction}.
\end{itemize}

Most of these approaches are subset extensions of an existing model $f$, so our formalisms provide useful tools for understanding how removal-based explanations remove features from models. However, consider two exceptions: the blurring technique (MP and EP) and LIME's approach with tabular data. Both provide functions of the form $F: \mathcal{X} \times \mathcal{P}(D) \mapsto \mathcal{Y}$ that agree with $f$ given all features, but that still exhibit dependence on removed features. Based on our mathematical characterization of subset functions and their invariance to held-out features, we argue that these two approaches do not fully remove features from the model. We conclude that the first dimension of our framework amounts to choosing an extension $F \in \mathfrak{F}$ of the model $f \in \mathcal{F}$.

% We defer consideration of the trade-offs among these approaches until Section~\ref{sec:information}, where we show that one way to remove features yields to connections with information theory
% % information-theoretic connections
% (marginalizing out removed features with the conditional distribution, Eq.~\ref{eq:conditional_expectation}).


==> Explaining by Removing - MLRSA/5_behaviors.tex <==
\section{Explaining Different Model Behaviors} \label{sec:behaviors}

Removal-based explanations all aim to demonstrate how a model works, but they can do so by analyzing a variety of model behaviors. We now consider the various choices of target quantities to observe as different features are withheld from the model.
% Many target quantities (i.e., the model behavior being explained) can be observed as different features are removed,
% % representing the choice of what model behavior to explain,
% so we now consider what options exist for removal-based explanations.
% % The choice of what to explain is represented by a target quantity that is observed as different features are removed, and we now consider what options exist for removal-based explanations.

The feature removal principle is flexible enough to explain virtually any function. For example, methods can explain a model's prediction, a model's loss function, a hidden layer in a neural network, or any node in a computation graph. In fact, removal-based explanations need not be restricted to the ML context: any function that accommodates missing inputs can be explained via feature removal by examining either its output or some function of its output as groups of inputs are removed. This perspective shows the broad potential applications for removal-based explanations.

However, since our focus is the ML context, we proceed by examining
% To explore the possibilities in the ML context, we examine
how existing model explanation methods work. Each method's target quantity can be understood as a function of the model output, which is represented by a subset function $F(x_S)$. Many methods explain the model output or a simple function of the output, such as the log-odds ratio. Other methods
% build on this by taking
take into account a measure of the model's loss, for either an individual input or the entire dataset. Ultimately, as we show below, each method generates explanations based on a set function of the form

\begin{equation*}
    u: \mathcal{P}(D) \mapsto \R,
\end{equation*}

\noindent which represents a value associated with each subset of features $S \subseteq D$. This set function represents the model behavior that a method is designed to explain.

We now examine the specific choices made by existing methods (see Appendix~\ref{app:methods} for further details on each method).
% For simplicity, we use $F$ to denote a subset function that is used to evaluate the model with subsets of features. (We direct readers to Appendix~\ref{app:methods} for further details on each method.)
The various model behaviors that methods analyze, and their corresponding set functions, include:

\begin{itemize}[leftmargin=2pc]
    \item (Prediction) Occlusion, RISE, PredDiff, MP, EP, MM, FIDO-CA, MIR, LIME, SHAP (including KernelSHAP and TreeSHAP), IME and QII all analyze a model's prediction for an individual input $x \in \mathcal{X}$:
    
    \begin{equation}
        u_x(S) = F(x_S). \label{eq:output_game}
    \end{equation}
    
    These methods examine how holding out different features makes an individual prediction either higher or lower. For multi-class classification models, methods often use a single output that corresponds to the class of interest, and they can optionally apply a simple function to the model's output (for example, using the log-odds ratio rather than the classification probability).
    
    \item (Prediction loss) LossSHAP and CXPlain take into account the true label $y$ for an input $x$ and calculate the prediction loss using a loss function $\ell$:
    
    \begin{equation}
        v_{xy}(S) = - \ell\big(F(x_S), y\big). \label{eq:shap_loss_game}
    \end{equation}
    
    By incorporating the label, these methods quantify whether certain features make the prediction more or less correct. Note that the minus sign is necessary to give the set function a higher value when more informative features are included.
    
    \item (Prediction mean loss) INVASE considers the expected loss for a given input $x$ according to the label's conditional distribution $p(Y \mid X = x)$:
    
    \begin{equation}
        v_x(S) = - \E_{p(Y \mid X = x)}\Big[\ell\big(F(x_S), Y\big)\Big]. \label{eq:pml_game}
    \end{equation}
    
    By averaging the loss across the label's distribution, INVASE highlights features that correctly predict what \textit{could} have occurred, on average.
    
    \item (Dataset loss) Shapley Net Effects, SAGE, SPVIM, feature ablation, permutation tests and univariate predictors consider the expected loss across the entire dataset:
    
    \begin{equation}
        v(S) = - \E_{XY}\Big[\ell\big(F(X_S), Y\big)\Big]. \label{eq:expected_loss_game}
    \end{equation}
    
    These methods quantify how much the model's performance degrades when different features are removed. This set function can also be viewed as the predictive power derived from sets of features~\citep{covert2020understanding}, and recent work has proposed a SHAP value aggregation that is a special case of this approach~\citep{frye2020shapley}.
    
    \item (Prediction loss w.r.t. output) L2X and REAL-X consider the loss between the full model output and the prediction given a subset of features:
    
    \begin{equation}
        w_x(S) = - \ell\big(F(x_S), F(x)\big). \label{eq:plo_game}
    \end{equation}
    
    These methods highlight features that on their own lead to similar predictions as the full feature set.
    
    \item (Dataset loss w.r.t. output) Shapley Effects considers the expected loss with respect to the full model output:
    
    \begin{equation}
        w(S) = - \E_X\Big[\ell\big(F(X_S), F(X)\big)\Big]. \label{eq:shapley_effects_game}
    \end{equation}
    
    Though related to the dataset loss approach~\citep{covert2020understanding}, this approach focuses on each feature's influence on the model output rather than on the model performance.
\end{itemize}

% \begin{itemize}[leftmargin=2pc]
%     \item (Prediction) Occlusion, RISE, PredDiff, MP, EP, MM, FIDO-CA, MIR, LIME, SHAP (including KernelSHAP and TreeSHAP), IME and QII all analyze a model's prediction for an individual input $x \in \mathcal{X}$:
    
%     \begin{equation}
%         v_x(S) = F(x_S). \label{eq:output_game}
%     \end{equation}
    
%     These methods quantify how holding out different features makes an individual prediction either higher or lower. For multi-class classification models, methods often use a single output that corresponds to the class of interest, and they can also apply a simple function to the model's output (for example, using the log-odds ratio rather than classification probability).
    
%     \item (Prediction loss) LossSHAP and CXPlain take into account the true label $y$ for an input $x$ and calculate the prediction loss using a loss function $\ell$:
    
%     \begin{equation}
%         v_{xy}(S) = - \ell\big(F(x_S), y\big). \label{eq:shap_loss_game}
%     \end{equation}
    
%     By incorporating label information, these methods quantify whether certain features make the prediction more or less correct. The minus sign is necessary to give the set function a higher value when more informative features are included.
    
%     \item (Prediction mean loss) L2X and INVASE consider the expected loss for a given input $x$ according to the label's conditional distribution $p(Y | X = x)$:
    
%     \begin{equation}
%         w_x(S) = - \E_{p(Y | X = x)}\Big[\ell\big(F(x_S), Y\big)\Big]. \label{eq:l2x_game}
%     \end{equation}
    
%     By averaging the loss across the label's distribution, these methods highlight features that correctly predict what \textit{could} have occurred, on average.
    
%     \item (Dataset loss w.r.t. label) Shapley Net Effects, SAGE, feature ablation (LOCO), permutation tests and univariate predictors consider the expected loss across the entire dataset:
    
%     \begin{equation}
%         v(S) = - \E_{XY}\Big[\ell\big(F(X_S), Y\big)\Big]. \label{eq:expected_loss_game}
%     \end{equation}
    
%     These methods quantify how much the model's performance degrades when different features are removed. This set function can also be viewed as the predictive power derived from sets of features~\citep{covert2020understanding}. Recent work has proposed a SHAP value aggregation scheme that can be considered a special case of this approach~\cite{frye2020shapley}.
    
%     \item (Dataset loss w.r.t. output) Shapley Effects considers the expected loss with respect to the full model output:
    
%     \begin{equation}
%         w(S) = - \E_X\Big[\ell\big(F(X_S), F(X)\big)\Big]. \label{eq:shapley_effects_game}
%     \end{equation}
    
%     Though related to the previous approach~\citep{covert2020understanding}, Shapley Effects focuses on each feature's influence on the model output rather than on the model performance.
% \end{itemize}

Each set function serves a distinct purpose in exposing a model's dependence on different features. The first three approaches listed above analyze the model's behavior for individual predictions (local explanations) while the last two take into account the model's behavior across the entire dataset (global explanations). Although their aims differ, these set functions are all in fact related. Each builds upon the previous ones by accounting for either the loss or data distribution, and their relationships can be summarized as follows:

\begin{align}
    v_{xy}(S) &= - \ell\big(u_x(S), y\big) \\
    w_x(S) &= - \ell\big( u_x(S), u_x(D) \big) \\
    v_x(S) &= \E_{p(Y \mid X = x)}\big[v_{xY}(S)\big] \\
    v(S) &= \E_{XY}\big[v_{XY}(S)\big] \label{eq:loss_shap_sage} \\
    w(S) &= \E_X\big[w_X(S)\big]
\end{align}

% \begin{align}
%     v_{xy}(S) &= \ell\big(v_x(S), y\big) \\
%     w_x(S) &= \E_{p(Y | X = x)}\big[v_{xY}(S)\big] \\
%     v(S) &= \E_{XY}\big[v_{XY}(S)\big] = \E_X\big[w_X(S)\big] \label{eq:loss_shap_sage} \\
%     w(S) &= \E_X\Big[\ell\big(v_X(S), v_X(D)\big)\Big]
% \end{align}

% In observing these set functions closely, it seems that a natural addition to the group would be a set functions that quantifies the sensitivity of a model's local behavior, similarly to $v_x$, but in a way that is agnostic to the direction of change. We denote this set function as $u_x$, and define it as:

% \begin{equation}
%     u_x(S) = \ell\big(F(x_S), f(x)\big).
% \end{equation}

% \noindent In contrast with measuring the impact on the model output, $u_x$ quantifies the proximity of the prediction to the model output with all features included, and it provides the benefit of accommodating multi-dimensional model outputs. To the authors' knowledge, no prior work has analyzed this set function, but it is connected to the other set functions through the following relationships:
% % This set function is related to the other set functions through the relationships below (Eqs.~\ref{eq:relationships1}-\ref{eq:relationships2}), but to the authors' knowledge, no prior work has analyzed this set function.

% \begin{align}
%     u_x(S) &= \ell\big(v_x(S), v_x(D)\big) \\
%     w(S) &= \E\big[u_X(S)\big]
% \end{align}

These relationships show that explanations based on one set function are in some cases related to explanations based on another. For example, Covert et al. showed that SAGE explanations are the expectation of explanations provided by LossSHAP~\cite{covert2020understanding}---a relationship reflected in Eq.~\ref{eq:loss_shap_sage}.

Understanding these connections is possible only because our framework disentangles each method's choices rather than viewing each method as a monolithic algorithm. We conclude by reiterating that removal-based explanations can explain virtually any function, and that choosing what to explain amounts to selecting a set function $u: \mathcal{P}(D) \mapsto \R$ to represent the model's dependence
% how the model depends
on different sets of features.
% We conclude by reiterating that the choice of what behavior a method explains amounts to the selection of a set function $u: \mathcal{P}(D) \mapsto \R$ that represents how the model depends on different subsets of features.


==> Explaining by Removing - MLRSA/6_explanations.tex <==
\section{Summarizing Feature Influence} \label{sec:explanations}

The third choice for removal-based explanations is how to summarize each feature's influence on the model. We examine the various summarization techniques and then discuss their computational complexity and approximation approaches.
% We examine summarization techniques used to generate explanations and then discuss their computational complexity and approximation approaches.

\subsection{Explaining set functions} \label{sec:summarization_strategies}

The set functions we used to represent a model's dependence on different features
% formulated
(Section~\ref{sec:behaviors}) are complicated mathematical objects that are difficult to communicate fully due to the exponential number of feature subsets and underlying feature interactions. Removal-based explanations confront this challenge by providing users with a concise summary of each feature's influence.

We distinguish between two main types of summarization approaches: feature attributions and feature selections. Many methods provide explanations in the form of \textit{feature attributions}, which are numerical scores $a_i\in \R$ given to each feature $i = 1, \ldots, d$. If we use $\mathcal{U}$ to denote the set of all functions $u: \mathcal{P}(D) \mapsto \R$, then we can represent feature attributions as mappings of the form $E: \mathcal{U} \mapsto \R^d$, which we refer to as \textit{explanation mappings}. Other methods take the alternative approach of summarizing set functions with a set $S^* \subseteq D$ of the most influential features. We represent these \textit{feature selection} summaries as explanation mappings of the form $E: \mathcal{U} \mapsto \mathcal{P}(D)$. Both approaches provide users with simple summaries of a feature's contribution to the set function.

We now consider the specific choices made by each method (see Appendix~\ref{app:methods} for further details). For simplicity, we let $u$ denote the set function each method analyzes. Surveying the various removal-based explanation methods, the techniques for summarizing each feature's influence include:

\begin{itemize}[leftmargin=2pc]
    \item (Remove individual) Occlusion, PredDiff, CXPlain, permutation tests and feature ablation (LOCO) calculate the impact of removing a single feature from the model, resulting in the following attribution values:
    
    \begin{equation}
        a_i= u(D) - u(D \setminus \{i\}). \label{eq:remove_individual}
    \end{equation}
    
    Occlusion, PredDiff and CXPlain can also be applied with groups of features, or superpixels, in image contexts.
    % Occlusion can also remove groups of pixels from images in a way that places each pixel in multiple groups. When the groups are denoted by $\mathcal{H} = \{H_1, H_2, \ldots, H_m\}$ and $\mathcal{H}_i = \{H \in \mathcal{H} : i \in H\}$ represents the groups that include feature $i$, Occlusion calculates the following attribution values:
    
    % \begin{equation*}
    %     a_i= u(D) - \frac{1}{|\mathcal{H}_i|} \sum_{H \in \mathcal{H}_i} u(D \setminus H).
    % \end{equation*}
    
    \item (Include individual) The univariate predictors approach calculates the impact of including individual features, resulting in the following attribution values:
    
    \begin{equation}
        a_i= u(\{i\}) - u(\{\}). \label{eq:include_individual}
    \end{equation}
    
    This is essentially the reverse of the previous approach: rather than removing individual features from the complete set, this approach adds individual features to the empty set.
    
    \item (Additive model) LIME fits a regularized additive model to a dataset of perturbed examples. In the limit of an infinite number of samples, this process approximates the following attribution values:
    
    \begin{equation}
        a_1, \ldots, a_d = \argmin_{b_0, \ldots, b_d} \; \sum_{S \subseteq D}\pi(S)\Big(b_0 + \sum_{i \in S} b_i - u(S)\Big)^2 + \Omega(b_1, \ldots, b_d). \label{eq:lime}
    \end{equation}
    
    In this problem, $\pi$ represents a weighting kernel and $\Omega$ is a regularization function that is often set to the $\ell_1$ penalty to encourage sparse attributions~\citep{tibshirani1996regression}. Since this summary is based on an additive model, the learned coefficients $(a_1, \ldots, a_d)$ represent the incremental value associated with including each feature.
    
    \item (Mean when included) RISE determines feature attributions by sampling many subsets $S \subseteq D$ and then calculating the mean value when a feature is included. Denoting the distribution of subsets as $p(S)$ and the conditional distribution as $p(S \mid i \in S)$, the attribution values are defined as
    
    \begin{equation}
        a_i= \E_{p(S \mid i \in S)}\big[u(S)\big].
    \end{equation}
    
    In practice, RISE samples the subsets $S \subseteq D$ by removing each feature $i$ independently with probability $p$, using $p = 0.5$ in their experiments~\citep{petsiuk2018rise}.
    % The paper mentions 0.5, but their code uses 0.1. Their implementation actually does not have a default value.
    
    \item (Shapley value) Shapley Net Effects, IME, Shapley Effects, QII, SHAP (including KernelSHAP, TreeSHAP and LossSHAP), SPVIM and SAGE all calculate feature attributions using the Shapley value, which we denote as $a_i = \phi_i(u)$.
    % Described in more detail in Section~\ref{sec:cooperative_game_theory}
    Shapley values are the only attributions that satisfy several desirable properties~\cite{shapley1953value}, and they are defined as follows:
    
    \begin{equation}
        \phi_i(v) = \frac{1}{d} \sum_{S \subseteq D \setminus \{i\}} \binom{d - 1}{|S|}^{-1} \Big( v(S \cup \{i\}) - v(S) \Big).
    \end{equation}
    
    \item (Low-value subset) MP selects a small set of features $S^*$ that can be removed to give the set function a low value. It does so by solving the following optimization problem:
    
    \begin{equation}
        S^* = \argmin_{S} \; u(D \setminus S) + \lambda |S|. \label{eq:mp_opt}
    \end{equation}
    
    In practice, MP incorporates additional regularizers and solves a relaxed version of this problem (see Section~\ref{sec:complexity}).
    
    \item (High-value subset) MIR solves an optimization problem to select a small set of features $S^*$ that alone can give the set function a high value. For a user-defined minimum value $t$, the problem is given by:

    \begin{equation}
        S^* = \argmin_S \; |S| \quad {\text s.t.} \;\; u(S) \geq t. \label{eq:mir_opt}
    \end{equation}
    
    L2X and EP solve a similar problem but switch the terms in the constraint and optimization objective. For a user-defined subset size $k$, the optimization problem is given by:
    
    \begin{equation}
        S^* = \argmax_S \; u(S) \quad \mathrm{s.t.} \;\; |S| = k. \label{eq:l2x_opt}
    \end{equation}
    
    Finally, INVASE, REAL-X and FIDO-CA solve a regularized version of the problem with a parameter $\lambda > 0$ controlling the trade-off between the subset value and subset size:
    
    \begin{equation}
        S^* = \argmax_S \; u(S) - \lambda |S|. \label{eq:invase_opt}
    \end{equation}
    
    \item (Partitioned subsets) MM solves an optimization problem to partition the features into $S^*$ and $D \setminus S^*$ while maximizing the difference in the set function's values. This approach is based on the idea that removing features to find a low-value subset (as in MP) and retaining features to get a high-value subset (as in MIR, L2X, EP, INVASE, REAL-X and FIDO-CA) are both reasonable approaches for identifying influential features. The problem is given by:
    
    \begin{equation}
        S^* = \argmax_S \; u(S) - \gamma u(D \setminus S) - \lambda |S|. \label{eq:mm_opt}
    \end{equation}
    
    In practice, MM also incorporates regularizers and monotonic link functions to enable a more flexible trade-off between $u(S)$ and $u(D \setminus S)$ (see Appendix~\ref{app:methods}).
\end{itemize}

% \begin{itemize}[leftmargin=2pc]
%     \item (Remove individual) Occlusion, PredDiff, CXPlain, permutation tests and feature ablation (LOCO) calculate the impact of removing a single feature from the set of all features, resulting in the following attribution values:
    
%     \begin{equation}
%         a_i= u(D) - u(D \setminus \{i\}). \label{eq:remove_individual}
%     \end{equation}
    
%     Occlusion, PredDiff and CXPlain can also be applied with groups of features in image contexts.
%     % Occlusion can also remove groups of pixels from images in a way that places each pixel in multiple groups. When the groups are denoted by $\mathcal{H} = \{H_1, H_2, \ldots, H_m\}$ and $\mathcal{H}_i = \{H \in \mathcal{H} : i \in H\}$ represents the groups that include feature $i$, Occlusion calculates the following attribution values:
    
%     % \begin{equation*}
%     %     a_i= u(D) - \frac{1}{|\mathcal{H}_i|} \sum_{H \in \mathcal{H}_i} u(D \setminus H).
%     % \end{equation*}
    
%     \item (Include individual) The univariate predictors approach calculates the impact of including individual features, resulting in the following attribution values:
    
%     \begin{equation}
%         a_i= u(\{i\}) - u(\{\}). \label{eq:include_individual}
%     \end{equation}
    
%     This is essentially the reverse of the previous approach: while that approach removes individual features from the complete set, this one adds individual features to the empty set.
    
%     \item (Linear model) LIME fits a regularized weighted linear model to a dataset of perturbed examples. In the limit of an infinitely large dataset, this process approximates the following attribution values:
    
%     \begin{equation}
%         a_1, \ldots, a_d = \argmin_{b_0, \ldots, b_d} \; \sum_{S \subseteq D}\pi(S)\Big(b_0 + \sum_{i \in S} b_i - u(S)\Big)^2 + \Omega(b_1, \ldots, b_d). \label{eq:lime}
%     \end{equation}
    
%     In this problem, $\pi$ represents a weighting kernel and $\Omega$ is a regularization function that is often set to the $\ell_1$ penalty to encourage sparse attributions~\cite{tibshirani1996regression}. Since this summary is based on an additive model, the learned coefficients $(a_1, \ldots, a_d)$ represent values associated with including each feature.
    
%     \item (Mean when included) RISE determines feature attributions by sampling many subsets $S \subseteq D$ and then calculating the mean value when a feature is included. Denoting the distribution of subsets as $p(S)$ and the conditional distribution as $p(S \; | \; i \in S)$, the attribution values are defined as
    
%     \begin{equation}
%         a_i= \E_{p(S | i \in S)}\big[u(S)\big].
%     \end{equation}
    
%     In practice, RISE samples the subsets $S \subseteq D$ by removing each feature $i$ independently with probability $p$, using $p = 0.5$ in the original experiments~\citep{petsiuk2018rise}.
%     % The paper mentions 0.5, but their code uses 0.1. Their implementation actually does not have a default value.
    
%     \item (Shapley value) Shapley Net Effects, IME, Shapley Effects, QII, SHAP (including KernelSHAP, TreeSHAP and LossSHAP) and SAGE all calculate feature attribution values using the Shapley value, which we denote as $a_i = \phi_i(u)$. Shapley values are the only attributions that satisfy a number of desirable properties~\citep{shapley1953value}.
%     % Described in more detail in Section~\ref{sec:cooperative_game_theory}, Shapley values are the only attributions that satisfy numerous desirable properties~\citep{shapley1953value}.
    
%     \item (Low-value subset) MP selects a small set of features $S^*$ that can be removed to give the set function a low value. It does so by solving the following optimization problem:
    
%     \begin{equation}
%         S^* = \argmin_{S} \; u(D \setminus S) + \lambda |S|. \label{eq:mp_opt}
%     \end{equation}
    
%     In practice, MP uses additional regularizers and solves a relaxed version of this problem (see Section~\ref{sec:complexity}).
    
%     \item (High-value subset) MIR solves an optimization problem to select a small set of features $S^*$ that alone can give the set function a high value. For a user-defined minimum value $t$, the problem is given by:

%     \begin{equation}
%         S^* = \argmin_S \; |S| \quad {\text s.t.} \;\; u(S) \geq t. \label{eq:mir_opt}
%     \end{equation}
    
%     % MIR solves this problem using a greedy optimization algorithm.
%     L2X and EP solve a similar problem but switch the terms in the constraint and optimization objective. For a user-defined subset size $k$, the optimization problem is given by:
    
%     \begin{equation}
%         S^* = \argmax_S \; u(S) \quad \mathrm{s.t.} \;\; |S| = k. \label{eq:l2x_opt}
%     \end{equation}
    
%     % L2X and EP use different approximations to make this problem tractable.
%     Finally, INVASE and FIDO-CA solve a regularized version of the problem with a parameter $\lambda > 0$ controlling the trade-off between the subset value and subset size:
    
%     \begin{equation}
%         S^* = \argmax_S \; u(S) - \lambda |S|. \label{eq:invase_opt}
%     \end{equation}
    
%     \item (Partitioned subsets) MM solves an optimization problem to partition the features into $S^*$ and $D \setminus S^*$ while maximizing the difference in the set function's values. This approach is based on the idea that removing features to find a low-value subset (as in MP) and retaining features to get a high-value subset (as in MIR, L2X, EP, INVASE and FIDO-CA)
%     % removing features to get a low value (as in MP) and retaining features to get a high value (as in MIR, L2X and EP)
%     are both reasonable approaches for identifying influential features. The problem is given by:
    
%     \begin{equation}
%         S^* = \argmax_S \; u(S) - \lambda u(D \setminus S) - \gamma |S|. \label{eq:mm_opt}
%     \end{equation}
    
%     In practice, MM incorporates regularizers and monotonic link functions to enable a more flexible trade-off between $u(S)$ and $u(D \setminus S)$ (see Appendix~\ref{app:methods}).
% \end{itemize}

As this discussion shows, every removal-based explanation generates summaries of each feature's influence on the underlying set function. In general, a model's dependencies are
% dependence on each feature is
too complex to communicate fully, so explanations must provide users with a concise summary instead. As noted, most methods we discuss generate feature attributions, but several others
% (MP, MIR, L2X, EP, MM, FIDO-CA, INVASE)
generate explanations by selecting the most important features. These feature selection explanations are essentially coarse attributions that assign binary importance rather than a real number.

Interestingly, if the high-value subset optimization problems solved by MIR, L2X, EP, INVASE and FIDO-CA were applied to the set function that represents the dataset loss (Eq.~\ref{eq:loss_shap_sage}), they would resemble conventional global feature selection~\citep{guyon2003introduction}. The problem in Eq.~\ref{eq:l2x_opt} determines the set of $k$ features with maximum predictive power, the problem in Eq.~\ref{eq:mir_opt} determines the smallest possible set of features that achieve the performance represented by $t$, and the problem in Eq.~\ref{eq:invase_opt} uses a parameter $\lambda$ to control the trade-off. Though not generally viewed as a model explanation approach, global feature selection serves an identical purpose of identifying highly predictive features.

We conclude by reiterating that the third dimension of our framework amounts to a choice of explanation mapping, which takes the form $E : \mathcal{U} \mapsto \R^d$ for feature attribution or $E: \mathcal{U} \mapsto \mathcal{P}(D)$ for feature selection. Our discussion so far has shown that removal-based explanations can be specified using three precise mathematical choices, as depicted in Figure~\ref{fig:framework}. These methods, which are often presented in ways that make their connections difficult to discern, are constructed in a remarkably similar fashion.
% The remainder of this paper addresses the relationships and trade-offs among these different choices, beginning by examining the computational complexity of each summarization approach.

\input{inserts/framework}

\subsection{Complexity and approximations} \label{sec:complexity}

Showing how certain explanation methods fit into our framework requires distinguishing between their implicit aims
% substance
% the substance of methods
and the approximations that make them practical. Our presentation of these methods deviates from the original papers, which often focus on details of a method's implementation. We now bridge the gap by describing these methods'
% significant
computational complexity and the approximations they use out of necessity.

The challenge with most summarization techniques described above is that they require calculating the underlying set function's value $u(S)$ for many subsets of features. In fact, without making any simplifying assumptions about the model or data distribution, several techniques must examine all $2^d$ subsets of features. This includes the Shapley value, RISE's summary technique and LIME's linear model. Finding exact solutions to several of the optimization problems (MP, MIR, MM, INVASE, FIDO-CA) also requires examining all subsets of features, and solving the constrained optimization problem (EP, L2X) for $k$ features requires examining $\binom{d}{k}$ subsets, or $2^d d^{-\frac{1}{2}}$ subsets in the worst case.\footnote{This can be seen by applying Stirling's approximation to $\binom{d}{d/2}$ as $d$ becomes large.}

The only approaches with lower computational complexity are those that remove individual features (Occlusion, PredDiff, CXPlain, permutation tests, feature ablation) or include individual features (univariate predictors). These require only one subset per feature, or $d$ total feature subsets.

Many summarization techniques have superpolynomial complexity in $d$, making them intractable for large numbers of features. However, these methods work in practice due to fast approximation approaches, and in some cases methods have even been devised to generate explanations in real-time. Strategies that yield fast approximations include:

\begin{itemize}[leftmargin=2pc]
    \item Attribution values that are the expectation of a random variable can be estimated by Monte Carlo approximation. IME~\citep{vstrumbelj2010efficient}, Shapley Effects~\citep{song2016shapley} and SAGE~\citep{covert2020understanding} use sampling strategies to approximate Shapley values, and RISE also estimates its attributions via sampling~\citep{petsiuk2018rise}.
    
    \item KernelSHAP, LIME and SPVIM are based on linear regression models fitted to datasets containing an exponential number of datapoints. In practice, these techniques fit models to smaller sampled datasets, which means optimizing an approximate version of their objective function~\citep{lundberg2017unified, covert2021improving}.
    
    \item TreeSHAP calculates Shapley values in polynomial time using a dynamic programming algorithm that exploits the structure of tree-based models. Similarly, L-Shapley and C-Shapley exploit the properties of models for structured data to provide fast Shapley value approximations~\citep{chen2018shapley}.
    
    \item Several of the feature selection methods (MP, L2X, REAL-X, EP, MM, FIDO-CA) solve continuous relaxations of their discrete optimization problems. While these optimization problems can be solved by representing the set of features $S \subseteq D$ as a mask $m \in \{0, 1\}^d$, these methods instead use a continuous mask variable of the form $m \in [0, 1]^d$. When these methods incorporate a penalty on the subset size $|S|$, they also sometimes use the convex relaxation $||m||_1$.
    
    \item One feature selection method (MIR) uses a greedy optimization algorithm. MIR determines a set of influential features $S \subseteq D$ by iteratively removing groups of features that do not reduce the predicted probability for the correct class.
    
    \item One feature attribution method (CXPlain) and several feature selection methods (L2X, INVASE, REAL-X, MM) generate real-time explanations by learning separate explainer models. CXPlain learns an explainer model using a dataset consisting of manually calculated explanations, which removes the need to iterate over each feature when generating new explanations. L2X learns a model that outputs a set of features (represented by a $k$-hot vector) and INVASE/REAL-X learn similar selector models that can output arbitrary numbers of features. Similarly, MM learns a model that outputs masks of the form $m \in [0, 1]^d$ for images. These techniques can be viewed as \textit{amortized} approaches because they learn models that perform the summarization step in a single forward pass.
\end{itemize}

In conclusion, many methods have developed approximations that enable efficient model explanation, despite sometimes using summarization techniques that are inherently intractable (e.g., Shapley values). Certain techniques are considerably faster than others (i.e., the amortized approaches), and some can trade off computational cost for approximation accuracy~\citep{vstrumbelj2010efficient, covert2021improving}, but they are all sufficiently fast to be used in practice.

We speculate, however, that more approaches will be made to run in real-time by learning separate explainer models, as in the MM, L2X, INVASE, CXPlain and REAL-X approaches~\citep{dabkowski2017real, chen2018learning, yoon2018invase, schwab2019cxplain, jethani2021have}. Besides these methods, others have been proposed that learn the explanation process either as a component of the original model~\citep{fan2017adversarial, taghanaki2019infomask} or as a separate model after training~\citep{schulz2020restricting}. Such approaches may be necessary to bypass the need for multiple model evaluations and make removal-based explanations as fast as gradient-based and propagation-based methods.
% \footnote{While this work was under review, Jethani et al.~\cite{jethani2021fastshap} introduced an amortized approach for real-time Shapley value estimation.}

% \begin{itemize}[leftmargin=2pc]
%     % \item When attribution values are the expectation of a random variable, they can be estimated using Monte Carlo approximation.
%     \item Attribution values that are the expectation of a random variable can be estimated using Monte Carlo approximations. IME~\citep{vstrumbelj2010efficient}, Shapley Effects~\citep{song2016shapley} and SAGE~\citep{covert2020understanding} use sampling strategies to approximate Shapley values, and RISE also estimates its attributions via sampling~\citep{petsiuk2018rise}.
    
%     \item KernelSHAP and LIME are both based on linear regression models fitted to datasets containing an exponential number of datapoints. In practice, these techniques fit models to smaller sampled datasets, which means optimizing an approximate version of their objective function.
    
%     \item TreeSHAP calculates Shapley values in polynomial time using a dynamic programming algorithm that exploits the structure of tree-based models. Similarly, L-Shapley and C-Shapley exploit the properties of models for structured data to provide fast Shapley value approximations~\citep{chen2018shapley}.
    
%     \item Several of the feature selection methods (MP, L2X, EP, MM, FIDO-CA) solve continuous relaxations of their discrete optimization problems. While these optimization problems could be solved by representing the set of features $S \subseteq D$ as a mask $m \in \{0, 1\}^d$, these methods instead use a mask variable of the form $m \in [0, 1]^d$. When these methods incorporate a penalty on the subset size $|S|$, they often use the convex relaxation $||m||_1$.
    
%     \item One feature selection method (MIR) uses a greedy optimization algorithm. MIR determines a set of influential features $S \subseteq D$ by iteratively removing groups of features that do not reduce the predicted probability for the correct class.
    
%     \item One feature attribution method (CXPlain) and three feature selection methods (L2X, INVASE, MM) generate real-time explanations by learning separate explainer models. CXPlain learns an explainer model using a dataset consisting of manually calculated explanations, which removes the need to iterate over each feature after training. L2X learns a model that outputs a set of features (represented by a $k$-hot vector) and INVASE learns a similar selector model that can output an arbitrary number of features; similarly, MM learns a model that outputs masks of the form $m \in [0, 1]^d$ for images. These techniques can be viewed as \textit{amortized optimization} approaches~\citep{shu2017amortized} because they learn models that output approximate solutions in a single forward pass (similar to amortized inference~\cite{kingma2013auto}).
% \end{itemize}

% In conclusion, many methods provide efficient explanations despite using summarization techniques that are inherently intractable. Each approximation significantly speeds up computation relative to a brute-force calculation, but we predict that more approaches could be made to run in real-time by learning explainer models, as in the MM, L2X, INVASE and CXPlain approaches~\citep{chen2018learning, dabkowski2017real, schwab2019cxplain, yoon2018invase}.


==> Explaining by Removing - MLRSA/7_discussion.tex <==
\section{Discussion} \label{sec:discussion}

In this work, we developed a unified framework that characterizes a significant portion of the model explanation literature (26 existing methods). Removal-based explanations have a great degree of flexibility, and we systematized their differences by showing that each method is specified by three precise mathematical choices:
% We began this work by observing that many explanation methods can be understood as simulating feature removal to quantify each feature's influence, and we developed a framework that unifies a significant portion of the model explanation literature. Our framework shows that removal-based explanations are specified by three precise mathematical choices:

\begin{enumerate}[leftmargin=2pc]
    \item \textbf{How the method removes features.} Each method specifies a subset function $F \in \mathfrak{F}$ to make predictions with subsets of features, often based on an existing model $f \in \mathcal{F}$.
    % remove features from an existing model $f \in \mathcal{F}$.
    
    \item \textbf{What model behavior the method analyzes.} Each method implicitly relies on a set function $u: \mathcal{P}(D) \mapsto \R$ to represent the model's dependence on different groups of features. The set function describes the model's behavior either for an individual prediction or across the entire dataset.

    \item \textbf{How the method summarizes each feature's influence.} Methods generate explanations that provide a concise summary of each feature's contribution to the set function $u \in \mathcal{U}$. Mappings of the form $E: \mathcal{U} \mapsto \R^d$ generate feature attribution explanations, and mappings of the form $E: \mathcal{U} \mapsto \mathcal{P}(D)$ generate feature selection explanations.
\end{enumerate}

The growing interest in black-box ML models has spurred a remarkable amount of model explanation research, and in the past decade we have seen a number of publications proposing innovative new methods. However, as the field has
% evolved and
matured we have also seen a growing number of unifying theories that reveal underlying similarities and implicit relationships~\cite{ancona2017towards, covert2020understanding, lundberg2017unified}. Our framework for removal-based explanations is perhaps the broadest unifying theory yet, and it bridges the gap between disparate parts of the explainability literature.

An improved understanding of the field presents new opportunities for both explainability users and researchers. For users, we hope that our framework will allow for more explicit reasoning about the trade-offs between available explanation tools.
The unique advantages of different methods are difficult to understand when they are viewed as monolithic algorithms, but disentangling their choices makes it simpler to reason about their strengths and weaknesses.

For researchers, our framework offers several promising directions for future work. We identify three key areas that can be explored to better understand the trade-offs between different removal-based explanations:

\begin{itemize}[leftmargin=2pc]
    \item Several of the methods characterized by our framework can be interpreted using ideas from information theory~\cite{chen2018learning, covert2020understanding}. We suspect that other methods can be understood with an information-theoretic perspective and that this may shed light on whether there are theoretically justified choices for each dimension of our framework.
    
    \item As we showed in Section~\ref{sec:behaviors}, every removal-based explanation is based on an underlying set function that represents the model's behavior. Set functions can be viewed as \textit{cooperative games}, and we suspect that methods besides those that use Shapley values~\cite{covert2020understanding, datta2016algorithmic, lundberg2017unified, owen2014sobol, vstrumbelj2009explaining} can be related to techniques from cooperative game theory.
    
    \item Finally, it is remarkable that so many researchers have developed, with some degree of independence, explanation methods based on the same feature removal principle. We speculate that cognitive psychology may shed light on why this represents a natural approach to explaining complex decision processes. This would be impactful for the field because, as recent work has pointed out, explainability research is surprisingly disconnected from the social sciences~\cite{miller2019explanation, miller2017explainable}.
\end{itemize}

In conclusion, as the field evolves and the number of removal-based explanations continues to grow, we hope that our framework can serve as a foundation upon which future research can build.


==> Explaining by Removing - MLRSA/inserts/brca_correlation.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\vskip -0.4in
\begin{center}
\centerline{\includegraphics[width=0.78\columnwidth]{images/brca_correlation.pdf}}

\vskip -0.8in

\centerline{\includegraphics[width=0.78\columnwidth]{images/brca_rank_correlation.pdf}}

\vskip -0.45in

\caption{Mean correlation (top) and Spearman rank correlation (bottom) between different explanation methods on the BRCA dataset.}
\label{fig:brca_correlation}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/brca_grid.tex <==
\begin{figure}%[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/brca_explanation_grid.pdf}
\caption{Grid of dataset loss explanations for the BRCA subtype classification. Each bar chart represents gene attribution values for a different explanation method. The vertical axis represents feature removal strategies, and the horizontal axis represents summary strategies.}
\label{fig:brca_grid}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/brca_selection.tex <==
\begin{figure}%[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/brca_multiple_selection.pdf}
\caption{Feature selection results when using the top genes identified by each explanation method. Each bar represents the average loss for models trained using 1-20 top genes (lower is better).}
\label{fig:brca_selection}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/census_correctness.tex <==
\begin{figure}[t]
% \vskip 0.2in
% \vskip -0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{images/census_correlation_correctness.pdf}}

\centerline{\includegraphics[width=\columnwidth]{images/census_mse_correctness.pdf}}

% \centerline{\includegraphics[width=\columnwidth]{images/census_correlation_correctness.pdf}}

\caption{Boxplots quantifying the similarity of census income explanations to comparable explanations generated using separate models (a proxy for using the true conditional distribution). The similarity metrics are correlation (top, higher is better) and MSE (bottom, lower is better).}
% , and they are calculated for 256 examples.}
\label{fig:census_correctness}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/census_correlation.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\vskip -0.4in
\begin{center}
\centerline{\includegraphics[width=0.78\columnwidth]{images/census_removal_similarity.pdf}}

\vskip -0.8in

\centerline{\includegraphics[width=0.78\columnwidth]{images/census_summary_similarity.pdf}}

\vskip -0.45in

\caption{Mean correlation between different explanation methods on the census income dataset.
% (blue represents positive correlation and red represents negative).
Methods are grouped by their feature removal approach (top) or summary approach (bottom).}
\label{fig:census_correlation}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/census_grid.tex <==
\begin{figure}%[t]
\vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/census_explanation_grid.pdf}
\caption{Grid of prediction explanations for a single example in the census income dataset. Each bar chart represents attribution values for a different explanation method. The vertical axis represents feature removal strategies, and the horizontal axis represents summary strategies.}
\label{fig:census_grid}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/common_jmlr.tex <==
%% Original, no check marks
% \begin{table}[t]
% \caption{Common combinations of choices in recent work.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccc}
% \toprule
% \textsc{Dimensions} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$v_x(S) = F(x_S)$ \\$E_i(v_x) = \phi_i(v_x)$} & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $v_{x}(S) = F(x_S)$} & Occlusion, LIME (images), MM, RISE\footnotemark[8] \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$w(S) = - \E\Big[\ell\big(F(X_S), Y\big)\Big]$ \\ $E_i(w) = w(D) - w(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO), permutation tests, \\conditional permutation tests} \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = f_S(x_S)$ \\ $w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$} & Univariate predictors, feature ablation (LOCO) \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$ \\ $E_i(w) = \phi_i(w)$} & SAGE, Shapley Net Effects \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$} & SAGE, conditional permutation tests \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(w) = \phi_i(w)$} & Shapley Net Effects, IME (2009) \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$v_{x}(S) = F(x_S)$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Occlusion, PredDiff \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Conditional permutation tests, PredDiff \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $v_{x}(S) = F(x_S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% %% Version 2, check marks, specific games
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{$v_x(S) = F(x_S)$ \\$E_i(v_x) = \phi_i(v_x)$} & \makecell{IME, QII, SHAP,\\KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $v_{x}(S) = F(x_S)$} & \makecell{Occlusion, LIME (images),\\MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{$v(S) = - \E\big[\ell\big(F(X_S), Y\big)\big]$ \\ $E_i(v) = v(D) - v(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO),\\permutation tests,\\cond. permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f_S(x_S)$ \\ $v(S) = - \E\big[\big(F(x_S), Y\big)\big]$} & \makecell{Univariate predictors,\\feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & \makecell{$v(S) = - \E\big[\big(F(x_S), Y\big)\big]$ \\ $E_i(v) = \phi_i(v)$} & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$v(S) = - \E\big[\big(F(x_S), Y\big)\big]$} & \makecell{SAGE,\\cond. permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(u) = \phi_i(u)$} & \makecell{Shapley Net Effects,\\IME (2009)} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & \makecell{$v_{x}(S) = F(x_S)$ \\ $E_i(v_x) = v_x(D) - v_x(D \setminus \{i\})$} & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Cond. permutation tests,\\PredDiff} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $v_{x}(S) = F(x_S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% Version 3, no specific games. This was a bad idea
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v_x(S)$ \\$E_i(u) = \phi_i(u)$} & \makecell{IME, QII, SHAP,\\KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $u(S) = v_{x}(S)$} & \makecell{Occlusion, LIME (images),\\MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v(S) = - \E\big[\ell\big(F(X_S), Y\big)\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO),\\permutation tests,\\cond. permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f_S(x_S)$ \\ $u(S) = v(S)$} & \makecell{Univariate predictors,\\feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v(S)$ \\ $E_i(u) = \phi_i(u)$} & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$u(S) = v(S)$} & \makecell{SAGE,\\cond. permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(u) = \phi_i(u)$} & \makecell{Shapley Net Effects,\\IME (2009)} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v_{x}(S)$ \\ $E_i(v_x) = v_x(D) - v_x(D \setminus \{i\})$} & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Cond. permutation tests,\\PredDiff} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $u(S) = v_{x}(S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% %% Version 4, no math notation
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{cccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{Occlusion, LIME (images), MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{Feature ablation (LOCO), permutation tests,\\conditional permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{Univariate predictors, feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{SAGE, conditional permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{Shapley Net Effects, IME (2009)} \\
% \midrule
% \cmark & & \cmark & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{Conditional permutation tests, PredDiff} \\
% \midrule
% \cmark & \cmark & & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

%% Version 5, cross marks
\begin{table}[t]
\caption{Common combinations of choices in existing methods. Check marks (\cmark) indicate choices that are identical between methods.}
\label{tab:common_combinations}
% \vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{cccc}
\toprule
\textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Methods} \\
\midrule
& \cmark & \cmark & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
\midrule
\cmark & & \cmark & \makecell{SHAP, LossSHAP, SAGE, Shapley Effects} \\
\midrule
\cmark & \cmark & & \makecell{Occlusion, LIME (images), MM, RISE} \\ % \footnotemark[2]} \\
\midrule
& \cmark & \cmark & \makecell{Feature ablation (LOCO), permutation tests,\\conditional permutation tests} \\
\midrule
\cmark & \cmark & & \makecell{Univariate predictors, feature ablation (LOCO),\\Shapley Net Effects, SPVIM} \\
\midrule
& \cmark & \cmark & SAGE, Shapley Net Effects, SPVIM \\
\midrule
\cmark & \cmark & & \makecell{SAGE, conditional permutation tests} \\
\midrule
\cmark & & \cmark & \makecell{Shapley Net Effects, SPVIM, IME (2009)} \\
\midrule
\cmark & & \cmark & Occlusion, CXPlain \\
\midrule
& \cmark & \cmark & Occlusion, PredDiff \\ % \footnotemark[3] \\
\midrule
\cmark & & \cmark & \makecell{Conditional permutation tests, PredDiff} \\
\midrule
\cmark & \cmark & & SHAP, PredDiff \\
\midrule
\cmark & \cmark & & MP, EP \\
\midrule
& \cmark & \cmark & EP, FIDO-CA \\
\midrule
\cmark & \cmark & \cmark & L2X, REAL-X\footnotemark[3] \\
\midrule
\cmark & \cmark & \cmark & Shapley Net Effects, SPVIM\footnotemark[4] \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

\footnotetext[3]{Although they share all three choices, L2X and REAL-X generate different explanations due to REAL-X's modified surrogate model training approach (Appendix~\ref{app:methods}).}
\addtocounter{footnote}{1}
\footnotetext[4]{SPVIM generalizes Shapley Net Effects to black-box models by using an efficient Shapley value estimation technique (Appendix~\ref{app:methods}).}
\addtocounter{footnote}{1}

==> Explaining by Removing - MLRSA/inserts/common_old.tex <==
%% Original, no check marks
% \begin{table}[t]
% \caption{Common combinations of choices in recent work.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccc}
% \toprule
% \textsc{Dimensions} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$v_x(S) = F(x_S)$ \\$E_i(v_x) = \phi_i(v_x)$} & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $v_{x}(S) = F(x_S)$} & Occlusion, LIME (images), MM, RISE\footnotemark[8] \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$w(S) = - \E\Big[\ell\big(F(X_S), Y\big)\Big]$ \\ $E_i(w) = w(D) - w(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO), permutation tests, \\conditional permutation tests} \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = f_S(x_S)$ \\ $w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$} & Univariate predictors, feature ablation (LOCO) \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$ \\ $E_i(w) = \phi_i(w)$} & SAGE, Shapley Net Effects \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$} & SAGE, conditional permutation tests \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(w) = \phi_i(w)$} & Shapley Net Effects, IME (2009) \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$v_{x}(S) = F(x_S)$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Occlusion, PredDiff \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Conditional permutation tests, PredDiff \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $v_{x}(S) = F(x_S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% %% Version 2, check marks, specific games
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{$v_x(S) = F(x_S)$ \\$E_i(v_x) = \phi_i(v_x)$} & \makecell{IME, QII, SHAP,\\KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $v_{x}(S) = F(x_S)$} & \makecell{Occlusion, LIME (images),\\MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{$v(S) = - \E\big[\ell\big(F(X_S), Y\big)\big]$ \\ $E_i(v) = v(D) - v(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO),\\permutation tests,\\cond. permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f_S(x_S)$ \\ $v(S) = - \E\big[\big(F(x_S), Y\big)\big]$} & \makecell{Univariate predictors,\\feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & \makecell{$v(S) = - \E\big[\big(F(x_S), Y\big)\big]$ \\ $E_i(v) = \phi_i(v)$} & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$v(S) = - \E\big[\big(F(x_S), Y\big)\big]$} & \makecell{SAGE,\\cond. permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(u) = \phi_i(u)$} & \makecell{Shapley Net Effects,\\IME (2009)} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & \makecell{$v_{x}(S) = F(x_S)$ \\ $E_i(v_x) = v_x(D) - v_x(D \setminus \{i\})$} & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Cond. permutation tests,\\PredDiff} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $v_{x}(S) = F(x_S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% Version 3, no specific games. This was a bad idea
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v_x(S)$ \\$E_i(u) = \phi_i(u)$} & \makecell{IME, QII, SHAP,\\KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $u(S) = v_{x}(S)$} & \makecell{Occlusion, LIME (images),\\MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v(S) = - \E\big[\ell\big(F(X_S), Y\big)\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO),\\permutation tests,\\cond. permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f_S(x_S)$ \\ $u(S) = v(S)$} & \makecell{Univariate predictors,\\feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v(S)$ \\ $E_i(u) = \phi_i(u)$} & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$u(S) = v(S)$} & \makecell{SAGE,\\cond. permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(u) = \phi_i(u)$} & \makecell{Shapley Net Effects,\\IME (2009)} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v_{x}(S)$ \\ $E_i(v_x) = v_x(D) - v_x(D \setminus \{i\})$} & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Cond. permutation tests,\\PredDiff} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $u(S) = v_{x}(S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% %% Version 4, no math notation
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{cccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{Occlusion, LIME (images), MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{Feature ablation (LOCO), permutation tests,\\conditional permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{Univariate predictors, feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{SAGE, conditional permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{Shapley Net Effects, IME (2009)} \\
% \midrule
% \cmark & & \cmark & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{Conditional permutation tests, PredDiff} \\
% \midrule
% \cmark & \cmark & & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

%% Version 5, cross marks
\begin{table}[t]
\caption{Common combinations of choices in existing methods. Check marks (\cmark) indicate choices that are identical between methods.}
\label{tab:common_combinations}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{tabular}{cccc}
\toprule
\textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Methods} \\
\midrule
& \cmark & \cmark & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
\midrule
\cmark & & \cmark & \makecell{SHAP, LossSHAP, SAGE, Shapley Effects} \\
\midrule
\cmark & \cmark & & \makecell{Occlusion, LIME (images), MM, RISE} \\ % \footnotemark[2]} \\
\midrule
& \cmark & \cmark & \makecell{Feature ablation (LOCO), permutation tests,\\conditional permutation tests} \\
\midrule
\cmark & \cmark & & \makecell{Univariate predictors, feature ablation (LOCO),\\Shapley Net Effects} \\
\midrule
& \cmark & \cmark & SAGE, Shapley Net Effects \\
\midrule
\cmark & \cmark & & \makecell{SAGE, conditional permutation tests} \\
\midrule
\cmark & & \cmark & \makecell{Shapley Net Effects, IME (2009)} \\
\midrule
\cmark & & \cmark & Occlusion, CXPlain \\
\midrule
& \cmark & \cmark & Occlusion, PredDiff \\ % \footnotemark[3] \\
\midrule
\cmark & & \cmark & \makecell{Conditional permutation tests, PredDiff} \\
\midrule
\cmark & \cmark & & SHAP, PredDiff \\
\midrule
\cmark & \cmark & & MP, EP \\
\midrule
& \cmark & \cmark & EP, FIDO-CA \\
\midrule
\cmark & \cmark & \cmark & L2X, INVASE \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% \footnotetext[2]{Setting removed features to zero is a special case of using default values.}
% \footnotetext[3]{PredDiff analyzes the log-odds ratio rather than the raw model output, but this is a minor difference.}
% \addtocounter{footnote}{2}

==> Explaining by Removing - MLRSA/inserts/concept.tex <==
\begin{figure*}[t]
\vskip 0.1in
\begin{center}
\includegraphics[width=\columnwidth]{images/concept.png}
\vskip 0.1in
\caption{A unified framework for \textit{removal-based explanations}. Each method is determined by three choices: how it removes features, what model behavior it analyzes, and how it summarizes feature influence.}
% \caption{Removal-based explanations quantify the impact of removing features from the model, and each method is specified by three choices: how it removes features, what model behavior it analyzes, and how it summarizes feature influence.}
\label{fig:concept}
\end{center}
\vskip -0.1in
\end{figure*}

==> Explaining by Removing - MLRSA/inserts/consistency.tex <==
\begin{table}[t]
\caption{Conventions for removing features may be consistent with the data distribution $p(X)$, consistent with another distribution $q(X) \neq p(X)$, or not consistent with any distribution.}
\label{tab:consistency}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{ccc}
\toprule
\textsc{Convention} & \textsc{Methods} & \textsc{Consistency} \\
\midrule
Marginalize (conditional) & \makecell{Cond. permutation tests, \\ PredDiff, SHAP, LossSHAP, \\SAGE, Shapley Effects} & Consistent with $p(X)$ \\
\midrule
Separate models & \makecell{Feature ablation (LOCO), \\univariate predictors, \\Shapley Net Effects, \\IME (2009)} & \multirow{3}{*}{\makecell{Consistent with $p(X)$\\ (assuming model optimality)}}\\
\cmidrule{1-2}
Missingness during training & L2X & \\
\midrule
Marginalize (marginals product) & QII & \multirow{2.5}{*}{\makecell{Consistent with a $q(X)$ that \\assumes feature independence}} \\
\cmidrule{1-2}
Marginalize (uniform) & IME (2010) & \\
\midrule
Zeros & \makecell{Occlusion, PredDiff \\ RISE, CXPlain} & \multirow{2.5}{*}{\makecell{Consistent with constant \\distributions $q(X)$}} \\
\cmidrule{1-2}
Default values & LIME (images), MM & \\
\midrule
Marginalize (marginal) & \makecell{Permutation tests, \\KernelSHAP, \\SAGE sampling} & \multirow{4}{*}{\makecell{Not consistent with \\any $q(X)$}}\\
\cmidrule{1-2}
Tree distribution & TreeSHAP & \\
\cmidrule{1-2}
Extend pixel values & MIR & \\
\midrule
Blurring & MP, EP & \multirow{2.5}{*}{Not valid $F \in \mathfrak{F}$}\\
\cmidrule{1-2}
Marginalize (replacement dist.) & LIME (tabular) & \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> Explaining by Removing - MLRSA/inserts/cooperative.tex <==
\begin{table}
\caption{Each method's summarization technique can each be understood in terms of concepts from cooperative game theory.}
\label{tab:cooperative}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{ccc}
\toprule
\textsc{Summarization} & \textsc{Methods} & \textsc{Related To} \\
\midrule
Shapley value & \makecell{Shapley Net Effects, IME, \\QII, SHAP (TreeSHAP, \\KernelSHAP, LossSHAP), \\Shapley Effects, SAGE} & \makecell{Shapley value, \\probabilistic values,\\modeling cooperative games} \\
\midrule
Mean value when included & RISE & \makecell{Banzhaf value, \\probabilistic values, \\modeling cooperative games} \\
\midrule
\makecell{Remove/include individual \\players} & \makecell{Occlusion, PredDiff, CXPlain, \\permutation tests,\\ univariate predictors, \\feature ablation (LOCO)} & \makecell{Probabilistic values, \\modeling cooperative games} \\
\midrule
Linear model & LIME & \makecell{Shapley value, Banzhaf value, \\modeling cooperative games} \\
\midrule
High/low value coalitions & MP, MIR, MM, L2X, EP & \makecell{Maximum/minimum excess} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> Explaining by Removing - MLRSA/inserts/framework.tex <==
\begin{figure*}[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/framework_color.png}
\vskip 0.1in
\caption{Removal-based explanations are specified by three precise mathematical choices: a subset function $F \in \mathfrak{F}$, a set function $u \in \mathcal{U}$, and an explanation mapping $E$ (for feature attribution or selection).}
\label{fig:framework}
\end{center}
% \vskip -0.2in
\end{figure*}

==> Explaining by Removing - MLRSA/inserts/genes.tex <==
\begin{table}[t]
\caption{List of genes analyzed.}
\label{tab:genes}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{cccccc}
\toprule
Genes 1-17 & Genes 18-34 & Genes 35-51 & Genes 52-68 & Genes 69-85 & Genes 86-100 \\
\midrule
OSTbeta & NBR2 & TSHR & HPS4 & GRINA & C20orf111 \\
STATH & CCDC64 & C7 & ZFPM1 & YTHDF3 & OMA1 \\
MAPK10 & NUP210 & CRYBB2 & OAS2 & TMCC1 & NCAPH2 \\
PLEKHG5 & HEMGN & PPAPDC3 & TUBA1C & UBE1DC1 & GPX2 \\
ERO1L & SLC25A3 & TXNL4B & OR8K5 & C6orf15 & BPY2C \\
ZNF711 & LEF1 & CHST9 & THSD3 & PDE6A & ZNF324 \\
ZNF385 & MVD & HACE1 & ATP6V0C & PEO1 & CDC27 \\
OR52E8 & OTUD3 & AYTL1 & RAB22A & TMEM52 & CCNB2 \\
SLC5A11 & KIAA1949 & PRSS35 & AP1B1 & PARP1 & CNOT7 \\
P4HA3 & SLC44A3 & ZNF408 & CTAGE6 & GSS & BIRC3 \\
LHFPL4 & ZNF775 & DDC & C6orf26 & RDH11 & GAL3ST3 \\
MGC33657 & THY1 & CSTL1 & ESR1 & STXBP1 & PLEKHM1 \\
CAPZB & DYNC1I2 & OR2F1 & UPK3B & ACLY & SPOCD1 \\
RBM15B & CYP1A1 & C12orf50 & ROBO4 & TMSB10 & PENK \\
C1orf176 & SPTA1 & SH3YL1 & TMEFF1 & TUBB & TAS2R9 \\
KLF3 & CLEC4M & SNUPN & KIAA1279 & LIPK & \\
OLFM4 & RXFP3 & COL25A1 & ZFP36L1 & HRC & \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> Explaining by Removing - MLRSA/inserts/information.tex <==
\begin{table}
\caption{Each method's underlying set function has an information-theoretic interpretation when features are removed appropriately.}
\label{tab:information}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{cccc}
\toprule
\textsc{Model Behavior} & \textsc{Set Function} & \textsc{Methods} & \textsc{Related To} \\
\midrule
Prediction & $v_x$ & \makecell{Occlusion, MIR, MM, \\IME, QII, LIME, MP, EP, \\SHAP, (KernelSHAP, \\TreeSHAP), RISE} & \makecell{Conditional probability, \\conditional expectation} \\
\midrule
Prediction loss & $v_{xy}$ & LossSHAP, CXPlain & \makecell{Pointwise mutual \\information} \\
\midrule
Prediction mean loss & $w_x$ & L2X & \makecell{KL divergence with \\conditional distribution} \\
\midrule
Dataset loss (label) & $v$ & \makecell{Permutation tests, \\univariate predictors, \\feature ablation (LOCO), \\Shapley Net Effects, SAGE} & \makecell{Mutual information \\(with label)} \\
\midrule
Dataset loss (output) & $w$ & Shapley Effects & \makecell{Mutual information \\(with output)} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}


==> Explaining by Removing - MLRSA/inserts/methods_grid.tex <==
\begin{figure*}[t]
\vskip -0.1in
\begin{center}
% \includegraphics[trim=1.35cm 0.2cm 5.5cm 0.6cm, clip=true, width=\textwidth]{images/methods_grid_large.pdf}
\includegraphics[trim=1.4cm 0.82cm 7.0cm 0.6cm, clip=true, width=\textwidth]{images/methods_grid_extended.pdf}
\vskip 0.1in
\caption{Visual depiction of the space of removal-based explanations.}
\label{fig:methods_grid}
\end{center}
\vskip -0.2in
\end{figure*}

==> Explaining by Removing - MLRSA/inserts/methods_grid_jmlr.tex <==
\begin{figure*}[t]
\vskip -0.2in
\begin{center}
% \includegraphics[trim=1.35cm 0.2cm 5.5cm 0.6cm, clip=true, width=\textwidth]{images/methods_grid_large.pdf}
% \includegraphics[trim=1.4cm 0.82cm 7.0cm 0.6cm, clip=true, width=\textwidth]{images/methods_grid_extended.pdf}
\includegraphics[trim=1.4cm 0cm 6.7cm 0cm, clip=true, width=\textwidth]{images/methods_grid_additive.pdf}
% \includegraphics[trim=1.4cm 0cm 6.7cm 0cm, clip=true, width=\textwidth]{images/methods_grid.pdf}
% \vskip -0.05in
\caption{Visual depiction of the space of removal-based explanations.}
\label{fig:methods_grid}
\end{center}
\vskip -0.2in
\end{figure*}

==> Explaining by Removing - MLRSA/inserts/mnist_examples.tex <==
\begin{figure}%[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/mnist_examples.pdf}
\caption{More MNIST prediction loss explanations using LossSHAP (feature removal with the conditional distribution and summary with the Shapley value).}
\label{fig:mnist_examples}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/mnist_grid.tex <==
\begin{figure}
% \vskip 0.2in
\vskip -0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/mnist_explanation_grid_digit.pdf}
\caption{Grid of prediction loss explanations for a single MNIST example. The vertical axis represents feature removal strategies and the horizontal axis represents summary strategies. Red pixels improve the loss, and blue ones hurt it (except for mean when included).}
\label{fig:mnist_grid}
\end{center}
\vskip -0.2in
\end{figure}

==> Explaining by Removing - MLRSA/inserts/table.tex <==
\begin{table}[t]
\caption{Choices made by existing removal-based explanations.}
\label{tab:methods}
\vskip -0.1in
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccc}
\toprule
\textsc{Method} & \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} \\
\midrule
IME (2009) & Separate models & Prediction & Shapley value \\
IME (2010) & Marginalize (uniform) & Prediction & Shapley value \\
QII & Marginalize (marginals product) & Prediction & Shapley value \\
SHAP & Marginalize (conditional/marginal) & Prediction & Shapley value \\
KernelSHAP & Marginalize (marginal) & Prediction & Shapley value \\
TreeSHAP & Tree distribution & Prediction & Shapley value \\
LossSHAP & Marginalize (conditional) & Prediction loss & Shapley value \\
SAGE & Marginalize (conditional) & Dataset loss (label) & Shapley value \\
Shapley Net Effects & Separate models & Dataset loss (label) & Shapley value \\
Shapley Effects & Marginalize (conditional) & Dataset loss (output) & Shapley value \\
Permutation Test & Marginalize (marginal) & Dataset loss (label) & Remove individual \\
Conditional Perm. Test & Marginalize (conditional) & Dataset loss (label) & Remove individual \\
Feature Ablation (LOCO) & Separate models & Dataset loss (label) & Remove individual \\
Univariate Predictors & Separate models & Dataset loss (label) & Include individual \\
L2X & Missingness during training & Prediction mean loss & High-value subset \\
INVASE & Missingness during training & Prediction mean loss & High-value subset \\
LIME (Images) & Default values & Prediction & Linear model \\
LIME (Tabular) & Marginalize (replacement dist.) & Prediction & Linear model \\
PredDiff & Marginalize (conditional) & Prediction & Remove individual \\
Occlusion & Zeros & Prediction & Remove individual \\
CXPlain & Zeros & Prediction loss & Remove individual \\
RISE & Zeros & Prediction & Mean when included \\
MM & Default values & Prediction & Partitioned subsets \\
MIR & Extend pixel values & Prediction & High-value subset \\
MP & Blurring & Prediction & Low-value subset \\
EP & Blurring & Prediction & High-value subset \\
FIDO-CA & Generative model & Prediction & High-value subset \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vskip -0.1in
\end{table}

==> Explaining by Removing - MLRSA/inserts/table_jmlr.tex <==
\begin{table}[t]
\caption{Choices made by existing removal-based explanations.}
\label{tab:methods}
% \vskip 0.2in
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccc}
\toprule
\textsc{Method} & \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} \\
\midrule
IME (2009) & Separate models & Prediction & Shapley value \\
IME (2010) & Marginalize (uniform) & Prediction & Shapley value \\
QII & Marginalize (marginals product) & Prediction & Shapley value \\
SHAP & Marginalize (conditional/marginal) & Prediction & Shapley value \\
KernelSHAP & Marginalize (marginal) & Prediction & Shapley value \\
TreeSHAP & Tree distribution & Prediction & Shapley value \\
LossSHAP & Marginalize (conditional) & Prediction loss & Shapley value \\
SAGE & Marginalize (conditional) & Dataset loss (label) & Shapley value \\
Shapley Net Effects & Separate models (linear) & Dataset loss (label) & Shapley value \\
SPVIM & Separate models & Dataset loss (label) & Shapley value \\
Shapley Effects & Marginalize (conditional) & Dataset loss (output) & Shapley value \\
Permutation Test & Marginalize (marginal) & Dataset loss (label) & Remove individual \\
Conditional Perm. Test & Marginalize (conditional) & Dataset loss (label) & Remove individual \\
Feature Ablation (LOCO) & Separate models & Dataset loss (label) & Remove individual \\
Univariate Predictors & Separate models & Dataset loss (label) & Include individual \\
L2X & Surrogate & Prediction loss (output) & High-value subset \\
REAL-X & Surrogate & Prediction loss (output) & High-value subset \\
INVASE & Missingness during training & Prediction mean loss & High-value subset \\
LIME (Images) & Default values & Prediction & Additive model \\
LIME (Tabular) & Marginalize (replacement dist.) & Prediction & Additive model \\
PredDiff & Marginalize (conditional) & Prediction & Remove individual \\
Occlusion & Zeros & Prediction & Remove individual \\
CXPlain & Zeros & Prediction loss & Remove individual \\
RISE & Zeros & Prediction & Mean when included \\
MM & Default values & Prediction & Partitioned subsets \\
MIR & Extend pixel values & Prediction & High-value subset \\
MP & Blurring & Prediction & Low-value subset \\
EP & Blurring & Prediction & High-value subset \\
FIDO-CA & Generative model & Prediction & High-value subset \\
% PMIM & Generative model & Prediction loss & Remove individual \\
% IGM & Generative model & ? & Remove individual
% MP2-G & Generative model & Prediction & Low-value subset
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vskip -0.2in
\end{table}

% \begin{table}[t]
% \caption{Choices made by existing removal-based explanations.}
% \label{tab:methods}
% \vskip 0.2in
% \begin{center}
% \begin{scriptsize}
% % \begin{tiny}
% \begin{tabular}{lccc}
% \toprule
% \textsc{Method} & \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} \\
% \midrule
% IME (2009) \citep{vstrumbelj2009explaining} & Separate models & Prediction & Shapley value \\
% \makecell[l]{IME (2010) \\ \citep{vstrumbelj2010efficient}} & Marginalize (uniform) & Prediction & Shapley value \\
% QII \citep{datta2016algorithmic} & Marginalize (marginals product) & Prediction & Shapley value \\
% SHAP \citep{lundberg2017unified} & Marginalize (conditional/marginal) & Prediction & Shapley value \\
% \makecell[l]{KernelSHAP \\ \citep{lundberg2017unified}} & Marginalize (marginal) & Prediction & Shapley value \\
% TreeSHAP \citep{lundberg2020local} & Tree distribution & Prediction & Shapley value \\
% \makecell[l]{LossSHAP \\ \citep{lundberg2020local}} & Marginalize (conditional) & Prediction loss & Shapley value \\
% \makecell[l]{SAGE \\ \citep{covert2020understanding}} & Marginalize (conditional) & Dataset loss (label) & Shapley value \\
% \makecell[l]{Shapley Net Effects \\ \citep{lipovetsky2001analysis}} & Separate models & Dataset loss (label) & Shapley value \\
% Shapley Effects \citep{owen2014sobol} & Marginalize (conditional) & Dataset loss (output) & Shapley value \\
% Permutation Test \citep{breiman2001random} & Marginalize (marginal) & Dataset loss (label) & Remove individual \\
% \makecell[l]{Conditional Perm. Test \\ \citep{strobl2008conditional}} & Marginalize (conditional) & Dataset loss (label) & Remove individual \\
% \makecell[l]{Feature Ablation (LOCO) \\ \citep{lei2018distribution}} & Separate models & Dataset loss (label) & Remove individual \\
% \makecell[l]{Univariate Predictors \\ \citep{guyon2003introduction}} & Separate models & Dataset loss (label) & Include individual \\
% L2X \cite{chen2018learning} & Missingness during training & Prediction mean loss & High-value subset \\
% INVASE \citep{yoon2018invase} & Missingness during training & Prediction mean loss & High-value subset \\
% \makecell[l]{LIME (Images) \\ \citep{ribeiro2016should}} & Default values & Prediction & Linear model \\
% \makecell[l]{LIME (Tabular) \\ \citep{ribeiro2016should}} & Marginalize (replacement dist.) & Prediction & Linear model \\
% PredDiff \citep{zintgraf2017visualizing} & Marginalize (conditional) & Prediction & Remove individual \\
% Occlusion \citep{zeiler2014visualizing} & Zeros & Prediction & Remove individual \\
% CXPlain \citep{schwab2019cxplain} & Zeros & Prediction loss & Remove individual \\
% RISE \citep{petsiuk2018rise} & Zeros & Prediction & Mean when included \\
% MM \citep{dabkowski2017real} & Default values & Prediction & Partitioned subsets \\
% MIR \citep{zhou2014object} & Extend pixel values & Prediction & High-value subset \\
% MP \citep{fong2017interpretable} & Blurring & Prediction & Low-value subset \\
% EP \citep{fong2019understanding} & Blurring & Prediction & High-value subset \\
% FIDO-CA \citep{chang2018explaining} & Generative model & Prediction & High-value subset \\
% % PMIM & Generative model & Prediction loss & Remove individual \\
% % IGM & Generative model & ? & Remove individual
% % MP2-G & Generative model & Prediction & Low-value subset
% \bottomrule
% \end{tabular}
% \end{scriptsize}
% % \end{tiny}
% \end{center}
% \vskip -0.2in
% \end{table}

==> Explaining by Removing - MLRSA/inserts/tradeoff.tex <==
\begin{figure*}[t]
\vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/tradeoff.png}
\caption{Each model explanation strategy represents a trade-off between an explanation's simplicity and its completeness.}
\label{fig:tradeoff}
\end{center}
\vskip -0.2in
\end{figure*}

==> Explaining by Removing - MLRSA/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Explaining by Removing - MLRSA/old/census_summary_correlation.tex <==
\begin{figure*}[h!]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.5\columnwidth]{images/census_summary_similarity.pdf}
\caption{Blah}
\label{fig:census_summary_correlation}
\end{center}
\vskip -0.2in
\end{figure*}

==> Explaining by Removing - MLRSA/old/methods_grid_table.tex <==
% \begin{table}[t]
% \caption{Systematization of existing methods.}
% \label{tab:methods_grid}
% \vskip 0.2in
% \begin{center}
% \begin{tiny}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% & \makecell{Remove \\Individual} & \makecell{Include\\Individual} & \makecell{Mean When\\Included} & \makecell{Shapley\\Value} & \makecell{Linear\\Model} & \makecell{High\\Value\\Subset} & \makecell{Low\\Value\\Subset} & \makecell{Partitioned\\Subsets} \\
% \hline
% \makecell{Zeros} & \makecell{Occlusion\\CXPlain} && RISE &&&&& \\
% \hline
% \makecell{Default\\Values} & & & & & \makecell{LIME\\(images)} & & & MM \\
% \hline
% \makecell{Extend\\pixels} &&&&&& MIR && \\
% \hline
% \makecell{Blurring} & \makecell{{}\\{}} &&&&& EP & MP & \\
% \hline
% \makecell{Marginalize\\(replacement\\dist.)} &&&&& \makecell{LIME\\(tabular)} &&& \\
% \hline
% \makecell{Marginalize\\(uniform)} &&&& IME (2010) &&&&\\
% \hline
% \makecell{Marginalize\\(marginals\\product)} &&&& QII &&&& \\
% \hline
% \makecell{Marginalize\\(marginal)} & \makecell{Permutation\\test} &&& \makecell{KernelSHAP,\\SHAP,\\SAGE Sampling} &&&& \\
% \hline
% \makecell{Marginalize\\(conditional)} & \makecell{PredDiff,\\cond. perm.\\test} &&& \makecell{SHAP,\\LossSHAP,\\SAGE,\\Shapley Effects} &&&& \\
% \hline
% \makecell{Tree\\distribution} &&&& TreeSHAP &&&& \\
% \hline
% \makecell{Missingness\\during\\training} &&&&&& L2X && \\
% \hline
% \makecell{Separate\\models} & \makecell{Feature\\ablation} & \makecell{Univariate\\predictors} && \makecell{IME (2009),\\Shapley Net Effects} &&&& \\
% \hline
% \end{tabular}
% \end{tiny}
% \end{center}
% \vskip -0.2in
% \end{table}

% % Version 2, no midrules/hlines
% \begin{table}[t]
% \caption{Systematization of existing methods.}
% \label{tab:methods_grid}
% \vskip 0.2in
% \begin{center}
% \begin{tiny}
% \begin{tabular}{ccccccccc}
% \toprule
% & \makecell{Remove \\Individual} & \makecell{Include\\Individual} & \makecell{Mean When\\Included} & \makecell{Shapley\\Value} & \makecell{Linear\\Model} & \makecell{High\\Value\\Subset} & \makecell{Low\\Value\\Subset} & \makecell{Partitioned\\Subsets} \\
% \midrule
% % \cmidrule(lr){2-9}
% \makecell{Zeros} & \makecell{Occlusion\\CXPlain} & \makecell{{}\\{}\\{}} & RISE &&&&& \\
% %\midrule
% \makecell{Default\\Values} & \makecell{{}\\{}\\{}} & & & & \makecell{LIME\\(images)} & & & MM \\
% %\midrule
% \makecell{Extend\\pixels} & \makecell{{}\\{}\\{}}&&&&& MIR && \\
% %\midrule
% \makecell{Blurring} & \makecell{{}\\{}} &&&&& EP & MP & \\
% %\midrule
% \makecell{Marginalize\\(replacement\\dist.)} &&&&& \makecell{LIME\\(tabular)} &&& \\
% %\midrule
% \makecell{Marginalize\\(uniform)} & \makecell{{}\\{}\\{}} &&& IME (2010) &&&&\\
% %\midrule
% \makecell{Marginalize\\(marginals\\product)} &&&& QII &&&& \\
% %\midrule
% \makecell{Marginalize\\(marginal)} & \makecell{Permutation\\test} & \makecell{{}\\{}\\{}\\{}} && \makecell{KernelSHAP,\\SHAP,\\SAGE Sampling} &&&& \\
% %\midrule
% \makecell{Marginalize\\(conditional)} & \makecell{PredDiff,\\cond. perm.\\test} & \makecell{{}\\{}\\{}\\{}\\{}} && \makecell{SHAP,\\LossSHAP,\\SAGE,\\Shapley Effects} &&&& \\
% %\midrule
% \makecell{Tree\\distribution} & \makecell{{}\\{}\\{}} &&& TreeSHAP &&&& \\
% %\midrule
% \makecell{Missingness\\during\\training} & \makecell{{}\\{}\\{}} &&&&& L2X && \\
% %\midrule
% \makecell{Separate\\models} & \makecell{Feature\\ablation} & \makecell{Univariate\\predictors} & \makecell{{}\\{}\\{}} & \makecell{IME (2009),\\Shapley Net Effects} &&&& \\
% \bottomrule
% \end{tabular}
% \end{tiny}
% \end{center}
% \vskip -0.2in
% \end{table}

% Version 3, colors
\begin{table}[t]
\caption{Systematization of existing methods.}
\label{tab:methods_grid}
\vskip 0.2in
\begin{center}
\begin{tiny}
\begin{tabular}{ccccccccc}
% \toprule
& \makecell{Remove \\Individual} & \makecell{Include\\Individual} & \makecell{Mean When\\Included} & \makecell{Shapley\\Value} & \makecell{Linear\\Model} & \makecell{High\\Value\\Subset} & \makecell{Low\\Value\\Subset} & \makecell{Partitioned\\Subsets} \\
% \midrule
% \cmidrule(lr){2-9}
\makecell{Zeros} & \makecell{\pred{Occlusion},\\\predloss{CXPlain}} & \makecell{{}\\{}\\{}} & \pred{RISE} &&&&& \\
%\midrule
\makecell{Default\\Values} & \makecell{{}\\{}\\{}} & & & & \makecell{\pred{LIME}\\\pred{(images)}} & & & \pred{MM} \\
%\midrule
\makecell{Extend\\pixels} & \makecell{{}\\{}\\{}}&&&&& \pred{MIR} && \\
%\midrule
\makecell{Blurring} & \makecell{{}\\{}} &&&&& \pred{EP} & \pred{MP} & \\
%\midrule
\makecell{Marginalize\\(replacement\\dist.)} & \makecell{{}\\{}\\{}\\{}} &&&& \makecell{\pred{LIME}\\\pred{(tabular)}} &&& \\
%\midrule
\makecell{Marginalize\\(uniform)} & \makecell{{}\\{}\\{}} &&& \pred{IME (2010)} &&&&\\
%\midrule
\makecell{Marginalize\\(marginals\\product)} & \makecell{{}\\{}\\{}\\{}} &&& \pred{QII} &&&& \\
%\midrule
\makecell{Marginalize\\(marginal)} & \makecell{\datasetloss{Permutation}\\\datasetloss{test}} & \makecell{{}\\{}\\{}\\{}} && \makecell{\pred{KernelSHAP},\\\pred{SHAP},\\\datasetloss{SAGE Sampling}} &&&& \\
%\midrule
\makecell{Marginalize\\(conditional)} & \makecell{\pred{PredDiff},\\\datasetloss{cond. perm.}\\\datasetloss{test}} & \makecell{{}\\{}\\{}\\{}\\{}} && \makecell{\pred{SHAP},\\\predloss{LossSHAP},\\\datasetloss{SAGE},\\\datasetmodelloss{Shapley Effects}} &&&& \\
%\midrule
\makecell{Tree\\distribution} & \makecell{{}\\{}\\{}} &&& \pred{TreeSHAP} &&&& \\
%\midrule
\makecell{Missingness\\during\\training} & \makecell{{}\\{}\\{}\\{}} &&&&& \predmeanloss{L2X} && \\
%\midrule
\makecell{Separate\\models} & \makecell{\datasetloss{Feature}\\\datasetloss{ablation}} & \makecell{\datasetloss{Univariate}\\\datasetloss{predictors}} & \makecell{{}\\{}\\{}} & \makecell{\pred{IME (2009)},\\\datasetloss{Shapley Net Effects}} &&&& \\
% \bottomrule
\end{tabular}
\end{tiny}
\end{center}
\vskip -0.2in
\end{table}

% \pred{$\blacksquare$ Prediction}

% \predloss{$\blacksquare$ Prediction Loss}

% \predmeanloss{$\blacksquare$ Prediction Mean Loss}

% \datasetloss{$\blacksquare$ Dataset Loss}

% \datasetmodelloss{$\blacksquare$ Dataset Loss (Output)}

==> Explaining by Removing - MLRSA/old/psychology_1.tex <==
\section{The Psychology of Learning by Ignoring} \label{sec:psychology}

Most model explanation methods are not derived from relevant research in psychology or philosophy \citep{miller2017explainable}. Here, we show that the methods discussed so far nonetheless have parallels with established ideas about how explanations should be formed for humans. We illuminate links with the social sciences by pointing to influential works whose proposals are consistent with methods in the learning by ignoring paradigm.

% Model explanation is implicitly a question about the causes for a model behaving in a particular way.
% % (We emphasize that it is not about potential causal relationships between the model input and the response variable).
% Even the question ``why does the model predict $y$'' is ambiguous, however; in a view that is representative of the literature on this topic, \cite{hilton1990conversational} claims that events are not explained per se, but that \textit{why} questions have either an implicit or explicit \textit{rather than} built in. \cite{lipton1990contrastive} refers to the alternative scenario as a \textit{foil}, and \cite{miller2019explanation} suggests that specific foils could be elicited from human observers in the context of machine learning interpretability.

% Methods in the learning by ignoring paradigm involve no human interaction, so they assume a certain behavior to be explained, as well as the corresponding foil. \textcolor{red}{TODO not sure what the foil is. It sounds stupid to say, why y instead of not y, because as Miller points out, that requires an explanation of the full chain of causality. This is not a fruitful perspective.}

% \textcolor{red}{The fact-foil perspective about unambiguous questions from Hilton, Van blah blah and Lipton is NOT useful. We do not elicit fact-foil pairs, and proposing implicit fact-foils pairs could sort of be done by looking at summarization methods; but the result won't be convincing, because the explanations provided are not perfect answers to those questions. Ultimately, suggesting the implicit questions being answered does not seem like a valuable endeavor.}

% Model explanation is implicitly a causality question about why a model behaves in a particular way.
% the causes for a model behaving in a particular way.
% (We emphasize that it is not about potential causal relationships between the model input and the response variable).
% For example, the underlying question may be about why the model makes a certain prediction, or why its cross entropy loss is a certain value.
% Such open ended questions are called \textit{plain fact} questions \citep{van2002remote}, and are generally thought to be more difficult to answer then more detailed why questions with built in alternative scenarios, or \textit{foils}, such as \textit{why A and not B?} \citep{hilton1990conversational, lipton1990contrastive, miller2019explanation}. Most model explanation methods, including those in the learning by ignoring paradigm, neglect to elicit particular foils from users, but we can consider whether they implicitly assume one.
% Such open ended questions are called \textit{plain fact} questions \citep{van2002remote}, which are generally more difficult to answer than why questions with specific alternative scenarios (foils) \citep{hilton1990conversational, lipton1990contrastive, miller2019explanation}.
% Rather than explaining these events relative to a particular alternative \cite{hilton1990conversational}, methods in the learning by ignoring paradigm answer so-called plain fact questions, which are generally more difficult to answer \cite{lipton1990contrastive}.
% \textcolor{red}{TODO are we sure that none of these methods have implicit foils? MP for example says why probability is high rather than low, and gives simple explanation with few causes.}

% For methods in the learning by ignoring paradigm, there is no single foil that is implicitly considered by all methods. Our approach is to consider individual methods, and given the explanations that are provided, point out the specific questions that these methods answer accurately. By providing an additive credit allocation, methods that use the Shapley value to provide explanations implicitly answer the question \textit{why was the set function equal to $u(D)$ rather than $u(\{\})$?} By finding sets of high-valued players, the optimization based methods implicitly answer the question \textit{why was the set function $u(D)$ large rather than small?}

% We cannot make a general claim about the foils that are considered by our class of explanation methods. What we can do is carefully consider an individual method, and given the explanation that it provides, point out what specific questions they answer. For example, SHAP answers the question \textit{why does the model predict $f(x)$, rather than $\E[f(X)]$?} And MP answers the question \textit{why did class $y$ seem probable rather than improbable?}

Model explanation is implicitly a \textit{causality} question about why a model behaves in a particular way.
% (We emphasize that it is not about potential causal relationships between the model input and the response variable).
For example, the underlying question may be about why the model makes a certain prediction, or why its cross entropy loss is a certain value. The subject of causality has attracted much work in the social sciences. \textcolor{red}{TODO should I be mentioning Pearl here?} There are a breadth of views in the literature, but many perspectives are based on the concept of counterfactual logic, where causation is determined by the impact of changing some facts on the outcome \citep{hume2000enquiry, mill1884system}. In the psychology literature, researchers have observed that people are able to mentally undo events by generating counterfactual scenarios \citep{tversky1982simulation}. \cite{wachter2017counterfactual} suggests that carefully chosen counterfactuals provide sufficient explanations for black box models. Methods in the learning by ignoring paradigm are built on counterfactual logic, albeit in a more subtle way.

Making predictions for different inputs is equivalent to a counterfactual, which may or may not change the outcome \citep{wachter2017counterfactual}. All of the conventions described for making predictions in the absence of features are in fact counterfactuals. In particular, the convention of marginalizing out missing features is highly similar to the mental model described by Norm Theory, in which a set of relevant exemplars is evoked, matching on certain immutable attributes but possibly varying on the mutable attributes \citep{kahneman1986norm}; the summary statistics from the evoked set are used to define a norm, or make a prediction in the absence of information.
% Alternatively, we can view the idea of making predictions with a subset of features as a counterfactual, where instead of prescribing alternative values, we prescribe ignorance of the values.

Individual counterfactuals are therefore the atoms of these explanation methods, rather than their final product. This is similar to the view of \cite{merrick2019explanation}, who define a counterfactual reference distribution to explain the large number of references used in Shapley-value based methods.

When it comes to providing explanations, the methods take different approaches. The methods that identify a set of important features provide simple explanations with few causes, which tend to be preferred by humans \citep{hilton1990conversational, miller2019explanation}. However, identifying a small number of causes without quantifying their impact is misleading, and could play into cognitive biases towards oversimplification \citep{}. By contrast, feature attribution methods consider every feature as a candidate cause, and distinguish between the different degrees of causality.

% Most machine learning explanation methods are not derived from relevant research in psychology, philosophy, or the cognitive sciences \citep{miller2017explainable}. We show that despite the apparent disconnect between these areas of research, methods in the learning by ignoring paradigm are consistent with influential ideas from the social sciences about how humans form explanations.

% Model explanation is implicitly a question of \textit{causality}, about what caused the model to make certain predictions. We emphasize that the causal question is not about potential causal relationships between the input and the response variable. 

% In a broad review of social science research that relates to machine learning interpretability, \cite{miller2019explanation} points out that most explanation methods are not derived from existing research in philosophy, psychology, or cognitive sciences. Although the methods in the learning by ignoring paradigm were not conceived with the explicit intention of building on social science research, we show that they can be understood in the context of existing ideas about how humans form explanations.

% I'm struggling with the decision to center this section around findings from social science papers, or to center it on learning by ignoring and bring things up as necessary.

% \begin{enumerate}
%     \item Contrastive explanations (fact and foil). Understanding how a model makes predictions is an ambiguous question, but Hilton says well founded questions are about why P happened rather then Q. Each method here implicitly assumes a fact based on their underlying set function (the prediction, the loss, etc.). The foil is not specific, but it why didn't some other value occur? Maybe clearer for additive methods.
%     \item Validity of counterfactual thinking for understanding causation (in this case, cause for specific model behavior) can be traced back to John Stuart Mill's method of difference. 
%     \item Counterfactual reasoning about causes. Kahneman and other citations in Asylum paper point out that people understand causality by undoing effects by mental simulation. Wachter cites lots of work to show that counterfactuals provide the best way of understanding models (need to read more closely). In machine learning, counterfactuals are represented by different inputs, and possibly different outputs. In learning by ignoring, a wide variety of counterfactuals are considered, like an evoked set, and their summary statistics summarized. Taly also likes counterfactual thinking, and talks about a counterfactual reference distribution. We do something similar, consider many counterfactuals.
%     \item Explanations are preferred to be simple and selected. The selection-based methods provide selections, which should be easier to understand. The attribution methods are less appealing because they're complicated, but more mathematically principled because they consider that everything is a cause to some degree.
% \end{enumerate}

% --

% --

% --

% --

% --

% Ideas:

% \begin{enumerate}
%     \item Kahneman has his thing about mentally undoing: explaining events by finding counterfactuals that are not too different, but change the outcome. Specific definition of not too different, because part of what's interesting is what people like to undo.
%     \item Think I've heard that people like counterfactuals in general. Ignoring a feature is a counterfactual, and its analogous to asking a doctor what would you think if I hadn't shown you this? Can distinguish between changing input to a specific value, and ignoring the value.
%     \item If you accept that ignoring information is like a counterfactual, then the set functions we describe represent $2^d$ possible counterfactuals, and the explanation methods summarize this information in a concise way. The attribution methods generally condense the information into scores for each feature. The optimization-based methods identify single insightful counterfactuals.
%     \item There's a tradeoff between summarizing all the counterfactuals in a way that provides as much information as possible (while satisfying good properties), and communicating something that's easy to understand (here are the most important features). Humans are bad at processing a lot of information, so there's something appealing about a simple explanation, even if is less informative than something complicated.
%     \item On the subject of ignoring features, worth talking about how humans would ignore features. Two doctors that make the same diagnoses in the presence of all information may differ when some information is missing, just like we can have two EPFs $F, G$ that satisfy $F(x, D) = G(x, D)$. Which one would you rather do the ignoring exercise with, someone who is consistent when information is held out, or something else? You learn more when they're consistent. But there's probably some logical fallacy that says people are bad at the mental simulation required to take into account the missing features' conditional distributions.
%     \item Although simple counterfactuals might be easier to understand, the lesson of the Shapley value is that giving a maximally representative summary is more complicated. People might like simplicily, but it probably plays into their inherent selection bias (or explanation bias, or hindsight bias), and makes them think that events are entirely due to the selected features and the others don't matter at all. The Shapley value tries to give an explanation that is more faithful to the full truth.
%     \item The simulation heuristic paper says that there are tasks of judgement where people seem to rely on simulating scenarios. Norm Theory proposes a mental model for how people define their norms: by recruiting recalled and constructed representations, and aggregating summary statistics. When constructing representations, there are certain mutable and certain immutable features. Parallel with how we use sets of information to evoke set of other representations, whose summary statistics are gathered, to give predictions in absence of some information. Summarizing many counterfactuals.
%     \item Although assigning specific attribute values can be seen as a counterfactual, can also see missing some information as a counterfactual. Shapley value aggregates that kind of information. 
%     \item Probably some named concept for how this would be too much computation for a person to actually perform.
%     \item There's a lot of work on psychology of causality attribution...
%     \item Maybe some papers that outright say people like to think in counterfactuals.
%     \item We have the choice of saying that predictions made in the absence of some information are made using the simulation heuristic, by aggregating information from a bunch of counterfactuals. Also have the choice of saying that a prediction in the absence of information is itself a counterfactual, and we can combine many of those. For the latter, more like evoking a category.
%     \item I want to make the point that counterfactuals are the atoms of explanations. Whereas Wachter paper thinks that counterfactuals and explanations are distinct. They advocate for using a wide variety of counterfactuals by leveraging domain knowledge and the needs of the recipient of the explanation, but we just combine a lot of them in a reasonable way, that does not take into account the recipient's objective. Holy SHIT, that was a 2017 paper! Simple, early-ish. Not so mad that they didn't see that counterfactuals are atoms and explanations are molecules. Their message is that counterfactuals are sufficient (or even exceed requirements), but there is also a message that you should provide multiple counterfactuals, and account for domain knowledge. We work with multiple counterfactuals, but also provide a default behavior for summarizing them.
%     \item Anything useful to say about Taly paper? They talk about a counterfactual reference distribution. Cite Norm Theory to justify working with counterfactuals to establish norms.
%     \item Big picture, my message here will be that even though these methods were not conceived with the explicit intention of matching up with social science research about how people tend to explain/understand things, it turns out they jive pretty well.
%     \item Hilton suggests that all explanations are contrastive, and that to give a good explanation, you require a fact and a foil. Do we implicitly have a foil in these cases? I think the foil is implicit in the set function.
% \end{enumerate}

==> Explaining by Removing - MLRSA/old/psychology_2.tex <==
\section{The Psychology of Explaining by Ignoring} \label{sec:psychology}

% In this section, we show that the explaining by ignoring framework has a compelling justification in terms of psychological theories about how humans explain events.
% Model explanation methods are not generally designed based on ideas from the social sciences, including psychology, philosophy, or cognitive sciences \citep{miller2017explainable}.
% In this section, we show that the explaining by ignoring framework has clear parallels with psychological theories about how humans explain the causes of events.
% It is rare for model explanation methods to be designed with psychology or philosophy research in mind \citep{miller2017explainable}, but since explanations are ultimately used by humans, it is important to make sure that methods build on the vast amount of social science research dedicated to the topic of explanation \citep{miller2019explanation}. Here, we show that methods in the explaining by ignoring framework have clear links with theories for how humans explain the causes of events.
Model explanation methods are not typically designed based on research in the social sciences, including psychology or philosophy \citep{miller2017explainable}. However, we are able to identify clear parallels between the explaining by ignoring paradigm and cognitive theories of how people understand the causes of events.

\subsection{Counterfactual Reasoning about Causality}

% Model explanation methods are not generally designed based on ideas from social science research, including psychology, philosophy, or cognitive sciences \citep{miller2017explainable, miller2019explanation}. 
% % The methods discussed in this work are not exceptions to this rule, but
% Perhaps surprisingly, we find that the methods discussed here have clear parallels with theories for how humans explain the causes of events. In particular, we show that the explaining by ignoring framework can be understood in terms of counterfactual reasoning. the simulation heuristic \citep{tversky1982simulation}, and Norm Theory \citep{kahneman1986norm}. \textcolor{red}{TODO could try to make a stronger statement.}
% has a compelling justification through its reliance on simulating a distribution of counterfactuals, and presenting explanations that rely on their summary statistics.
% based on counterfactual reasoning, and that explanations are provided by summarizing the results from a distribution of counterfactuals.
% Prior work has encouraged the incorporation of social science findings into explanation methods \cite{miller2019explanation}, and while we support such efforts, we find that explanation methods designed by computer scientists have remarkable parallels with how humans form explanations.

Explaining a model's predictions is fundamentally a causality question: the question is, \textit{why does the model behave this way?} Each input feature is a candidate cause, multiple features may be causal, and the role of an explanation is to quantify each feature's degree of causality. We emphasize that this is distinct from reasoning about causal relationships between the inputs and the response variable, because such relationships cannot be inferred from observational data \citep{pearl2009causality}.

Within the philosophy and psychology literature, \textit{counterfactual reasoning} is one of the dominant tools for understanding causality. A counterfactual example changes certain facts of a situation (e.g., the route a person drove to get home) to potentially achieve a different outcome (e.g., avoiding a car crash), and counterfactuals can shed light on whether each aspect of a situation caused the actual outcome (e.g., a car crash). In an influential philosophical account of causality, John Stuart Mill presents his five methods of induction that use counterfactual thinking to explain cause-effect relationships \citep{mill1884system, mackie1974cement}. And in the psychology literature, counterfactual thinking is the basis of multiple theories about how people explain events \citep{tversky1982simulation, hilton1990conversational}.

Relying on counterfactuals is a natural idea in the context of model explanation. Machine learning models are functions on high dimensional domains, so to understand a model is to understand how it maps different inputs to different outputs. Some work has embraced counterfactual reasoning by suggesting that model predictions should be explained by presenting users with a small number of counterfactual examples \citep{wachter2017counterfactual}.

% In their work that draws on analytic philosophy,
In their work, \cite{wachter2017counterfactual} suggest generating the closest possible counterfactual that achieves a user-specified alternative outcome. But while a single counterfactual can suggest a direction for changing one's outcome or contesting an adverse decision, individual counterfactuals provide insufficient information for understanding each feature's influence on the model. For example, if there are multiple causes for an outcome (e.g., a person's loan application was approved because of a good credit score and a high income level), and the outcome can be changed by reversing any single cause, the closest possible counterfactual may arbitrarily highlight one cause over another (e.g., by showing that a lower credit score would have led to the loan being rejected). It may take a large number of counterfactuals to represent the inner workings of a complex model.

In order to provide a more faithful representation of each feature's influence on the model, we show that rather than directly presenting counterfactuals to users, methods in the explaining by ignoring provide explanations that summarize outcomes from a large number of counterfactuals.

\subsection{Summarizing Counterfactuals}

I'm not sure this is the right section title. And I'm not sure the previous section covers what I need it to. Here's the new direction I want to take.

Everyone thinks you should use counterfactual reasoning to think about causality. That sure makes sense in the context of model explanation, because models are just functions.

How do I work this in... every method wo

A particularly relevant area of psychology research is the study of ``mentally undoing,'' which is about identifying the facts that people blame most for causing events. As an example, one study told people a story about a person who got in a car crash and asked them to imagine what the family would say if they said ``if only...'' The participants came up with counterfactuals that might occur to the people in the story, which effectively identify the causes. For example, many people blamed the unusual way the driver entered the intersection, or the unusual route the man drove (aspects that were emphasized in the story). 

% Given an input $x \in \mathcal{X}$ and the outcome $f(x)$, a counterfactual example may indicate that the feature $X_i$ causes the model output if it shows that changing $X_i$ changes the output. For example, showing that a fifty point reduction to a customer's credit score leads to their loan application being rejected suggests that their credit score is one of the causes for their application being accepted originally.

% Methods in the explaining by ignoring framework do not perform searches to find values that change the output. But by ignoring a feature $X_i = x_i$ or a group of features $X_{\bar S} = x_{\bar S}$, these methods consider the outcomes that arise with alternative values. Each method's approach for removing features uses counterfactuals, either by setting the removed features to specific alternative values, or by integrating over a distribution of alternative values (Section~\ref{sec:missingness_strategies}). We focus here on approaches that marginalize out missing features, because these have a more compelling justification in the psychology literature. In particular, we focus the approach that marginalizes out features with their conditional distribution.

% When $X_{\bar S}$ is ignored, we effectively simulate counterfactual values from the distribution $p(X_{\bar S} \; | \; X_S)$ and record the mean model output from these counterfactuals. A similar process for generating counterfactuals and recording their summary statistics is described by the cognitive model in Norm Theory \citep{kahneman1986norm}. In this work, the authors describe a process wherein a probe (e.g., the input $x$) evokes a set of recalled and simulated alternatives (e.g., counterfactual examples) whose summary statistics define a person's perspective of normal outcomes. SHAP's connections with Norm Theory have been recognized in prior work, which refers to the distribution of alternative values as a \textit{counterfactual reference distribution} \citep{merrick2019explanation}.
% on normal behavior for the phenomenon in question.
% For example, a ``normal'' outcome for a loan application may be considered by recalling acquaintances who applied for loans, or articles about the process, as well as imagining potential applicants and their outcomes. 
% The authors refer to \textit{mutable} and \textit{immutable} features to distinguish between the features that may diverge from the probe, and the features that must remain constant in the counterfactual alternatives.

% In our case, it is as if the probe $x$ evokes a set of counterfactuals, which are constrained to retain certain immutable features $X_S = x_S$, but which may diverge in the mutable features $X_{\bar S}$. And the mutable features for our set of counterfactuals are drawn from a specific distribution $p(X_{\bar S} \; | \; X_S = x_S)$; in Norm Theory, the authors suggest that the primary factors controlling the weight of stimuli in a norm are the strength of the connection (or the similarity) with the probe, and factors affecting the memorability of the stimulus in a person's mind. 

\textcolor{red}{Should maybe give up on finding clear parallels. Norm Theory isn't so specific, or if it is, I don't understand it clearly. Paint a broader picture of what Norm Theory and study of mentally undoing have to say.}

\begin{enumerate}
    \item Counterfactual reasoning about causality: model explanation is a causality question, and lots of people say that causality questions should be addressed using counterfactual reasoning. Some people in ML have embraced that idea by saying that model explanations should just be counterfactuals.
    \item Summarizing counterfactuals: explaining by ignoring means considering counterfactual inputs, because features are removed by setting them to alternative values or integrating over a distribution of alternative values. For the approaches that marginalize out removed features, it is as if the average behavior if defined by integrating over a counterfactual reference distribution (Taly).
    \item Connections with Norm Theory and simulation heuristic: Kahneman and Tversy, and later Kahneman and Miller, developed two related theories for cognitive processes that relate to explaining the causes of events that are relevant to this framework of model explanation methods. In Norm Theory, Kahneman suggests that people follow a cognitive process where they define normal behavior by gathering summary statistics from a set of recalled and simulated representations.
\end{enumerate}

\textcolor{red}{TODO write this from scratch}

\begin{enumerate}
    % \item Like most explanation methods, these were not designed with human psychology research in mind (Miller). But the designers were reasonable people, so maybe that's not necessary. We find clear links with theories about how humans explain the causes of events.
    % \item Explaining a model's behavior is fundamentally a causality question: what made the model behave this way? Emphasize that we're not talking about causal relationships with response variable, which cannot be inferred from observational data (Pearl)
    % \item Everyone agrees that counterfactual reasoning is the most important tool for understanding causality (Hume, Mill, Hilton, etc). Counterfactuals simply change some aspects of the situation, in order to possibly change the outcome. Wachter understands counterfactuals in the context of machine learning as simply evaluating the model with different inputs. Indeed, it seems natural that to understand a model, which is just a function, we must understand how it behaves given different inputs.
    % \item However, it is not obvious which counterfactual examples to present. Wachter suggested presenting several, and Miller suggested soliciting user preference for what kind of different outcomes the user wants to see achieved. We argue that methods that following the explaining by ignoring framework provide explanations that summarize a large number of counterfactual examples, rather than presenting a small number of counterfactuals directly (Wachter).
    \item Begin by observing that when features are ignored, each approach provides counterfactual values for the missing features (Section 3). Some approaches prescribe a single set of values, while others integrate over a distribution of possible values. When integrating across the counterfactual distribution, these approaches consider the different outcomes (model outputs) that might be achieved in proportion to their likelihood. This idea is very similar to Taly's idea of a counterfactual reference distribution, which, as they noted, is reminiscent of Norm Theory (Kahneman).
    \item Feel like I had more to say about Kahneman than Taly did. Don't want to end the section by saying they had the right idea!
    \item It is easy to identify links with psychology research about how people explain the causes of events. Certain conventions for ignoring features are more justified, so we focus our attention on the approach of marginalizing out missing features with their conditional distribution.
    \item Simulation heuristic suggested that people perform certain tasks of judgement by mentally simulating potential outcomes. In the context of mentally undoing events (identifying their causes), people were able to imagine alternative (counterfactual) realities in which different outcomes were achieved. One of the points of the study was to identify people's preferences when generating counterfactual situations. One of the most important findings was that people prefer downhill changes---substituting unlikely inputs for more likely alternatives (a person driving on their regular route, rather than an unusual one).
    \item People's preference for downhill changes suggests that they are sensitive to a measure of events' likelihood. Rather than identifying an event as causal because it has one high likelihood alternative value that changes the outcome, we might consider a distribution of alternative values, and consider the different outcomes in proportion to their likelihood.
    \item Wanted to work in mutable, immutable features.
\end{enumerate}

==> Explaining by Removing - MLRSA/old/psychology_3.tex <==
\section{The Psychology of Removal-Based Explanations} \label{sec:psychology}

Model explanation methods are not typically designed based on research from the social sciences, including either psychology or philosophy \citep{miller2017explainable}. However, we are able to identify clear parallels between removal-based explanations and cognitive theories about how people understand the causes of events. We begin by discussing the role of counterfactual reasoning in our framework, and we then discuss a trade-off between simple explanations and explanations that convey more information about the model.

\subsection{Counterfactual reasoning about causality}

Explaining a model's predictions is fundamentally a causality question: the question is, \textit{why does the model behave this way?} Each input feature is a candidate cause, multiple features may be causal, and the role of an explanation is to quantify each feature's degree of influence on the model. We emphasize that this is distinct from reasoning about causal relationships in the data (e.g., whether smoking causes cancer), because these relationships are difficult to infer from observational data \citep{pearl2009causality}.

Within the philosophy and psychology literature, \textit{counterfactual reasoning} is one of the dominant tools for understanding causality. A counterfactual example changes certain facts of a situation (e.g., the route a person drove to get home) to potentially achieve a different outcome (e.g., avoiding a car crash), and counterfactuals can shed light on whether each aspect of a situation caused the actual outcome (e.g., a fatal car crash). In an influential philosophical account of causality, John Stuart Mill presents his five methods of induction that use counterfactual thinking to explain cause-effect relationships \citep{mill1884system, mackie1974cement}. In the psychology literature, counterfactual thinking is the basis of multiple theories about how people explain events \citep{tversky1982simulation, hilton1990conversational}.

In a well-known empirical study, \cite{tversky1982simulation} examined the process of \textit{mental undoing}, or imagining counterfactuals to change an event's outcome. The authors theorized that to mentally undo an event, people would identify facts of the story that could be changed in order to mentally simulate a different outcome occurring. The authors then observed people's tendencies by designing a survey in which participants were told a story about an event that occurred, a man who got in a car crash, and were then asked to suggest the causes to which the family attributed the accident.

Depending on the version of the story that the participants were told, they were found to be more likely to point to different aspects of the story, such as the route the man drove, or the unusual way in which he entered the intersection where the crash happened. The clearest finding from their study was the \textit{downhill rule}, which says that people mentally undo events by removing unlikely occurrences. As the authors explain, ``a downhill change is one that removes a surprising or unexpected aspect of the story, or otherwise increases its internal coherence'' \citep{tversky1982simulation}.

The downhill rule suggests that people will assign blame to an attribute if it is easy to imagine a counterfactual situation where that attribute is changed, and the outcome is different. In the next section, we show how model explanation techniques build on this idea through their particular use of counterfactual reasoning. 

\subsection{Counterfactuals for model explanation}

Relying on counterfactuals is a natural idea in the context of model explanation. Machine learning models are functions on high dimensional domains, so to understand a model is to understand how it maps different inputs to different outputs. And any method that generates explanations by perturbing the input, whether it is by removing features or not, is based on some form of counterfactual reasoning.

Some work has embraced counterfactual reasoning by suggesting that model predictions should be explained by presenting users with a small number of counterfactual examples \citep{wachter2017counterfactual}. The authors suggest generating the nearest possible counterfactual that achieves a user-specified alternative outcome, which is reminiscent of the downhill rule \citep{tversky1982simulation}. In this approach, proximity is used as a placeholder for internal coherence when identifying counterfactual changes that can alter the outcome.

However, while a single counterfactual can suggest a direction for changing an outcome or for contesting an adverse decision, individual counterfactuals provide insufficient information for understanding each feature's influence on the model. For example, if there are multiple causes for an outcome (e.g., a person's loan application was approved because of a good credit score and a high income level), and the outcome can be changed by reversing any single cause, then the closest possible counterfactual may arbitrarily highlight one cause over another (e.g., by showing that a lower credit score would have led to the loan being rejected). The problem is that many counterfactuals may be required to understand a complex model.

When assessing whether a feature influences the model, the downhill rule suggests that we should determine whether the feature has a high likelihood alternative value that changes the model output. In the framework of removal-based explanations, methods do not perform a search over alternative values; but by \textit{removing} the feature, they integrate the model output over a distribution of alternative values (or in some cases, by setting the feature to a default value). The justification for this, in light of the downhill rule, is that if there are high likelihood values that change the model output, this influence will become apparent when integrating over the distribution.

Of particular note is the approach that marginalizes out missing features using the conditional distribution (the focus of Section~\ref{sec:information}). In this approach, counterfactuals are considered in proportion to their internal coherence, which is represented by the likelihood under the data distribution $p(X_{\bar S} \; | \; X_S) \propto p(X)$. This approach to removing features has a clear correspondence with the downhill rule observed by \cite{tversky1982simulation}.

The framework of removal-based explanations is based on summarizing the results of many counterfactuals, while, by contrast, the approach from \cite{wachter2017counterfactual} presents individual counterfactuals directly to users. When assessing the impact of removing a particular set of features, each set of counterfactuals varies from the original input in only those features, and their values are drawn from a distribution that ideally relates to the internal coherence of those different values.

A similar observation was made by \cite{merrick2019explanation}, who remarked that the process of summarizing many counterfactuals resembles the cognitive process described by Norm Theory \citep{kahneman1986norm}. In this cognitive theory, people are said to gather summary statistics from a mentally constructed set of recalled and simulated representations of a phenomena, such as loan application outcomes for people with a given age and income. Norm Theory provides a cognitive analogue to the process of making predictions while certain features are removed.

In summary, we have identified two well-known cognitive theories that provide a basis for the framework of removal-based explanations---the theory of mentally undoing \citep{tversky1982simulation} and Norm Theory \citep{kahneman1986norm}. We emphasize that these theories do not prescribe a precise approach to model explanation; rather, they provide reassurance that certain existing approaches have some degree of correspondence with how humans are thought to understand causality.
% We also emphasize that these theories relate to the idea of removing features, which is the first choice in our framework, but that they do not relate to what model behaviors should be analyzed (the second dimension), or how concise explanations should be generated (the third dimension).

\subsection{Simplicity versus completeness}

When generating explanations, there is a trade-off between the amount of information conveyed and the user's likelihood of drawing the right conclusions. An explanation that paints an incomplete picture may prove to be more useful, if the user can understand it better.

% For example,
On one end of the spectrum, an individual counterfactual is easy to process, but it may not convey much insight about how a model works \citep{wachter2017counterfactual}. By contrast, SHAP's feature attributions provide a more complex summary of each feature's impact on the model,
% represent a more complex explanation that summarizes each feature's impact on the model,
% SHAP is among the more complex explanation methods,
% and although SHAP is among the most widely used interpretability tools \citep{bhatt2020explainable},
but a recent user study showed that even savvy users were less likely to understand SHAP visualizations, and experienced a higher cognitive load than users who viewed explanations for simpler generalized additive models \citep{kaur2020interpreting}. Similarly, another user study found that longer explanations required more time and effort to understand, and in some cases impeded users' ability to draw appropriate conclusions \citep{lage2019human}.

We refer to this as the trade-off between simplicity and completeness, because explanations are typically more complex when they provide a more complete picture of the model. For the purpose of helping the user build a mental model of the machine learning model, or to be able to mentally simulate the model \citep{lipton2018mythos}, providing a more complete picture seems preferable. But complicated explanations will leave users cognitively overloaded, possibly leaving them with a false sense of understanding of the model, and may even leave them worse off.

Recognizing this trade-off and its implications for the utility of explanations motivates the consideration of simplicity as a design principle. Within our framework, we have the flexibility to strike a balance between completeness and simplicity. To avoid cognitively overloading users, one might focus on global explanations rather than local explanations. One approach is to provide visualizations that aggregate the results of many local explanations, such as global SHAP plots \citep{lundberg2020local}. Alternatively, we might focus on providing global explanations that represent the model's behavior across the entire dataset, such as SAGE or Shapley Effects \citep{covert2020understanding, owen2014sobol}.

Certain formats of explanations convey more information than others. Feature attributions provide a granular view of the model by citing every feature as a cause and quantifying each feature's influence. However, psychology research has shown that people report higher satisfaction with explanations that cite fewer causes \citep{thagard1989explanatory, read1993explanatory, lombrozo2007simplicity, miller2019explanation}. Users may therefore derive more insight from explanation that highlight fewer causes, such as the sparse feature attributions that LIME can provide \cite{ribeiro2016should}.

The feature selection explanations go even further in the direction of simplicity. These explanations cite fewer causes because they directly penalize the number of selected features (Section~\ref{sec:summarization_strategies}). Furthermore, they omit information about the granularity of each feature's influence. For a non-technical user, it may be preferable to communicate that a model's prediction was dominated by a small number of features; it may take a more sophisticated user to absorb each feature's numerical contribution, and to internalize the interpretation of each attribution value as an additive decomposition of the model's behavior with subsets of features (Section~\ref{sec:linear_models}).

Designers of explanation methods must be wary of overestimating people's abilities to store complex mental models \citep{norman1983some}, and the community can be mindful of this by tailoring explanations to the user's degree of sophistication. Savvy users may benefit from getting a more complete picture of the model, but non-technical users may get more out of explanations that convey less information.

% Script
% Simplicity is an important design principle, because if people don't understand an explanation, they won't draw the right conclusions.
% There's a tradeoff between providing a more complete picture of the model and a user digesting the information properly.
% Within our framework (but also among other methods), we have the ability to provide more or less information in an explanation.
% For more savvy users, we might provide more information (attribution). For less savvy users, we might provide less information.
% In both cases, our objective is to help people build mental models of the model (simulatibility). 

% User studies have not found the sources of people's confusion, but we speculate that it could arise from the complex algorithms that estimate SHAP values, from the amount of information conveyed in a feature attribution, or from the visualizations (force plots).
% We speculate that several factors contribute to a user's ability to understand an explanation method: the complexity of the algorithm that generates the explanation, of the explanation itself, and of the explanation's presentation.
% For our framework, the two sources of complexity that are most important to discuss are the complexity of the algorithm that generates the explanation, and the complexity of the explanation itself.

% For people to understand explanations and draw the right conclusions, they should ideally have an understanding of the process that generated the explanation. 

% Users should also have an understanding of the meaning of the explanation itself, independently of the algorithm that generated it. The methods discussed in this work produce only two kinds of explanations: feature attributions, and selections of the most important features.

% -

% Kaur: people don't understand SHAP as well as simpler methods, and it causes them to fail to answer questions based on visualizations, and leaves them with high cognitive load. Poursabzi and Lage also document problems with cognitive overload arising from model explanations.

% Bhatt: people rely on SHAP more than anything else.

% Lombrozo and Co.: people are more satisfied with explanations that cite few causes.

% Lipton: one thing that people should get from interpretability methods is ability to simulate a model. Relates to simulation heuristic (Kahneman), and also to mental models (Norman).

% Attributions help people simulate the model given subsets of features, by quantifying impact of including a feature. Selections say that the selected features on their own achieve roughly the same prediction.

% When people have a poor mental model of how an explanation is generated (e.g. Shapley values), possibly because the process is genuinely complicated, they will have a harder time drawing appropriate conclusions.

% -----From Kaur-----
% Kaur shows that ML practitioners can't explain how SHAP works. They report lower confidence, and they perform worse at answering questions based on it
% Poursabzi-Sangdeh finds that too much transparency into a model causes information overload and makes people follow a model even when it makes a mistake
% Lage finds that longer explanations overload people's cognitive abilities
% Lombrozo (and Miller) propose three criteria: simplicity, generality, and coherence. However, I don't yet know what they mean by generality and coherence in ML context!
% Their user studies show that people have lower confidence, less accurate answers to simple questions, and higher cognitive load with SHAP
% Norman (from HCI) suggests that it's important to have mental and conceptual model of a tool. If the tool is really complicated, it would be hard to have an accurate mental model

% -----From Bhatt-----
% More people use SHAP than anything else

% -----From Lipton-----
% Authors of interpretability papers have different ideas of what interpretability means, different goals
% What people might want from interpretability is an ability to simulate a model. Like forming a mental model of...the model

% -----From Lombrozo-----
% People prefer explanations that cite fewer propositions ("simpler" explanations). They appear to have a prior belief that there should be few causes
% People's preference for explanations was measured through "satisfaction," which is vague. Imagine that it has something to do with belief that the explanation (a speculation) is true
% There's competition between explanations with few causes and explanations whose causes are likely. People like both "simplicity" and probability
% Read paper, and another paper, both tried to get at simplicity and/or probability. They both bungled it. Serious confounding, and bad methodology
% Theory is that people place their prior belief on small number of causes. Possibly because they believe the world to be simple? 

% -----From Read-----
% People like simple explanations (fewer causes)
% Authors findings support Thagard's model (not just his principles)

% -----From Thagard-----
% Has a theory about principles that are relevant to acceptance of hypotheses about causes. Turns these principles into a model
% One aspect of the theory is the prediction that smaller sets of causes will be preferred. He did not test this, but multiple psychology papers took him up on it

% -----From Spellman 1996-----
% Intuitive scientists (like intuitive stasisticians)
% An existing normative rule for how people evaluate the influence of something is difference between probability of outcome with that treatment, and without it
% It had been observed that in instances with multiple causes, people do not use that rule. One theory was that people might conditionalize their influence estimation on some fixed causes
% Experiments provided evidence that this is true

% -----From Spellman 2001-----
% Same shit about how people conditionalize to evaluate influence. But who could advocate for not conditioning? Marginalizing gives a summary that is, in the best case, not misleading

% -----From Norman-----
% People have conceptions that they bring to any task. People form mental models of themselves and of the things they interact with. Mental models provide predictive and explanatory power over interactions
% Target system; conceptual model of target system; mental model of target system; scientist's conception of the mental model
% Conceptual models are invented by teachers, designers and engineers
% Mental models evolve naturally through interaction. They are usually not technically accurate, but ought to be "functional" (successfully predict aspects of interactions?). This is in line with Lipton's idea of simulatability
% Scientist's conceptualization is model of the mental model
% Lots of observations about people's mental models. One is that people's ability to run them is severely limited
% People have superstitions, maintain behavior that does not make sense but seems to work. Worried about fragility. Reduce mental effort but increase usage effort
% He's really talking about interaction with devices and maybe software. Will need to pick out ideas that are relevant to me
% There is often difference between conceptual model (model of how one should interact) and mental model (which governs how one interacts)
% The purpose of a mental model is to help a person understand and anticipate behavior of a system during an interaction. Would be helpful for someone to be able to run their model mentally
% I wonder what Norman has to say about design principles, and how it relates to someone's ability to form an accurate mental model
% For designer, goal is to design around a conceptual model that the user can replicate in their mental model. It should not be too complicated for them to learn. "it is our duty to develop conceptual models that will aid the learner to develop adequate and appropriate mental models"


% -----From Fiske and Taylor-----
% Can't access without buying it


==> inserts/brca_correlation.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\vskip -0.4in
\begin{center}
\centerline{\includegraphics[width=0.78\columnwidth]{images/brca_correlation.pdf}}

\vskip -0.8in

\centerline{\includegraphics[width=0.78\columnwidth]{images/brca_rank_correlation.pdf}}

\vskip -0.45in

\caption{Mean correlation (top) and Spearman rank correlation (bottom) between different explanation methods on the BRCA dataset.}
\label{fig:brca_correlation}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/brca_grid.tex <==
\begin{figure}%[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/brca_explanation_grid.pdf}
\caption{Grid of dataset loss explanations for the BRCA subtype classification. Each bar chart represents gene attribution values for a different explanation method. The vertical axis represents feature removal strategies, and the horizontal axis represents summary strategies.}
\label{fig:brca_grid}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/brca_selection.tex <==
\begin{figure}%[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/brca_multiple_selection.pdf}
\caption{Feature selection results when using the top genes identified by each explanation method. Each bar represents the average loss for models trained using 1-20 top genes (lower is better).}
\label{fig:brca_selection}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/census_correctness.tex <==
\begin{figure}[t]
% \vskip 0.2in
% \vskip -0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{images/census_correlation_correctness.pdf}}

\centerline{\includegraphics[width=\columnwidth]{images/census_mse_correctness.pdf}}

% \centerline{\includegraphics[width=\columnwidth]{images/census_correlation_correctness.pdf}}

\caption{Boxplots quantifying the similarity of census income explanations to comparable explanations generated using separate models (a proxy for using the true conditional distribution). The similarity metrics are correlation (top, higher is better) and MSE (bottom, lower is better).}
% , and they are calculated for 256 examples.}
\label{fig:census_correctness}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/census_correlation.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\vskip -0.4in
\begin{center}
\centerline{\includegraphics[width=0.78\columnwidth]{images/census_removal_similarity.pdf}}

\vskip -0.8in

\centerline{\includegraphics[width=0.78\columnwidth]{images/census_summary_similarity.pdf}}

\vskip -0.45in

\caption{Mean correlation between different explanation methods on the census income dataset.
% (blue represents positive correlation and red represents negative).
Methods are grouped by their feature removal approach (top) or summary approach (bottom).}
\label{fig:census_correlation}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/census_grid.tex <==
\begin{figure}%[t]
\vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/census_explanation_grid.pdf}
\caption{Grid of prediction explanations for a single example in the census income dataset. Each bar chart represents attribution values for a different explanation method. The vertical axis represents feature removal strategies, and the horizontal axis represents summary strategies.}
\label{fig:census_grid}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/common_old.tex <==
%% Original, no check marks
% \begin{table}[t]
% \caption{Common combinations of choices in recent work.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccc}
% \toprule
% \textsc{Dimensions} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$v_x(S) = F(x_S)$ \\$E_i(v_x) = \phi_i(v_x)$} & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $v_{x}(S) = F(x_S)$} & Occlusion, LIME (images), MM, RISE\footnotemark[8] \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$w(S) = - \E\Big[\ell\big(F(X_S), Y\big)\Big]$ \\ $E_i(w) = w(D) - w(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO), permutation tests, \\conditional permutation tests} \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = f_S(x_S)$ \\ $w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$} & Univariate predictors, feature ablation (LOCO) \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$ \\ $E_i(w) = \phi_i(w)$} & SAGE, Shapley Net Effects \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$w(S) = - \E\Big[\big(F(x_S), Y\big)\Big]$} & SAGE, conditional permutation tests \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(w) = \phi_i(w)$} & Shapley Net Effects, IME (2009) \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% \makecell{Behavior\\Summary} & \makecell{$v_{x}(S) = F(x_S)$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Occlusion, PredDiff \\
% \midrule
% \makecell{Removal\\Summary} & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(w) = u(D) - u(D \setminus \{i\})$} & Conditional permutation tests, PredDiff \\
% \midrule
% \makecell{Removal\\Behavior} & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $v_{x}(S) = F(x_S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% %% Version 2, check marks, specific games
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{$v_x(S) = F(x_S)$ \\$E_i(v_x) = \phi_i(v_x)$} & \makecell{IME, QII, SHAP,\\KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $v_{x}(S) = F(x_S)$} & \makecell{Occlusion, LIME (images),\\MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{$v(S) = - \E\big[\ell\big(F(X_S), Y\big)\big]$ \\ $E_i(v) = v(D) - v(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO),\\permutation tests,\\cond. permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f_S(x_S)$ \\ $v(S) = - \E\big[\big(F(x_S), Y\big)\big]$} & \makecell{Univariate predictors,\\feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & \makecell{$v(S) = - \E\big[\big(F(x_S), Y\big)\big]$ \\ $E_i(v) = \phi_i(v)$} & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$v(S) = - \E\big[\big(F(x_S), Y\big)\big]$} & \makecell{SAGE,\\cond. permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(u) = \phi_i(u)$} & \makecell{Shapley Net Effects,\\IME (2009)} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & \makecell{$v_{x}(S) = F(x_S)$ \\ $E_i(v_x) = v_x(D) - v_x(D \setminus \{i\})$} & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Cond. permutation tests,\\PredDiff} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $v_{x}(S) = F(x_S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% Version 3, no specific games. This was a bad idea
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Choices} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v_x(S)$ \\$E_i(u) = \phi_i(u)$} & \makecell{IME, QII, SHAP,\\KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $u(S) = v_{x}(S)$} & \makecell{Occlusion, LIME (images),\\MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v(S) = - \E\big[\ell\big(F(X_S), Y\big)\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Feature ablation (LOCO),\\permutation tests,\\cond. permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = f_S(x_S)$ \\ $u(S) = v(S)$} & \makecell{Univariate predictors,\\feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v(S)$ \\ $E_i(u) = \phi_i(u)$} & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\$u(S) = v(S)$} & \makecell{SAGE,\\cond. permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f_S(x_S)$ \\ $E_i(u) = \phi_i(u)$} & \makecell{Shapley Net Effects,\\IME (2009)} \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = f(x_S, r_{\bar S})$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & \makecell{$u(S) = v_{x}(S)$ \\ $E_i(v_x) = v_x(D) - v_x(D \setminus \{i\})$} & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{$F(x_S) = \E\big[f(X) \; | \; X_S = x_S\big]$ \\ $E_i(u) = u(D) - u(D \setminus \{i\})$} & \makecell{Cond. permutation tests,\\PredDiff} \\
% \midrule
% \cmark & \cmark & & \makecell{$F(x, S) = \mathrm{Blur}(x, S)$ \\ $u(S) = v_{x}(S)$} & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

% %% Version 4, no math notation
% \begin{table}[t]
% \caption{Common combinations of choices in recent work. Check marks (\cmark) indicate choices that methods have in common.}
% \label{tab:common_combinations}
% \vskip 0.2in
% \begin{center}
% \begin{small}
% \begin{tabular}{cccc}
% \toprule
% \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Methods} \\
% \midrule
% & \cmark & \cmark & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
% \midrule
% \cmark & \cmark & & \makecell{Occlusion, LIME (images), MM, RISE\footnotemark[8]} \\
% \midrule
% & \cmark & \cmark & \makecell{Feature ablation (LOCO), permutation tests,\\conditional permutation tests} \\
% \midrule
% \cmark & \cmark & & \makecell{Univariate predictors, feature ablation (LOCO)} \\
% \midrule
% & \cmark & \cmark & SAGE, Shapley Net Effects \\
% \midrule
% \cmark & \cmark & & \makecell{SAGE, conditional permutation tests} \\
% \midrule
% \cmark & & \cmark & \makecell{Shapley Net Effects, IME (2009)} \\
% \midrule
% \cmark & & \cmark & Occlusion, CXPlain \\
% \midrule
% & \cmark & \cmark & Occlusion, PredDiff\footnotemark[9] \\
% \midrule
% \cmark & & \cmark & \makecell{Conditional permutation tests, PredDiff} \\
% \midrule
% \cmark & \cmark & & MP, EP \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.2in
% \end{table}

%% Version 5, cross marks
\begin{table}[t]
\caption{Common combinations of choices in existing methods. Check marks (\cmark) indicate choices that are identical between methods.}
\label{tab:common_combinations}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{tabular}{cccc}
\toprule
\textsc{Removal} & \textsc{Behavior} & \textsc{Summary} & \textsc{Methods} \\
\midrule
& \cmark & \cmark & \makecell{IME, QII, SHAP, KernelSHAP, TreeSHAP} \\
\midrule
\cmark & & \cmark & \makecell{SHAP, LossSHAP, SAGE, Shapley Effects} \\
\midrule
\cmark & \cmark & & \makecell{Occlusion, LIME (images), MM, RISE} \\ % \footnotemark[2]} \\
\midrule
& \cmark & \cmark & \makecell{Feature ablation (LOCO), permutation tests,\\conditional permutation tests} \\
\midrule
\cmark & \cmark & & \makecell{Univariate predictors, feature ablation (LOCO),\\Shapley Net Effects} \\
\midrule
& \cmark & \cmark & SAGE, Shapley Net Effects \\
\midrule
\cmark & \cmark & & \makecell{SAGE, conditional permutation tests} \\
\midrule
\cmark & & \cmark & \makecell{Shapley Net Effects, IME (2009)} \\
\midrule
\cmark & & \cmark & Occlusion, CXPlain \\
\midrule
& \cmark & \cmark & Occlusion, PredDiff \\ % \footnotemark[3] \\
\midrule
\cmark & & \cmark & \makecell{Conditional permutation tests, PredDiff} \\
\midrule
\cmark & \cmark & & SHAP, PredDiff \\
\midrule
\cmark & \cmark & & MP, EP \\
\midrule
& \cmark & \cmark & EP, FIDO-CA \\
\midrule
\cmark & \cmark & \cmark & L2X, INVASE \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% \footnotetext[2]{Setting removed features to zero is a special case of using default values.}
% \footnotetext[3]{PredDiff analyzes the log-odds ratio rather than the raw model output, but this is a minor difference.}
% \addtocounter{footnote}{2}

==> inserts/consistency.tex <==
\begin{table}[t]
\caption{Conventions for removing features may be consistent with the data distribution $p(X)$, consistent with another distribution $q(X) \neq p(X)$, or not consistent with any distribution.}
\label{tab:consistency}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{ccc}
\toprule
\textsc{Convention} & \textsc{Methods} & \textsc{Consistency} \\
\midrule
Marginalize (conditional) & \makecell{Cond. permutation tests, \\ PredDiff, SHAP, LossSHAP, \\SAGE, Shapley Effects} & Consistent with $p(X)$ \\
\midrule
Separate models & \makecell{Feature ablation (LOCO), \\univariate predictors, \\Shapley Net Effects, \\IME (2009)} & \multirow{3}{*}{\makecell{Consistent with $p(X)$\\ (assuming model optimality)}}\\
\cmidrule{1-2}
Missingness during training & L2X & \\
\midrule
Marginalize (marginals product) & QII & \multirow{2.5}{*}{\makecell{Consistent with a $q(X)$ that \\assumes feature independence}} \\
\cmidrule{1-2}
Marginalize (uniform) & IME (2010) & \\
\midrule
Zeros & \makecell{Occlusion, PredDiff \\ RISE, CXPlain} & \multirow{2.5}{*}{\makecell{Consistent with constant \\distributions $q(X)$}} \\
\cmidrule{1-2}
Default values & LIME (images), MM & \\
\midrule
Marginalize (marginal) & \makecell{Permutation tests, \\KernelSHAP, \\SAGE sampling} & \multirow{4}{*}{\makecell{Not consistent with \\any $q(X)$}}\\
\cmidrule{1-2}
Tree distribution & TreeSHAP & \\
\cmidrule{1-2}
Extend pixel values & MIR & \\
\midrule
Blurring & MP, EP & \multirow{2.5}{*}{Not valid $F \in \mathfrak{F}$}\\
\cmidrule{1-2}
Marginalize (replacement dist.) & LIME (tabular) & \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> inserts/cooperative.tex <==
\begin{table}
\caption{Each method's summarization technique can each be understood in terms of concepts from cooperative game theory.}
\label{tab:cooperative}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{ccc}
\toprule
\textsc{Summarization} & \textsc{Methods} & \textsc{Related To} \\
\midrule
Shapley value & \makecell{Shapley Net Effects, IME, \\QII, SHAP (TreeSHAP, \\KernelSHAP, LossSHAP), \\Shapley Effects, SAGE} & \makecell{Shapley value, \\probabilistic values,\\modeling cooperative games} \\
\midrule
Mean value when included & RISE & \makecell{Banzhaf value, \\probabilistic values, \\modeling cooperative games} \\
\midrule
\makecell{Remove/include individual \\players} & \makecell{Occlusion, PredDiff, CXPlain, \\permutation tests,\\ univariate predictors, \\feature ablation (LOCO)} & \makecell{Probabilistic values, \\modeling cooperative games} \\
\midrule
Linear model & LIME & \makecell{Shapley value, Banzhaf value, \\modeling cooperative games} \\
\midrule
High/low value coalitions & MP, MIR, MM, L2X, EP & \makecell{Maximum/minimum excess} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> inserts/genes.tex <==
\begin{table}[t]
\caption{List of genes analyzed.}
\label{tab:genes}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{cccccc}
\toprule
Genes 1-17 & Genes 18-34 & Genes 35-51 & Genes 52-68 & Genes 69-85 & Genes 86-100 \\
\midrule
OSTbeta & NBR2 & TSHR & HPS4 & GRINA & C20orf111 \\
STATH & CCDC64 & C7 & ZFPM1 & YTHDF3 & OMA1 \\
MAPK10 & NUP210 & CRYBB2 & OAS2 & TMCC1 & NCAPH2 \\
PLEKHG5 & HEMGN & PPAPDC3 & TUBA1C & UBE1DC1 & GPX2 \\
ERO1L & SLC25A3 & TXNL4B & OR8K5 & C6orf15 & BPY2C \\
ZNF711 & LEF1 & CHST9 & THSD3 & PDE6A & ZNF324 \\
ZNF385 & MVD & HACE1 & ATP6V0C & PEO1 & CDC27 \\
OR52E8 & OTUD3 & AYTL1 & RAB22A & TMEM52 & CCNB2 \\
SLC5A11 & KIAA1949 & PRSS35 & AP1B1 & PARP1 & CNOT7 \\
P4HA3 & SLC44A3 & ZNF408 & CTAGE6 & GSS & BIRC3 \\
LHFPL4 & ZNF775 & DDC & C6orf26 & RDH11 & GAL3ST3 \\
MGC33657 & THY1 & CSTL1 & ESR1 & STXBP1 & PLEKHM1 \\
CAPZB & DYNC1I2 & OR2F1 & UPK3B & ACLY & SPOCD1 \\
RBM15B & CYP1A1 & C12orf50 & ROBO4 & TMSB10 & PENK \\
C1orf176 & SPTA1 & SH3YL1 & TMEFF1 & TUBB & TAS2R9 \\
KLF3 & CLEC4M & SNUPN & KIAA1279 & LIPK & \\
OLFM4 & RXFP3 & COL25A1 & ZFP36L1 & HRC & \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> inserts/information.tex <==
\begin{table}
\caption{Each method's underlying set function has an information-theoretic interpretation when features are removed appropriately.}
\label{tab:information}
\vskip 0.2in
\begin{center}
\begin{small}
\begin{tabular}{cccc}
\toprule
\textsc{Model Behavior} & \textsc{Set Function} & \textsc{Methods} & \textsc{Related To} \\
\midrule
Prediction & $v_x$ & \makecell{Occlusion, MIR, MM, \\IME, QII, LIME, MP, EP, \\SHAP, (KernelSHAP, \\TreeSHAP), RISE} & \makecell{Conditional probability, \\conditional expectation} \\
\midrule
Prediction loss & $v_{xy}$ & LossSHAP, CXPlain & \makecell{Pointwise mutual \\information} \\
\midrule
Prediction mean loss & $w_x$ & L2X & \makecell{KL divergence with \\conditional distribution} \\
\midrule
Dataset loss (label) & $v$ & \makecell{Permutation tests, \\univariate predictors, \\feature ablation (LOCO), \\Shapley Net Effects, SAGE} & \makecell{Mutual information \\(with label)} \\
\midrule
Dataset loss (output) & $w$ & Shapley Effects & \makecell{Mutual information \\(with output)} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table}


==> inserts/methods_grid.tex <==
\begin{figure*}[t]
\vskip -0.1in
\begin{center}
% \includegraphics[trim=1.35cm 0.2cm 5.5cm 0.6cm, clip=true, width=\textwidth]{images/methods_grid_large.pdf}
\includegraphics[trim=1.4cm 0.82cm 7.0cm 0.6cm, clip=true, width=\textwidth]{images/methods_grid_extended.pdf}
\vskip 0.1in
\caption{Visual depiction of the space of removal-based explanations.}
\label{fig:methods_grid}
\end{center}
\vskip -0.2in
\end{figure*}

==> inserts/mnist_examples.tex <==
\begin{figure}%[t]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/mnist_examples.pdf}
\caption{More MNIST prediction loss explanations using LossSHAP (feature removal with the conditional distribution and summary with the Shapley value).}
\label{fig:mnist_examples}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/mnist_grid.tex <==
\begin{figure}
% \vskip 0.2in
\vskip -0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/mnist_explanation_grid_digit.pdf}
\caption{Grid of prediction loss explanations for a single MNIST example. The vertical axis represents feature removal strategies and the horizontal axis represents summary strategies. Red pixels improve the loss, and blue ones hurt it (except for mean when included).}
\label{fig:mnist_grid}
\end{center}
\vskip -0.2in
\end{figure}

==> inserts/table.tex <==
\begin{table}[t]
\caption{Choices made by existing removal-based explanations.}
\label{tab:methods}
\vskip -0.1in
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccc}
\toprule
\textsc{Method} & \textsc{Removal} & \textsc{Behavior} & \textsc{Summary} \\
\midrule
IME (2009) & Separate models & Prediction & Shapley value \\
IME (2010) & Marginalize (uniform) & Prediction & Shapley value \\
QII & Marginalize (marginals product) & Prediction & Shapley value \\
SHAP & Marginalize (conditional/marginal) & Prediction & Shapley value \\
KernelSHAP & Marginalize (marginal) & Prediction & Shapley value \\
TreeSHAP & Tree distribution & Prediction & Shapley value \\
LossSHAP & Marginalize (conditional) & Prediction loss & Shapley value \\
SAGE & Marginalize (conditional) & Dataset loss (label) & Shapley value \\
Shapley Net Effects & Separate models & Dataset loss (label) & Shapley value \\
Shapley Effects & Marginalize (conditional) & Dataset loss (output) & Shapley value \\
Permutation Test & Marginalize (marginal) & Dataset loss (label) & Remove individual \\
Conditional Perm. Test & Marginalize (conditional) & Dataset loss (label) & Remove individual \\
Feature Ablation (LOCO) & Separate models & Dataset loss (label) & Remove individual \\
Univariate Predictors & Separate models & Dataset loss (label) & Include individual \\
L2X & Missingness during training & Prediction mean loss & High-value subset \\
INVASE & Missingness during training & Prediction mean loss & High-value subset \\
LIME (Images) & Default values & Prediction & Linear model \\
LIME (Tabular) & Marginalize (replacement dist.) & Prediction & Linear model \\
PredDiff & Marginalize (conditional) & Prediction & Remove individual \\
Occlusion & Zeros & Prediction & Remove individual \\
CXPlain & Zeros & Prediction loss & Remove individual \\
RISE & Zeros & Prediction & Mean when included \\
MM & Default values & Prediction & Partitioned subsets \\
MIR & Extend pixel values & Prediction & High-value subset \\
MP & Blurring & Prediction & Low-value subset \\
EP & Blurring & Prediction & High-value subset \\
FIDO-CA & Generative model & Prediction & High-value subset \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vskip -0.1in
\end{table}

==> inserts/tradeoff.tex <==
\begin{figure*}[t]
\vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/tradeoff.png}
\caption{Each model explanation strategy represents a trade-off between an explanation's simplicity and its completeness.}
\label{fig:tradeoff}
\end{center}
\vskip -0.2in
\end{figure*}

==> old/census_summary_correlation.tex <==
\begin{figure*}[h!]
\vskip 0.2in
\begin{center}
\includegraphics[width=0.5\columnwidth]{images/census_summary_similarity.pdf}
\caption{Blah}
\label{fig:census_summary_correlation}
\end{center}
\vskip -0.2in
\end{figure*}

==> old/methods_grid_table.tex <==
% \begin{table}[t]
% \caption{Systematization of existing methods.}
% \label{tab:methods_grid}
% \vskip 0.2in
% \begin{center}
% \begin{tiny}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% & \makecell{Remove \\Individual} & \makecell{Include\\Individual} & \makecell{Mean When\\Included} & \makecell{Shapley\\Value} & \makecell{Linear\\Model} & \makecell{High\\Value\\Subset} & \makecell{Low\\Value\\Subset} & \makecell{Partitioned\\Subsets} \\
% \hline
% \makecell{Zeros} & \makecell{Occlusion\\CXPlain} && RISE &&&&& \\
% \hline
% \makecell{Default\\Values} & & & & & \makecell{LIME\\(images)} & & & MM \\
% \hline
% \makecell{Extend\\pixels} &&&&&& MIR && \\
% \hline
% \makecell{Blurring} & \makecell{{}\\{}} &&&&& EP & MP & \\
% \hline
% \makecell{Marginalize\\(replacement\\dist.)} &&&&& \makecell{LIME\\(tabular)} &&& \\
% \hline
% \makecell{Marginalize\\(uniform)} &&&& IME (2010) &&&&\\
% \hline
% \makecell{Marginalize\\(marginals\\product)} &&&& QII &&&& \\
% \hline
% \makecell{Marginalize\\(marginal)} & \makecell{Permutation\\test} &&& \makecell{KernelSHAP,\\SHAP,\\SAGE Sampling} &&&& \\
% \hline
% \makecell{Marginalize\\(conditional)} & \makecell{PredDiff,\\cond. perm.\\test} &&& \makecell{SHAP,\\LossSHAP,\\SAGE,\\Shapley Effects} &&&& \\
% \hline
% \makecell{Tree\\distribution} &&&& TreeSHAP &&&& \\
% \hline
% \makecell{Missingness\\during\\training} &&&&&& L2X && \\
% \hline
% \makecell{Separate\\models} & \makecell{Feature\\ablation} & \makecell{Univariate\\predictors} && \makecell{IME (2009),\\Shapley Net Effects} &&&& \\
% \hline
% \end{tabular}
% \end{tiny}
% \end{center}
% \vskip -0.2in
% \end{table}

% % Version 2, no midrules/hlines
% \begin{table}[t]
% \caption{Systematization of existing methods.}
% \label{tab:methods_grid}
% \vskip 0.2in
% \begin{center}
% \begin{tiny}
% \begin{tabular}{ccccccccc}
% \toprule
% & \makecell{Remove \\Individual} & \makecell{Include\\Individual} & \makecell{Mean When\\Included} & \makecell{Shapley\\Value} & \makecell{Linear\\Model} & \makecell{High\\Value\\Subset} & \makecell{Low\\Value\\Subset} & \makecell{Partitioned\\Subsets} \\
% \midrule
% % \cmidrule(lr){2-9}
% \makecell{Zeros} & \makecell{Occlusion\\CXPlain} & \makecell{{}\\{}\\{}} & RISE &&&&& \\
% %\midrule
% \makecell{Default\\Values} & \makecell{{}\\{}\\{}} & & & & \makecell{LIME\\(images)} & & & MM \\
% %\midrule
% \makecell{Extend\\pixels} & \makecell{{}\\{}\\{}}&&&&& MIR && \\
% %\midrule
% \makecell{Blurring} & \makecell{{}\\{}} &&&&& EP & MP & \\
% %\midrule
% \makecell{Marginalize\\(replacement\\dist.)} &&&&& \makecell{LIME\\(tabular)} &&& \\
% %\midrule
% \makecell{Marginalize\\(uniform)} & \makecell{{}\\{}\\{}} &&& IME (2010) &&&&\\
% %\midrule
% \makecell{Marginalize\\(marginals\\product)} &&&& QII &&&& \\
% %\midrule
% \makecell{Marginalize\\(marginal)} & \makecell{Permutation\\test} & \makecell{{}\\{}\\{}\\{}} && \makecell{KernelSHAP,\\SHAP,\\SAGE Sampling} &&&& \\
% %\midrule
% \makecell{Marginalize\\(conditional)} & \makecell{PredDiff,\\cond. perm.\\test} & \makecell{{}\\{}\\{}\\{}\\{}} && \makecell{SHAP,\\LossSHAP,\\SAGE,\\Shapley Effects} &&&& \\
% %\midrule
% \makecell{Tree\\distribution} & \makecell{{}\\{}\\{}} &&& TreeSHAP &&&& \\
% %\midrule
% \makecell{Missingness\\during\\training} & \makecell{{}\\{}\\{}} &&&&& L2X && \\
% %\midrule
% \makecell{Separate\\models} & \makecell{Feature\\ablation} & \makecell{Univariate\\predictors} & \makecell{{}\\{}\\{}} & \makecell{IME (2009),\\Shapley Net Effects} &&&& \\
% \bottomrule
% \end{tabular}
% \end{tiny}
% \end{center}
% \vskip -0.2in
% \end{table}

% Version 3, colors
\begin{table}[t]
\caption{Systematization of existing methods.}
\label{tab:methods_grid}
\vskip 0.2in
\begin{center}
\begin{tiny}
\begin{tabular}{ccccccccc}
% \toprule
& \makecell{Remove \\Individual} & \makecell{Include\\Individual} & \makecell{Mean When\\Included} & \makecell{Shapley\\Value} & \makecell{Linear\\Model} & \makecell{High\\Value\\Subset} & \makecell{Low\\Value\\Subset} & \makecell{Partitioned\\Subsets} \\
% \midrule
% \cmidrule(lr){2-9}
\makecell{Zeros} & \makecell{\pred{Occlusion},\\\predloss{CXPlain}} & \makecell{{}\\{}\\{}} & \pred{RISE} &&&&& \\
%\midrule
\makecell{Default\\Values} & \makecell{{}\\{}\\{}} & & & & \makecell{\pred{LIME}\\\pred{(images)}} & & & \pred{MM} \\
%\midrule
\makecell{Extend\\pixels} & \makecell{{}\\{}\\{}}&&&&& \pred{MIR} && \\
%\midrule
\makecell{Blurring} & \makecell{{}\\{}} &&&&& \pred{EP} & \pred{MP} & \\
%\midrule
\makecell{Marginalize\\(replacement\\dist.)} & \makecell{{}\\{}\\{}\\{}} &&&& \makecell{\pred{LIME}\\\pred{(tabular)}} &&& \\
%\midrule
\makecell{Marginalize\\(uniform)} & \makecell{{}\\{}\\{}} &&& \pred{IME (2010)} &&&&\\
%\midrule
\makecell{Marginalize\\(marginals\\product)} & \makecell{{}\\{}\\{}\\{}} &&& \pred{QII} &&&& \\
%\midrule
\makecell{Marginalize\\(marginal)} & \makecell{\datasetloss{Permutation}\\\datasetloss{test}} & \makecell{{}\\{}\\{}\\{}} && \makecell{\pred{KernelSHAP},\\\pred{SHAP},\\\datasetloss{SAGE Sampling}} &&&& \\
%\midrule
\makecell{Marginalize\\(conditional)} & \makecell{\pred{PredDiff},\\\datasetloss{cond. perm.}\\\datasetloss{test}} & \makecell{{}\\{}\\{}\\{}\\{}} && \makecell{\pred{SHAP},\\\predloss{LossSHAP},\\\datasetloss{SAGE},\\\datasetmodelloss{Shapley Effects}} &&&& \\
%\midrule
\makecell{Tree\\distribution} & \makecell{{}\\{}\\{}} &&& \pred{TreeSHAP} &&&& \\
%\midrule
\makecell{Missingness\\during\\training} & \makecell{{}\\{}\\{}\\{}} &&&&& \predmeanloss{L2X} && \\
%\midrule
\makecell{Separate\\models} & \makecell{\datasetloss{Feature}\\\datasetloss{ablation}} & \makecell{\datasetloss{Univariate}\\\datasetloss{predictors}} & \makecell{{}\\{}\\{}} & \makecell{\pred{IME (2009)},\\\datasetloss{Shapley Net Effects}} &&&& \\
% \bottomrule
\end{tabular}
\end{tiny}
\end{center}
\vskip -0.2in
\end{table}

% \pred{$\blacksquare$ Prediction}

% \predloss{$\blacksquare$ Prediction Loss}

% \predmeanloss{$\blacksquare$ Prediction Mean Loss}

% \datasetloss{$\blacksquare$ Dataset Loss}

% \datasetmodelloss{$\blacksquare$ Dataset Loss (Output)}

==> old/psychology_1.tex <==
\section{The Psychology of Learning by Ignoring} \label{sec:psychology}

Most model explanation methods are not derived from relevant research in psychology or philosophy \citep{miller2017explainable}. Here, we show that the methods discussed so far nonetheless have parallels with established ideas about how explanations should be formed for humans. We illuminate links with the social sciences by pointing to influential works whose proposals are consistent with methods in the learning by ignoring paradigm.

% Model explanation is implicitly a question about the causes for a model behaving in a particular way.
% % (We emphasize that it is not about potential causal relationships between the model input and the response variable).
% Even the question ``why does the model predict $y$'' is ambiguous, however; in a view that is representative of the literature on this topic, \cite{hilton1990conversational} claims that events are not explained per se, but that \textit{why} questions have either an implicit or explicit \textit{rather than} built in. \cite{lipton1990contrastive} refers to the alternative scenario as a \textit{foil}, and \cite{miller2019explanation} suggests that specific foils could be elicited from human observers in the context of machine learning interpretability.

% Methods in the learning by ignoring paradigm involve no human interaction, so they assume a certain behavior to be explained, as well as the corresponding foil. \textcolor{red}{TODO not sure what the foil is. It sounds stupid to say, why y instead of not y, because as Miller points out, that requires an explanation of the full chain of causality. This is not a fruitful perspective.}

% \textcolor{red}{The fact-foil perspective about unambiguous questions from Hilton, Van blah blah and Lipton is NOT useful. We do not elicit fact-foil pairs, and proposing implicit fact-foils pairs could sort of be done by looking at summarization methods; but the result won't be convincing, because the explanations provided are not perfect answers to those questions. Ultimately, suggesting the implicit questions being answered does not seem like a valuable endeavor.}

% Model explanation is implicitly a causality question about why a model behaves in a particular way.
% the causes for a model behaving in a particular way.
% (We emphasize that it is not about potential causal relationships between the model input and the response variable).
% For example, the underlying question may be about why the model makes a certain prediction, or why its cross entropy loss is a certain value.
% Such open ended questions are called \textit{plain fact} questions \citep{van2002remote}, and are generally thought to be more difficult to answer then more detailed why questions with built in alternative scenarios, or \textit{foils}, such as \textit{why A and not B?} \citep{hilton1990conversational, lipton1990contrastive, miller2019explanation}. Most model explanation methods, including those in the learning by ignoring paradigm, neglect to elicit particular foils from users, but we can consider whether they implicitly assume one.
% Such open ended questions are called \textit{plain fact} questions \citep{van2002remote}, which are generally more difficult to answer than why questions with specific alternative scenarios (foils) \citep{hilton1990conversational, lipton1990contrastive, miller2019explanation}.
% Rather than explaining these events relative to a particular alternative \cite{hilton1990conversational}, methods in the learning by ignoring paradigm answer so-called plain fact questions, which are generally more difficult to answer \cite{lipton1990contrastive}.
% \textcolor{red}{TODO are we sure that none of these methods have implicit foils? MP for example says why probability is high rather than low, and gives simple explanation with few causes.}

% For methods in the learning by ignoring paradigm, there is no single foil that is implicitly considered by all methods. Our approach is to consider individual methods, and given the explanations that are provided, point out the specific questions that these methods answer accurately. By providing an additive credit allocation, methods that use the Shapley value to provide explanations implicitly answer the question \textit{why was the set function equal to $u(D)$ rather than $u(\{\})$?} By finding sets of high-valued players, the optimization based methods implicitly answer the question \textit{why was the set function $u(D)$ large rather than small?}

% We cannot make a general claim about the foils that are considered by our class of explanation methods. What we can do is carefully consider an individual method, and given the explanation that it provides, point out what specific questions they answer. For example, SHAP answers the question \textit{why does the model predict $f(x)$, rather than $\E[f(X)]$?} And MP answers the question \textit{why did class $y$ seem probable rather than improbable?}

Model explanation is implicitly a \textit{causality} question about why a model behaves in a particular way.
% (We emphasize that it is not about potential causal relationships between the model input and the response variable).
For example, the underlying question may be about why the model makes a certain prediction, or why its cross entropy loss is a certain value. The subject of causality has attracted much work in the social sciences. \textcolor{red}{TODO should I be mentioning Pearl here?} There are a breadth of views in the literature, but many perspectives are based on the concept of counterfactual logic, where causation is determined by the impact of changing some facts on the outcome \citep{hume2000enquiry, mill1884system}. In the psychology literature, researchers have observed that people are able to mentally undo events by generating counterfactual scenarios \citep{tversky1982simulation}. \cite{wachter2017counterfactual} suggests that carefully chosen counterfactuals provide sufficient explanations for black box models. Methods in the learning by ignoring paradigm are built on counterfactual logic, albeit in a more subtle way.

Making predictions for different inputs is equivalent to a counterfactual, which may or may not change the outcome \citep{wachter2017counterfactual}. All of the conventions described for making predictions in the absence of features are in fact counterfactuals. In particular, the convention of marginalizing out missing features is highly similar to the mental model described by Norm Theory, in which a set of relevant exemplars is evoked, matching on certain immutable attributes but possibly varying on the mutable attributes \citep{kahneman1986norm}; the summary statistics from the evoked set are used to define a norm, or make a prediction in the absence of information.
% Alternatively, we can view the idea of making predictions with a subset of features as a counterfactual, where instead of prescribing alternative values, we prescribe ignorance of the values.

Individual counterfactuals are therefore the atoms of these explanation methods, rather than their final product. This is similar to the view of \cite{merrick2019explanation}, who define a counterfactual reference distribution to explain the large number of references used in Shapley-value based methods.

When it comes to providing explanations, the methods take different approaches. The methods that identify a set of important features provide simple explanations with few causes, which tend to be preferred by humans \citep{hilton1990conversational, miller2019explanation}. However, identifying a small number of causes without quantifying their impact is misleading, and could play into cognitive biases towards oversimplification \citep{}. By contrast, feature attribution methods consider every feature as a candidate cause, and distinguish between the different degrees of causality.

% Most machine learning explanation methods are not derived from relevant research in psychology, philosophy, or the cognitive sciences \citep{miller2017explainable}. We show that despite the apparent disconnect between these areas of research, methods in the learning by ignoring paradigm are consistent with influential ideas from the social sciences about how humans form explanations.

% Model explanation is implicitly a question of \textit{causality}, about what caused the model to make certain predictions. We emphasize that the causal question is not about potential causal relationships between the input and the response variable. 

% In a broad review of social science research that relates to machine learning interpretability, \cite{miller2019explanation} points out that most explanation methods are not derived from existing research in philosophy, psychology, or cognitive sciences. Although the methods in the learning by ignoring paradigm were not conceived with the explicit intention of building on social science research, we show that they can be understood in the context of existing ideas about how humans form explanations.

% I'm struggling with the decision to center this section around findings from social science papers, or to center it on learning by ignoring and bring things up as necessary.

% \begin{enumerate}
%     \item Contrastive explanations (fact and foil). Understanding how a model makes predictions is an ambiguous question, but Hilton says well founded questions are about why P happened rather then Q. Each method here implicitly assumes a fact based on their underlying set function (the prediction, the loss, etc.). The foil is not specific, but it why didn't some other value occur? Maybe clearer for additive methods.
%     \item Validity of counterfactual thinking for understanding causation (in this case, cause for specific model behavior) can be traced back to John Stuart Mill's method of difference. 
%     \item Counterfactual reasoning about causes. Kahneman and other citations in Asylum paper point out that people understand causality by undoing effects by mental simulation. Wachter cites lots of work to show that counterfactuals provide the best way of understanding models (need to read more closely). In machine learning, counterfactuals are represented by different inputs, and possibly different outputs. In learning by ignoring, a wide variety of counterfactuals are considered, like an evoked set, and their summary statistics summarized. Taly also likes counterfactual thinking, and talks about a counterfactual reference distribution. We do something similar, consider many counterfactuals.
%     \item Explanations are preferred to be simple and selected. The selection-based methods provide selections, which should be easier to understand. The attribution methods are less appealing because they're complicated, but more mathematically principled because they consider that everything is a cause to some degree.
% \end{enumerate}

% --

% --

% --

% --

% --

% Ideas:

% \begin{enumerate}
%     \item Kahneman has his thing about mentally undoing: explaining events by finding counterfactuals that are not too different, but change the outcome. Specific definition of not too different, because part of what's interesting is what people like to undo.
%     \item Think I've heard that people like counterfactuals in general. Ignoring a feature is a counterfactual, and its analogous to asking a doctor what would you think if I hadn't shown you this? Can distinguish between changing input to a specific value, and ignoring the value.
%     \item If you accept that ignoring information is like a counterfactual, then the set functions we describe represent $2^d$ possible counterfactuals, and the explanation methods summarize this information in a concise way. The attribution methods generally condense the information into scores for each feature. The optimization-based methods identify single insightful counterfactuals.
%     \item There's a tradeoff between summarizing all the counterfactuals in a way that provides as much information as possible (while satisfying good properties), and communicating something that's easy to understand (here are the most important features). Humans are bad at processing a lot of information, so there's something appealing about a simple explanation, even if is less informative than something complicated.
%     \item On the subject of ignoring features, worth talking about how humans would ignore features. Two doctors that make the same diagnoses in the presence of all information may differ when some information is missing, just like we can have two EPFs $F, G$ that satisfy $F(x, D) = G(x, D)$. Which one would you rather do the ignoring exercise with, someone who is consistent when information is held out, or something else? You learn more when they're consistent. But there's probably some logical fallacy that says people are bad at the mental simulation required to take into account the missing features' conditional distributions.
%     \item Although simple counterfactuals might be easier to understand, the lesson of the Shapley value is that giving a maximally representative summary is more complicated. People might like simplicily, but it probably plays into their inherent selection bias (or explanation bias, or hindsight bias), and makes them think that events are entirely due to the selected features and the others don't matter at all. The Shapley value tries to give an explanation that is more faithful to the full truth.
%     \item The simulation heuristic paper says that there are tasks of judgement where people seem to rely on simulating scenarios. Norm Theory proposes a mental model for how people define their norms: by recruiting recalled and constructed representations, and aggregating summary statistics. When constructing representations, there are certain mutable and certain immutable features. Parallel with how we use sets of information to evoke set of other representations, whose summary statistics are gathered, to give predictions in absence of some information. Summarizing many counterfactuals.
%     \item Although assigning specific attribute values can be seen as a counterfactual, can also see missing some information as a counterfactual. Shapley value aggregates that kind of information. 
%     \item Probably some named concept for how this would be too much computation for a person to actually perform.
%     \item There's a lot of work on psychology of causality attribution...
%     \item Maybe some papers that outright say people like to think in counterfactuals.
%     \item We have the choice of saying that predictions made in the absence of some information are made using the simulation heuristic, by aggregating information from a bunch of counterfactuals. Also have the choice of saying that a prediction in the absence of information is itself a counterfactual, and we can combine many of those. For the latter, more like evoking a category.
%     \item I want to make the point that counterfactuals are the atoms of explanations. Whereas Wachter paper thinks that counterfactuals and explanations are distinct. They advocate for using a wide variety of counterfactuals by leveraging domain knowledge and the needs of the recipient of the explanation, but we just combine a lot of them in a reasonable way, that does not take into account the recipient's objective. Holy SHIT, that was a 2017 paper! Simple, early-ish. Not so mad that they didn't see that counterfactuals are atoms and explanations are molecules. Their message is that counterfactuals are sufficient (or even exceed requirements), but there is also a message that you should provide multiple counterfactuals, and account for domain knowledge. We work with multiple counterfactuals, but also provide a default behavior for summarizing them.
%     \item Anything useful to say about Taly paper? They talk about a counterfactual reference distribution. Cite Norm Theory to justify working with counterfactuals to establish norms.
%     \item Big picture, my message here will be that even though these methods were not conceived with the explicit intention of matching up with social science research about how people tend to explain/understand things, it turns out they jive pretty well.
%     \item Hilton suggests that all explanations are contrastive, and that to give a good explanation, you require a fact and a foil. Do we implicitly have a foil in these cases? I think the foil is implicit in the set function.
% \end{enumerate}

==> old/psychology_2.tex <==
\section{The Psychology of Explaining by Ignoring} \label{sec:psychology}

% In this section, we show that the explaining by ignoring framework has a compelling justification in terms of psychological theories about how humans explain events.
% Model explanation methods are not generally designed based on ideas from the social sciences, including psychology, philosophy, or cognitive sciences \citep{miller2017explainable}.
% In this section, we show that the explaining by ignoring framework has clear parallels with psychological theories about how humans explain the causes of events.
% It is rare for model explanation methods to be designed with psychology or philosophy research in mind \citep{miller2017explainable}, but since explanations are ultimately used by humans, it is important to make sure that methods build on the vast amount of social science research dedicated to the topic of explanation \citep{miller2019explanation}. Here, we show that methods in the explaining by ignoring framework have clear links with theories for how humans explain the causes of events.
Model explanation methods are not typically designed based on research in the social sciences, including psychology or philosophy \citep{miller2017explainable}. However, we are able to identify clear parallels between the explaining by ignoring paradigm and cognitive theories of how people understand the causes of events.

\subsection{Counterfactual Reasoning about Causality}

% Model explanation methods are not generally designed based on ideas from social science research, including psychology, philosophy, or cognitive sciences \citep{miller2017explainable, miller2019explanation}. 
% % The methods discussed in this work are not exceptions to this rule, but
% Perhaps surprisingly, we find that the methods discussed here have clear parallels with theories for how humans explain the causes of events. In particular, we show that the explaining by ignoring framework can be understood in terms of counterfactual reasoning. the simulation heuristic \citep{tversky1982simulation}, and Norm Theory \citep{kahneman1986norm}. \textcolor{red}{TODO could try to make a stronger statement.}
% has a compelling justification through its reliance on simulating a distribution of counterfactuals, and presenting explanations that rely on their summary statistics.
% based on counterfactual reasoning, and that explanations are provided by summarizing the results from a distribution of counterfactuals.
% Prior work has encouraged the incorporation of social science findings into explanation methods \cite{miller2019explanation}, and while we support such efforts, we find that explanation methods designed by computer scientists have remarkable parallels with how humans form explanations.

Explaining a model's predictions is fundamentally a causality question: the question is, \textit{why does the model behave this way?} Each input feature is a candidate cause, multiple features may be causal, and the role of an explanation is to quantify each feature's degree of causality. We emphasize that this is distinct from reasoning about causal relationships between the inputs and the response variable, because such relationships cannot be inferred from observational data \citep{pearl2009causality}.

Within the philosophy and psychology literature, \textit{counterfactual reasoning} is one of the dominant tools for understanding causality. A counterfactual example changes certain facts of a situation (e.g., the route a person drove to get home) to potentially achieve a different outcome (e.g., avoiding a car crash), and counterfactuals can shed light on whether each aspect of a situation caused the actual outcome (e.g., a car crash). In an influential philosophical account of causality, John Stuart Mill presents his five methods of induction that use counterfactual thinking to explain cause-effect relationships \citep{mill1884system, mackie1974cement}. And in the psychology literature, counterfactual thinking is the basis of multiple theories about how people explain events \citep{tversky1982simulation, hilton1990conversational}.

Relying on counterfactuals is a natural idea in the context of model explanation. Machine learning models are functions on high dimensional domains, so to understand a model is to understand how it maps different inputs to different outputs. Some work has embraced counterfactual reasoning by suggesting that model predictions should be explained by presenting users with a small number of counterfactual examples \citep{wachter2017counterfactual}.

% In their work that draws on analytic philosophy,
In their work, \cite{wachter2017counterfactual} suggest generating the closest possible counterfactual that achieves a user-specified alternative outcome. But while a single counterfactual can suggest a direction for changing one's outcome or contesting an adverse decision, individual counterfactuals provide insufficient information for understanding each feature's influence on the model. For example, if there are multiple causes for an outcome (e.g., a person's loan application was approved because of a good credit score and a high income level), and the outcome can be changed by reversing any single cause, the closest possible counterfactual may arbitrarily highlight one cause over another (e.g., by showing that a lower credit score would have led to the loan being rejected). It may take a large number of counterfactuals to represent the inner workings of a complex model.

In order to provide a more faithful representation of each feature's influence on the model, we show that rather than directly presenting counterfactuals to users, methods in the explaining by ignoring provide explanations that summarize outcomes from a large number of counterfactuals.

\subsection{Summarizing Counterfactuals}

I'm not sure this is the right section title. And I'm not sure the previous section covers what I need it to. Here's the new direction I want to take.

Everyone thinks you should use counterfactual reasoning to think about causality. That sure makes sense in the context of model explanation, because models are just functions.

How do I work this in... every method wo

A particularly relevant area of psychology research is the study of ``mentally undoing,'' which is about identifying the facts that people blame most for causing events. As an example, one study told people a story about a person who got in a car crash and asked them to imagine what the family would say if they said ``if only...'' The participants came up with counterfactuals that might occur to the people in the story, which effectively identify the causes. For example, many people blamed the unusual way the driver entered the intersection, or the unusual route the man drove (aspects that were emphasized in the story). 

% Given an input $x \in \mathcal{X}$ and the outcome $f(x)$, a counterfactual example may indicate that the feature $X_i$ causes the model output if it shows that changing $X_i$ changes the output. For example, showing that a fifty point reduction to a customer's credit score leads to their loan application being rejected suggests that their credit score is one of the causes for their application being accepted originally.

% Methods in the explaining by ignoring framework do not perform searches to find values that change the output. But by ignoring a feature $X_i = x_i$ or a group of features $X_{\bar S} = x_{\bar S}$, these methods consider the outcomes that arise with alternative values. Each method's approach for removing features uses counterfactuals, either by setting the removed features to specific alternative values, or by integrating over a distribution of alternative values (Section~\ref{sec:missingness_strategies}). We focus here on approaches that marginalize out missing features, because these have a more compelling justification in the psychology literature. In particular, we focus the approach that marginalizes out features with their conditional distribution.

% When $X_{\bar S}$ is ignored, we effectively simulate counterfactual values from the distribution $p(X_{\bar S} \; | \; X_S)$ and record the mean model output from these counterfactuals. A similar process for generating counterfactuals and recording their summary statistics is described by the cognitive model in Norm Theory \citep{kahneman1986norm}. In this work, the authors describe a process wherein a probe (e.g., the input $x$) evokes a set of recalled and simulated alternatives (e.g., counterfactual examples) whose summary statistics define a person's perspective of normal outcomes. SHAP's connections with Norm Theory have been recognized in prior work, which refers to the distribution of alternative values as a \textit{counterfactual reference distribution} \citep{merrick2019explanation}.
% on normal behavior for the phenomenon in question.
% For example, a ``normal'' outcome for a loan application may be considered by recalling acquaintances who applied for loans, or articles about the process, as well as imagining potential applicants and their outcomes. 
% The authors refer to \textit{mutable} and \textit{immutable} features to distinguish between the features that may diverge from the probe, and the features that must remain constant in the counterfactual alternatives.

% In our case, it is as if the probe $x$ evokes a set of counterfactuals, which are constrained to retain certain immutable features $X_S = x_S$, but which may diverge in the mutable features $X_{\bar S}$. And the mutable features for our set of counterfactuals are drawn from a specific distribution $p(X_{\bar S} \; | \; X_S = x_S)$; in Norm Theory, the authors suggest that the primary factors controlling the weight of stimuli in a norm are the strength of the connection (or the similarity) with the probe, and factors affecting the memorability of the stimulus in a person's mind. 

\textcolor{red}{Should maybe give up on finding clear parallels. Norm Theory isn't so specific, or if it is, I don't understand it clearly. Paint a broader picture of what Norm Theory and study of mentally undoing have to say.}

\begin{enumerate}
    \item Counterfactual reasoning about causality: model explanation is a causality question, and lots of people say that causality questions should be addressed using counterfactual reasoning. Some people in ML have embraced that idea by saying that model explanations should just be counterfactuals.
    \item Summarizing counterfactuals: explaining by ignoring means considering counterfactual inputs, because features are removed by setting them to alternative values or integrating over a distribution of alternative values. For the approaches that marginalize out removed features, it is as if the average behavior if defined by integrating over a counterfactual reference distribution (Taly).
    \item Connections with Norm Theory and simulation heuristic: Kahneman and Tversy, and later Kahneman and Miller, developed two related theories for cognitive processes that relate to explaining the causes of events that are relevant to this framework of model explanation methods. In Norm Theory, Kahneman suggests that people follow a cognitive process where they define normal behavior by gathering summary statistics from a set of recalled and simulated representations.
\end{enumerate}

\textcolor{red}{TODO write this from scratch}

\begin{enumerate}
    % \item Like most explanation methods, these were not designed with human psychology research in mind (Miller). But the designers were reasonable people, so maybe that's not necessary. We find clear links with theories about how humans explain the causes of events.
    % \item Explaining a model's behavior is fundamentally a causality question: what made the model behave this way? Emphasize that we're not talking about causal relationships with response variable, which cannot be inferred from observational data (Pearl)
    % \item Everyone agrees that counterfactual reasoning is the most important tool for understanding causality (Hume, Mill, Hilton, etc). Counterfactuals simply change some aspects of the situation, in order to possibly change the outcome. Wachter understands counterfactuals in the context of machine learning as simply evaluating the model with different inputs. Indeed, it seems natural that to understand a model, which is just a function, we must understand how it behaves given different inputs.
    % \item However, it is not obvious which counterfactual examples to present. Wachter suggested presenting several, and Miller suggested soliciting user preference for what kind of different outcomes the user wants to see achieved. We argue that methods that following the explaining by ignoring framework provide explanations that summarize a large number of counterfactual examples, rather than presenting a small number of counterfactuals directly (Wachter).
    \item Begin by observing that when features are ignored, each approach provides counterfactual values for the missing features (Section 3). Some approaches prescribe a single set of values, while others integrate over a distribution of possible values. When integrating across the counterfactual distribution, these approaches consider the different outcomes (model outputs) that might be achieved in proportion to their likelihood. This idea is very similar to Taly's idea of a counterfactual reference distribution, which, as they noted, is reminiscent of Norm Theory (Kahneman).
    \item Feel like I had more to say about Kahneman than Taly did. Don't want to end the section by saying they had the right idea!
    \item It is easy to identify links with psychology research about how people explain the causes of events. Certain conventions for ignoring features are more justified, so we focus our attention on the approach of marginalizing out missing features with their conditional distribution.
    \item Simulation heuristic suggested that people perform certain tasks of judgement by mentally simulating potential outcomes. In the context of mentally undoing events (identifying their causes), people were able to imagine alternative (counterfactual) realities in which different outcomes were achieved. One of the points of the study was to identify people's preferences when generating counterfactual situations. One of the most important findings was that people prefer downhill changes---substituting unlikely inputs for more likely alternatives (a person driving on their regular route, rather than an unusual one).
    \item People's preference for downhill changes suggests that they are sensitive to a measure of events' likelihood. Rather than identifying an event as causal because it has one high likelihood alternative value that changes the outcome, we might consider a distribution of alternative values, and consider the different outcomes in proportion to their likelihood.
    \item Wanted to work in mutable, immutable features.
\end{enumerate}

==> old/psychology_3.tex <==
\section{The Psychology of Removal-Based Explanations} \label{sec:psychology}

Model explanation methods are not typically designed based on research from the social sciences, including either psychology or philosophy \citep{miller2017explainable}. However, we are able to identify clear parallels between removal-based explanations and cognitive theories about how people understand the causes of events. We begin by discussing the role of counterfactual reasoning in our framework, and we then discuss a trade-off between simple explanations and explanations that convey more information about the model.

\subsection{Counterfactual reasoning about causality}

Explaining a model's predictions is fundamentally a causality question: the question is, \textit{why does the model behave this way?} Each input feature is a candidate cause, multiple features may be causal, and the role of an explanation is to quantify each feature's degree of influence on the model. We emphasize that this is distinct from reasoning about causal relationships in the data (e.g., whether smoking causes cancer), because these relationships are difficult to infer from observational data \citep{pearl2009causality}.

Within the philosophy and psychology literature, \textit{counterfactual reasoning} is one of the dominant tools for understanding causality. A counterfactual example changes certain facts of a situation (e.g., the route a person drove to get home) to potentially achieve a different outcome (e.g., avoiding a car crash), and counterfactuals can shed light on whether each aspect of a situation caused the actual outcome (e.g., a fatal car crash). In an influential philosophical account of causality, John Stuart Mill presents his five methods of induction that use counterfactual thinking to explain cause-effect relationships \citep{mill1884system, mackie1974cement}. In the psychology literature, counterfactual thinking is the basis of multiple theories about how people explain events \citep{tversky1982simulation, hilton1990conversational}.

In a well-known empirical study, \cite{tversky1982simulation} examined the process of \textit{mental undoing}, or imagining counterfactuals to change an event's outcome. The authors theorized that to mentally undo an event, people would identify facts of the story that could be changed in order to mentally simulate a different outcome occurring. The authors then observed people's tendencies by designing a survey in which participants were told a story about an event that occurred, a man who got in a car crash, and were then asked to suggest the causes to which the family attributed the accident.

Depending on the version of the story that the participants were told, they were found to be more likely to point to different aspects of the story, such as the route the man drove, or the unusual way in which he entered the intersection where the crash happened. The clearest finding from their study was the \textit{downhill rule}, which says that people mentally undo events by removing unlikely occurrences. As the authors explain, ``a downhill change is one that removes a surprising or unexpected aspect of the story, or otherwise increases its internal coherence'' \citep{tversky1982simulation}.

The downhill rule suggests that people will assign blame to an attribute if it is easy to imagine a counterfactual situation where that attribute is changed, and the outcome is different. In the next section, we show how model explanation techniques build on this idea through their particular use of counterfactual reasoning. 

\subsection{Counterfactuals for model explanation}

Relying on counterfactuals is a natural idea in the context of model explanation. Machine learning models are functions on high dimensional domains, so to understand a model is to understand how it maps different inputs to different outputs. And any method that generates explanations by perturbing the input, whether it is by removing features or not, is based on some form of counterfactual reasoning.

Some work has embraced counterfactual reasoning by suggesting that model predictions should be explained by presenting users with a small number of counterfactual examples \citep{wachter2017counterfactual}. The authors suggest generating the nearest possible counterfactual that achieves a user-specified alternative outcome, which is reminiscent of the downhill rule \citep{tversky1982simulation}. In this approach, proximity is used as a placeholder for internal coherence when identifying counterfactual changes that can alter the outcome.

However, while a single counterfactual can suggest a direction for changing an outcome or for contesting an adverse decision, individual counterfactuals provide insufficient information for understanding each feature's influence on the model. For example, if there are multiple causes for an outcome (e.g., a person's loan application was approved because of a good credit score and a high income level), and the outcome can be changed by reversing any single cause, then the closest possible counterfactual may arbitrarily highlight one cause over another (e.g., by showing that a lower credit score would have led to the loan being rejected). The problem is that many counterfactuals may be required to understand a complex model.

When assessing whether a feature influences the model, the downhill rule suggests that we should determine whether the feature has a high likelihood alternative value that changes the model output. In the framework of removal-based explanations, methods do not perform a search over alternative values; but by \textit{removing} the feature, they integrate the model output over a distribution of alternative values (or in some cases, by setting the feature to a default value). The justification for this, in light of the downhill rule, is that if there are high likelihood values that change the model output, this influence will become apparent when integrating over the distribution.

Of particular note is the approach that marginalizes out missing features using the conditional distribution (the focus of Section~\ref{sec:information}). In this approach, counterfactuals are considered in proportion to their internal coherence, which is represented by the likelihood under the data distribution $p(X_{\bar S} \; | \; X_S) \propto p(X)$. This approach to removing features has a clear correspondence with the downhill rule observed by \cite{tversky1982simulation}.

The framework of removal-based explanations is based on summarizing the results of many counterfactuals, while, by contrast, the approach from \cite{wachter2017counterfactual} presents individual counterfactuals directly to users. When assessing the impact of removing a particular set of features, each set of counterfactuals varies from the original input in only those features, and their values are drawn from a distribution that ideally relates to the internal coherence of those different values.

A similar observation was made by \cite{merrick2019explanation}, who remarked that the process of summarizing many counterfactuals resembles the cognitive process described by Norm Theory \citep{kahneman1986norm}. In this cognitive theory, people are said to gather summary statistics from a mentally constructed set of recalled and simulated representations of a phenomena, such as loan application outcomes for people with a given age and income. Norm Theory provides a cognitive analogue to the process of making predictions while certain features are removed.

In summary, we have identified two well-known cognitive theories that provide a basis for the framework of removal-based explanations---the theory of mentally undoing \citep{tversky1982simulation} and Norm Theory \citep{kahneman1986norm}. We emphasize that these theories do not prescribe a precise approach to model explanation; rather, they provide reassurance that certain existing approaches have some degree of correspondence with how humans are thought to understand causality.
% We also emphasize that these theories relate to the idea of removing features, which is the first choice in our framework, but that they do not relate to what model behaviors should be analyzed (the second dimension), or how concise explanations should be generated (the third dimension).

\subsection{Simplicity versus completeness}

When generating explanations, there is a trade-off between the amount of information conveyed and the user's likelihood of drawing the right conclusions. An explanation that paints an incomplete picture may prove to be more useful, if the user can understand it better.

% For example,
On one end of the spectrum, an individual counterfactual is easy to process, but it may not convey much insight about how a model works \citep{wachter2017counterfactual}. By contrast, SHAP's feature attributions provide a more complex summary of each feature's impact on the model,
% represent a more complex explanation that summarizes each feature's impact on the model,
% SHAP is among the more complex explanation methods,
% and although SHAP is among the most widely used interpretability tools \citep{bhatt2020explainable},
but a recent user study showed that even savvy users were less likely to understand SHAP visualizations, and experienced a higher cognitive load than users who viewed explanations for simpler generalized additive models \citep{kaur2020interpreting}. Similarly, another user study found that longer explanations required more time and effort to understand, and in some cases impeded users' ability to draw appropriate conclusions \citep{lage2019human}.

We refer to this as the trade-off between simplicity and completeness, because explanations are typically more complex when they provide a more complete picture of the model. For the purpose of helping the user build a mental model of the machine learning model, or to be able to mentally simulate the model \citep{lipton2018mythos}, providing a more complete picture seems preferable. But complicated explanations will leave users cognitively overloaded, possibly leaving them with a false sense of understanding of the model, and may even leave them worse off.

Recognizing this trade-off and its implications for the utility of explanations motivates the consideration of simplicity as a design principle. Within our framework, we have the flexibility to strike a balance between completeness and simplicity. To avoid cognitively overloading users, one might focus on global explanations rather than local explanations. One approach is to provide visualizations that aggregate the results of many local explanations, such as global SHAP plots \citep{lundberg2020local}. Alternatively, we might focus on providing global explanations that represent the model's behavior across the entire dataset, such as SAGE or Shapley Effects \citep{covert2020understanding, owen2014sobol}.

Certain formats of explanations convey more information than others. Feature attributions provide a granular view of the model by citing every feature as a cause and quantifying each feature's influence. However, psychology research has shown that people report higher satisfaction with explanations that cite fewer causes \citep{thagard1989explanatory, read1993explanatory, lombrozo2007simplicity, miller2019explanation}. Users may therefore derive more insight from explanation that highlight fewer causes, such as the sparse feature attributions that LIME can provide \cite{ribeiro2016should}.

The feature selection explanations go even further in the direction of simplicity. These explanations cite fewer causes because they directly penalize the number of selected features (Section~\ref{sec:summarization_strategies}). Furthermore, they omit information about the granularity of each feature's influence. For a non-technical user, it may be preferable to communicate that a model's prediction was dominated by a small number of features; it may take a more sophisticated user to absorb each feature's numerical contribution, and to internalize the interpretation of each attribution value as an additive decomposition of the model's behavior with subsets of features (Section~\ref{sec:linear_models}).

Designers of explanation methods must be wary of overestimating people's abilities to store complex mental models \citep{norman1983some}, and the community can be mindful of this by tailoring explanations to the user's degree of sophistication. Savvy users may benefit from getting a more complete picture of the model, but non-technical users may get more out of explanations that convey less information.

% Script
% Simplicity is an important design principle, because if people don't understand an explanation, they won't draw the right conclusions.
% There's a tradeoff between providing a more complete picture of the model and a user digesting the information properly.
% Within our framework (but also among other methods), we have the ability to provide more or less information in an explanation.
% For more savvy users, we might provide more information (attribution). For less savvy users, we might provide less information.
% In both cases, our objective is to help people build mental models of the model (simulatibility). 

% User studies have not found the sources of people's confusion, but we speculate that it could arise from the complex algorithms that estimate SHAP values, from the amount of information conveyed in a feature attribution, or from the visualizations (force plots).
% We speculate that several factors contribute to a user's ability to understand an explanation method: the complexity of the algorithm that generates the explanation, of the explanation itself, and of the explanation's presentation.
% For our framework, the two sources of complexity that are most important to discuss are the complexity of the algorithm that generates the explanation, and the complexity of the explanation itself.

% For people to understand explanations and draw the right conclusions, they should ideally have an understanding of the process that generated the explanation. 

% Users should also have an understanding of the meaning of the explanation itself, independently of the algorithm that generated it. The methods discussed in this work produce only two kinds of explanations: feature attributions, and selections of the most important features.

% -

% Kaur: people don't understand SHAP as well as simpler methods, and it causes them to fail to answer questions based on visualizations, and leaves them with high cognitive load. Poursabzi and Lage also document problems with cognitive overload arising from model explanations.

% Bhatt: people rely on SHAP more than anything else.

% Lombrozo and Co.: people are more satisfied with explanations that cite few causes.

% Lipton: one thing that people should get from interpretability methods is ability to simulate a model. Relates to simulation heuristic (Kahneman), and also to mental models (Norman).

% Attributions help people simulate the model given subsets of features, by quantifying impact of including a feature. Selections say that the selected features on their own achieve roughly the same prediction.

% When people have a poor mental model of how an explanation is generated (e.g. Shapley values), possibly because the process is genuinely complicated, they will have a harder time drawing appropriate conclusions.

% -----From Kaur-----
% Kaur shows that ML practitioners can't explain how SHAP works. They report lower confidence, and they perform worse at answering questions based on it
% Poursabzi-Sangdeh finds that too much transparency into a model causes information overload and makes people follow a model even when it makes a mistake
% Lage finds that longer explanations overload people's cognitive abilities
% Lombrozo (and Miller) propose three criteria: simplicity, generality, and coherence. However, I don't yet know what they mean by generality and coherence in ML context!
% Their user studies show that people have lower confidence, less accurate answers to simple questions, and higher cognitive load with SHAP
% Norman (from HCI) suggests that it's important to have mental and conceptual model of a tool. If the tool is really complicated, it would be hard to have an accurate mental model

% -----From Bhatt-----
% More people use SHAP than anything else

% -----From Lipton-----
% Authors of interpretability papers have different ideas of what interpretability means, different goals
% What people might want from interpretability is an ability to simulate a model. Like forming a mental model of...the model

% -----From Lombrozo-----
% People prefer explanations that cite fewer propositions ("simpler" explanations). They appear to have a prior belief that there should be few causes
% People's preference for explanations was measured through "satisfaction," which is vague. Imagine that it has something to do with belief that the explanation (a speculation) is true
% There's competition between explanations with few causes and explanations whose causes are likely. People like both "simplicity" and probability
% Read paper, and another paper, both tried to get at simplicity and/or probability. They both bungled it. Serious confounding, and bad methodology
% Theory is that people place their prior belief on small number of causes. Possibly because they believe the world to be simple? 

% -----From Read-----
% People like simple explanations (fewer causes)
% Authors findings support Thagard's model (not just his principles)

% -----From Thagard-----
% Has a theory about principles that are relevant to acceptance of hypotheses about causes. Turns these principles into a model
% One aspect of the theory is the prediction that smaller sets of causes will be preferred. He did not test this, but multiple psychology papers took him up on it

% -----From Spellman 1996-----
% Intuitive scientists (like intuitive stasisticians)
% An existing normative rule for how people evaluate the influence of something is difference between probability of outcome with that treatment, and without it
% It had been observed that in instances with multiple causes, people do not use that rule. One theory was that people might conditionalize their influence estimation on some fixed causes
% Experiments provided evidence that this is true

% -----From Spellman 2001-----
% Same shit about how people conditionalize to evaluate influence. But who could advocate for not conditioning? Marginalizing gives a summary that is, in the best case, not misleading

% -----From Norman-----
% People have conceptions that they bring to any task. People form mental models of themselves and of the things they interact with. Mental models provide predictive and explanatory power over interactions
% Target system; conceptual model of target system; mental model of target system; scientist's conception of the mental model
% Conceptual models are invented by teachers, designers and engineers
% Mental models evolve naturally through interaction. They are usually not technically accurate, but ought to be "functional" (successfully predict aspects of interactions?). This is in line with Lipton's idea of simulatability
% Scientist's conceptualization is model of the mental model
% Lots of observations about people's mental models. One is that people's ability to run them is severely limited
% People have superstitions, maintain behavior that does not make sense but seems to work. Worried about fragility. Reduce mental effort but increase usage effort
% He's really talking about interaction with devices and maybe software. Will need to pick out ideas that are relevant to me
% There is often difference between conceptual model (model of how one should interact) and mental model (which governs how one interacts)
% The purpose of a mental model is to help a person understand and anticipate behavior of a system during an interaction. Would be helpful for someone to be able to run their model mentally
% I wonder what Norman has to say about design principles, and how it relates to someone's ability to form an accurate mental model
% For designer, goal is to design around a conceptual model that the user can replicate in their mental model. It should not be too complicated for them to learn. "it is our duty to develop conceptual models that will aid the learner to develop adequate and appropriate mental models"


% -----From Fiske and Taylor-----
% Can't access without buying it

